HeLP -- A GAP-package for torsion units in integral group rings

We briefly summarize the background of the HeLP-method for torsion units in group rings and present some functionality of a GAP-package implementing it.

==> cleveref.tex <==
%%
%% This is file `cleveref.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% cleveref.dtx  (with options: `package')
%% 
%% LaTeX package for automatic cross-referencing text.
%% 
%% Copyright (C) 2006  Toby Cubitt
%% See the files README and COPYING.
%% 
\def\packagedate{2012/01/18}
\def\packageversion{0.18.3}
%% This file may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.2
%% of this license or (at your option) any later version.
%% The latest version of this license is in:
%%
%%    http://www.latex-project.org/lppl.txt
%%
%% and version 1.2 or later is part of all distributions of LaTeX
%% version 1999/12/01 or later.
\NeedsTeXFormat{LaTeX2e}[1999/12/01]
\ProvidesPackage{cleveref}
 [\packagedate{} v\packageversion{} Intelligent cross-referencing]
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
\def\cref@currentlabel{}
\let\cref@old@refstepcounter\refstepcounter
\def\refstepcounter{%
  \@ifnextchar[{\refstepcounter@optarg}{\refstepcounter@noarg}%]
}
\def\refstepcounter@noarg#1{%
  \cref@old@refstepcounter{#1}%
  \cref@constructprefix{#1}{\cref@result}%
  \@ifundefined{cref@#1@alias}%
    {\def\@tempa{#1}}%
    {\def\@tempa{\csname cref@#1@alias\endcsname}}%
  \protected@xdef\cref@currentlabel{%
    [\@tempa][\arabic{#1}][\cref@result]%
    \csname p@#1\endcsname\csname the#1\endcsname}}
\def\refstepcounter@optarg[#1]#2{%
  \cref@old@refstepcounter{#2}%
  \cref@constructprefix{#2}{\cref@result}%
  \protected@xdef\cref@currentlabel{%
    [#1][\arabic{#2}][\cref@result]%
    \csname p@#2\endcsname\csname the#2\endcsname}}
\AtBeginDocument{%
  \let\cref@old@label\label
  \def\label{\@ifnextchar[\label@optarg\label@noarg}%]
  \let\cref@label\label
  \def\label@noarg#1{%
    \@bsphack%
    \cref@old@label{#1}%
    \protected@write\@auxout{}%
      {\string\newlabel{cref@#1}{{\cref@currentlabel}{\thepage}}}%
    \@esphack}%
  \def\label@optarg[#1]#2{%
    \@bsphack%
    \cref@old@label{#2}%
    \protected@xdef\cref@currentlabel{%
      \expandafter\cref@override@label@type%
        \cref@currentlabel\@nil{#1}}%
    \protected@write\@auxout{}%
      {\string\newlabel{cref@#2}{{\cref@currentlabel}{\thepage}}}%
    \@esphack}
}% end of AtBeginDocument
\let\cref@old@footnotetext\@footnotetext
\let\cref@old@mpfootnotetext\@mpfootnotetext
\def\@footnotetext{%
  \cref@constructprefix{footnote}{\cref@result}%
  \protected@xdef\cref@currentlabel{%
    [footnote][\arabic{footnote}][\cref@result]%
    \p@footnote\@thefnmark}%
  \cref@old@footnotetext}
\def\@mpfootnotetext#1{%
  \cref@constructprefix{mpfootnote}{\cref@result}%
  \protected@xdef\cref@currentlabel{%
    [footnote][\arabic{mpfootnote}][\cref@result]%
    \p@footnote\@thefnmark}%
  \cref@old@mpfootnotetext{#1}}
\let\cref@old@othm\@othm
\def\@othm#1[#2]#3{%
  \edef\@tempa{\expandafter\noexpand%
    \csname cref@#1@name@preamble\endcsname}%
  \edef\@tempb{\expandafter\noexpand%
      \csname Cref@#1@name@preamble\endcsname}%
  \def\@tempc{#3}%
  \ifx\@tempc\@empty\relax%
    \expandafter\gdef\@tempa{}%
    \expandafter\gdef\@tempb{}%
  \else%
    \if@cref@capitalise%
      \expandafter\expandafter\expandafter\gdef\expandafter%
        \@tempa\expandafter{\MakeUppercase #3}%
    \else%
      \expandafter\expandafter\expandafter\gdef\expandafter%
        \@tempa\expandafter{\MakeLowercase #3}%
    \fi%
    \expandafter\expandafter\expandafter\gdef\expandafter%
      \@tempb\expandafter{\MakeUppercase #3}%
  \fi%
  \cref@stack@add{#1}{\cref@label@types}%
  \cref@old@othm{#1}[#2]{#3}}
\let\cref@old@xnthm\@xnthm
\def\@xnthm#1#2[#3]{%
  \edef\@tempa{\expandafter\noexpand%
    \csname cref@#1@name@preamble\endcsname}%
  \edef\@tempb{\expandafter\noexpand%
      \csname Cref@#1@name@preamble\endcsname}%
  \def\@tempc{#2}%
  \ifx\@tempc\@empty\relax%
    \expandafter\gdef\@tempa{}%
    \expandafter\gdef\@tempb{}%
  \else%
    \if@cref@capitalise%
      \expandafter\expandafter\expandafter\gdef\expandafter%
        \@tempa\expandafter{\MakeUppercase #2}%
    \else%
      \expandafter\expandafter\expandafter\gdef\expandafter%
        \@tempa\expandafter{\MakeLowercase #2}%
    \fi%
    \expandafter\expandafter\expandafter\gdef\expandafter%
      \@tempb\expandafter{\MakeUppercase #2}%
  \fi%
  \cref@stack@add{#1}{\cref@label@types}%
  \cref@old@xnthm{#1}{#2}[#3]}
\let\cref@old@ynthm\@ynthm
\def\@ynthm#1#2{%
  \edef\@tempa{\expandafter\noexpand%
    \csname cref@#1@name@preamble\endcsname}%
  \edef\@tempb{\expandafter\noexpand%
      \csname Cref@#1@name@preamble\endcsname}%
  \def\@tempc{#2}%
  \ifx\@tempc\@empty\relax%
    \expandafter\gdef\@tempa{}%
    \expandafter\gdef\@tempb{}%
  \else%
    \if@cref@capitalise%
      \expandafter\expandafter\expandafter\gdef\expandafter%
        \@tempa\expandafter{\MakeUppercase #2}%
    \else%
      \expandafter\expandafter\expandafter\gdef\expandafter%
        \@tempa\expandafter{\MakeLowercase #2}%
    \fi%
    \expandafter\expandafter\expandafter\gdef\expandafter%
      \@tempb\expandafter{\MakeUppercase #2}%
  \fi%
  \cref@stack@add{#1}{\cref@label@types}%
  \cref@old@ynthm{#1}{#2}}
\@ifundefined{appendix}{}{%
  \let\cref@old@appendix\appendix
  \renewcommand\appendix{%
    \cref@old@appendix%
    \@ifundefined{chapter}{%
      \gdef\refstepcounter@noarg##1{%
        \cref@old@refstepcounter{##1}%
        \cref@constructprefix{##1}{\cref@result}%
        \ifx\cref@result\@empty%
          \def\cref@result{2147483647}%
        \else%
          \edef\cref@result{2147483647,\cref@result}%
        \fi%
        \def\@tempa{##1}%
        \def\@tempb{section}%
        \ifx\@tempa\@tempb%
          \protected@xdef\cref@currentlabel{%
            [appendix][\arabic{##1}][\cref@result]%
            \csname p@##1\endcsname\csname the##1\endcsname}%
        \else%
          \def\@tempa{##1}%
          \def\@tempb{subsection}%
          \ifx\@tempa\@tempb%
            \protected@xdef\cref@currentlabel{%
              [subappendix][\arabic{##1}][\cref@result]%
              \csname p@##1\endcsname\csname the##1\endcsname}%
          \else%
            \def\@tempa{##1}%
            \def\@tempb{subsubsection}%
            \ifx\@tempa\@tempb%
              \protected@xdef\cref@currentlabel{%
                [subsubappendix][\arabic{##1}][\cref@result]%
                \csname p@##1\endcsname\csname the##1\endcsname}%
            \else%
              \@ifundefined{cref@##1@alias}%
                {\def\@tempa{##1}}%
                {\def\@tempa{\csname cref@##1@alias\endcsname}}%
              \protected@xdef\cref@currentlabel{%
                [\@tempa][\arabic{##1}][\cref@result]%
                \csname p@##1\endcsname\csname the##1\endcsname}
            \fi%
          \fi%
        \fi}%
    }{%
      \def\refstepcounter@noarg##1{%
        \cref@old@refstepcounter{##1}%
        \cref@constructprefix{##1}{\cref@result}%
        \ifx\cref@result\@empty%
          \def\cref@result{2147483647}%
        \else%
          \edef\cref@result{2147483647,\cref@result}%
        \fi%
        \def\@tempa{##1}%
        \def\@tempb{chapter}%
        \ifx\@tempa\@tempb%
          \protected@xdef\cref@currentlabel{%
            [appendix][\arabic{##1}][\cref@result]%
            \csname p@##1\endcsname\csname the##1\endcsname}%
        \else%
          \def\@tempa{##1}%
          \def\@tempb{section}%
          \ifx\@tempa\@tempb%
            \protected@xdef\cref@currentlabel{%
              [subappendix][\arabic{##1}][\cref@result]%
              \csname p@##1\endcsname\csname the##1\endcsname}%
          \else%
            \def\@tempa{##1}%
            \def\@tempb{subsection}%
            \ifx\@tempa\@tempb%
              \protected@xdef\cref@currentlabel{%
                [subsubappendix][\arabic{##1}][\cref@result]%
                \csname p@##1\endcsname\csname the##1\endcsname}%
            \else%
              \def\@tempa{##1}%
              \def\@tempb{subsubsection}%
              \ifx\@tempa\@tempb%
                \protected@xdef\cref@currentlabel{%
                  [subsubsubappendix][\arabic{##1}][\cref@result]%
                  \csname p@##1\endcsname\csname the##1\endcsname}%
              \else%
                \@ifundefined{cref@##1@alias}%
                  {\def\@tempa{##1}}%
                  {\def\@tempa{\csname cref@##1@alias\endcsname}}%
                \protected@xdef\cref@currentlabel{%
                  [\@tempa][\arabic{##1}][\cref@result]%
                  \csname p@##1\endcsname\csname the##1\endcsname}
              \fi%
            \fi%
          \fi%
        \fi}%
    }%
  }%
}% end of \@ifundefined{appendix}
\def\@gobble@optarg{\@ifnextchar[\@@gobble@optarg\@gobble@orig}%]
\def\@gobble@orig#1{}
\def\@@gobble@optarg[#1]#2{}
\def\cref@append@toks#1#2{\toks0={#2}%
  \edef\act{\noexpand#1={\the#1\the\toks0}}%
  \act}%
\def\cref@getref#1#2{%
  \expandafter\let\expandafter#2\csname r@cref@#1\endcsname%
  \expandafter\expandafter\expandafter\def%
    \expandafter\expandafter\expandafter#2%
    \expandafter\expandafter\expandafter{%
      \expandafter\@firstoftwo#2}}
\def\cref@getpageref#1#2{%
  \expandafter\let\expandafter#2\csname r@cref@#1\endcsname%
  \expandafter\expandafter\expandafter\def%
    \expandafter\expandafter\expandafter#2%
    \expandafter\expandafter\expandafter{%
      \expandafter\@secondoftwo#2}}
\def\cref@getlabel#1#2{%
  \cref@getref{#1}{\@tempa}%
  \expandafter\@cref@getlabel\@tempa\@nil#2}%
\def\@cref@getlabel{\@ifnextchar[%]
  \@@cref@getlabel{\@@cref@getlabel[][][]}}
\def\@@cref@getlabel[#1][#2][#3]#4\@nil#5{\def#5{#4}}
\def\cref@gettype#1#2{%
  \cref@getref{#1}{\@tempa}%
  \expandafter\@cref@gettype\@tempa\@nil#2}%
\def\@cref@gettype{\@ifnextchar[%]
  \@@cref@gettype{\@@cref@gettype[][][]}}
\def\@@cref@gettype[#1][#2][#3]#4\@nil#5{\def#5{#1}}
\def\cref@getcounter#1#2{%
  \cref@getref{#1}{\@tempa}%
  \expandafter\@cref@getcounter\@tempa\@nil#2}
\def\@cref@getcounter{\@ifnextchar[%]
  \@@cref@getcounter{\@@cref@getcounter[][][]}}
\def\@@cref@getcounter[#1][#2][#3]#4\@nil#5{\def#5{#2}}
\def\cref@getprefix#1#2{%
  \cref@getref{#1}{\@tempa}%
  \expandafter\@cref@getprefix\@tempa\@nil#2}
\def\@cref@getprefix{\@ifnextchar[%]
  \@@cref@getprefix{\@@cref@getprefix[][][]}}
\def\@@cref@getprefix[#1][#2][#3]#4\@nil#5{\def#5{#3}}
\def\cref@override@label@type[#1][#2][#3]#4\@nil#5{[#5][#2][#3]#4}
\def\cref@constructprefix#1#2{%
  \cref@stack@init{\@tempstack}%
  \edef\@tempa{\noexpand{#1\noexpand}}%
  \expandafter\def\expandafter\@tempa\expandafter{\@tempa{#2}}%
  \expandafter\@cref@constructprefix\@tempa%
  \cref@stack@to@list{\@tempstack}{\@tempa}%
  \expandafter\def\expandafter#2\expandafter{\@tempa}}
\def\@cref@constructprefix#1#2{%
  \cref@resetby{#1}{#2}%
  \ifx#2\relax%
  \else%
    \edef\@tempa{\the\csname c@#2\endcsname}%
    \expandafter\cref@stack@push\expandafter{\@tempa}{\@tempstack}%
    \edef\@tempa{{#2}}%
    \expandafter\expandafter\expandafter\@cref@constructprefix%
      \expandafter\@tempa\expandafter{\expandafter#2\expandafter}%
  \fi}
\def\cref@stack@init#1{\def#1{\@nil}}
\def\cref@stack@top#1{\expandafter\@cref@stack@top#1}
\def\@cref@stack@top#1,#2\@nil{#1}
\def\cref@stack@pop#1{\expandafter\@cref@stack@pop#1#1}
\def\@cref@stack@pop#1,#2\@nil#3{\def#3{#2\@nil}}
\def\cref@stack@push#1#2{%
  \expandafter\@cref@stack@push\expandafter{#2}{#1}{#2}}
\def\@cref@stack@push#1#2#3{\def#3{#2,#1}}
\def\cref@stack@pull#1#2{\expandafter\@cref@stack@pull#2{#1}{#2}}
\def\@cref@stack@pull#1\@nil#2#3{\def#3{#1#2,\@nil}}
\def\cref@stack@to@list#1#2{%
  \cref@isstackfull{#1}%
  \if@cref@stackfull%
    \expandafter\expandafter\expandafter\def%
    \expandafter\expandafter\expandafter#2%
    \expandafter\expandafter\expandafter{%
      \expandafter\@cref@stack@to@list#1}%
  \else%
    \def#2{}%
  \fi}
\def\@cref@stack@to@list#1,\@nil{#1}
\def\cref@stack@topandbottom#1#2#3{%
  \def#2{}%
  \def#3{}%
  \cref@isstackfull{#1}%
  \if@cref@stackfull%
    \edef#2{\cref@stack@top{#1}}%
    \cref@stack@pop{#1}%
    \cref@isstackfull{#1}%
    \@whilesw\if@cref@stackfull\fi{%
      \edef#3{\cref@stack@top{#1}}%
      \cref@stack@pop{#1}%
      \cref@isstackfull{#1}}%
  \fi}
\def\cref@stack@add#1#2{%
  \begingroup%
    \def\@arg1{#1}%
    \let\@tempstack#2%
    \newif\if@notthere%
    \@nottheretrue%
    \cref@isstackfull{\@tempstack}%
    \@whilesw\if@cref@stackfull\fi{%
      \edef\@tempb{\cref@stack@top{\@tempstack}}%
      \def\@tempa{#1}%
      \ifx\@tempa\@tempb%
        \@cref@stackfullfalse%
        \@nottherefalse%
      \else%
        \cref@stack@pop{\@tempstack}%
        \cref@isstackfull{\@tempstack}%
      \fi}%
  \expandafter\endgroup%
  \if@notthere\cref@stack@push{#1}{#2}\fi}
\newif\if@cref@stackempty
\newif\if@cref@stackfull
\def\cref@isstackempty#1{%
  \def\@tempa{\@nil}%
  \ifx#1\@tempa\@cref@stackemptytrue%
  \else\@cref@stackemptyfalse\fi}
\def\cref@isstackfull#1{%
  \def\@tempa{\@nil}%
  \ifx#1\@tempa\@cref@stackfullfalse%
  \else\@cref@stackfulltrue\fi}
\def\cref@stack@sort#1#2{%
  \begingroup%
  \cref@stack@init{\@sortstack}%
  \edef\@element{\cref@stack@top{#1}}%
  \expandafter\cref@stack@push\expandafter{\@element}{\@sortstack}%
  \cref@stack@pop{#1}%
  \cref@isstackfull{#1}%
  \if@cref@stackfull%
    \edef\@tempa{\cref@stack@top{#1}}%
    \@whilesw\ifx\@tempa\@empty\fi{%
      \cref@stack@pull{}{\@sortstack}%
      \cref@stack@pop{#1}%
      \cref@isstackempty{#1}%
      \if@cref@stackempty%
        \let\@tempa\relax%
      \else%
        \edef\@tempa{\cref@stack@top{#1}}%
      \fi}%
  \fi%
  \cref@isstackfull{#1}%
  \@whilesw\if@cref@stackfull\fi{%
    \edef\@element{\cref@stack@top{#1}}%
    \cref@stack@pop{#1}%
    \def\@empties{}%
    \cref@isstackfull{#1}%
    \if@cref@stackfull%
      \edef\@tempa{\cref@stack@top{#1}}%
      \@whilesw\ifx\@tempa\@empty\fi{%
        \edef\@empties{\@empties,}%
        \cref@stack@pop{#1}%
        \cref@isstackempty{#1}%
        \if@cref@stackempty%
          \let\@tempa\relax%
        \else%
          \edef\@tempa{\cref@stack@top{#1}}%
        \fi}%
    \fi%
    \edef\@tempa{{\expandafter\noexpand\@element}%
      {\expandafter\noexpand\@empties}%
      {\noexpand\@sortstack}{\noexpand#2}}%
    \expandafter\cref@stack@insert\@tempa%
    \cref@isstackfull{#1}}%
  \expandafter\endgroup\expandafter%
  \def\expandafter#1\expandafter{\@sortstack}}
\def\cref@stack@insert#1#2#3#4{%
  \let\@cmp#4%
  \@cref@stack@insert{}{#1}{#2}{#3}%
  \cref@stack@pop{#3}}
\def\@cref@stack@insert#1#2#3#4{%
  \let\cref@iterate\relax%
  \cref@isstackempty{#4}%
  \if@cref@stackempty%
    \cref@stack@push{#1,#2#3}{#4}%
  \else%
    \edef\cref@elem{\cref@stack@top{#4}}%
    \expandafter\@cmp\expandafter{\cref@elem}{#2}{\cref@result}%
    \ifnum\cref@result=2\relax%
      \cref@stack@push{#1,#2#3}{#4}%
    \else%
      \cref@stack@pop{#4}%
      \edef\cref@elem{{\noexpand#1,\cref@elem}{\noexpand#2}%
        {\noexpand#3}{\noexpand#4}}%
      \expandafter\def\expandafter\cref@iterate\expandafter%
        {\expandafter\@cref@stack@insert\cref@elem}%
    \fi%
  \fi%
  \cref@iterate}
\def\cref@counter@first#1#2\@nil{#1}
\def\cref@counter@rest#1#2\@nil{#2}
\def\cref@countercmp#1#2#3{%
  \begingroup%
  \def\@tempa{#1}%
  \ifx\@tempa\@empty%
    \def\cref@result{1}%
  \else%
    \def\@tempa{#2}%
    \ifx\@tempa\@empty%
      \def\cref@result{2}%
    \else%
      \expandafter\ifx\csname r@cref@#1\endcsname\relax%
        \def\cref@result{2}%
      \else%
        \expandafter\ifx\csname r@cref@#2\endcsname\relax%
          \def\cref@result{1}%
        \else%
          \cref@getcounter{#1}{\@countera}%
          \cref@getprefix{#1}{\@prefixa}%
          \cref@getcounter{#2}{\@counterb}%
          \cref@getprefix{#2}{\@prefixb}%
          \cref@stack@init{\@countstacka}%
          \expandafter\cref@stack@push\expandafter%
            {\@countera}{\@countstacka}%
          \ifx\@prefixa\@empty\else%
            \expandafter\cref@stack@push\expandafter%
              {\@prefixa}{\@countstacka}%
          \fi%
          \cref@stack@init{\@countstackb}%
          \expandafter\cref@stack@push\expandafter%
            {\@counterb}{\@countstackb}%
          \ifx\@prefixb\@empty\else%
            \expandafter\cref@stack@push\expandafter%
              {\@prefixb}{\@countstackb}%
          \fi%
          \@cref@countercmp%
        \fi%
      \fi%
    \fi%
  \fi%
  \expandafter\endgroup\expandafter%
  \chardef\expandafter#3\expandafter=\cref@result\relax}
\def\@cref@countercmp{%
  \let\@iterate\relax%
  \cref@isstackempty{\@countstacka}%
  \if@cref@stackempty%
    \cref@isstackempty{\@countstackb}%
    \if@cref@stackempty%
      \def\cref@result{0}%
    \else%
      \def\cref@result{1}%
    \fi%
  \else%
    \cref@isstackempty{\@countstackb}%
    \if@cref@stackempty%
      \def\cref@result{2}%
    \else%
      \edef\@tempa{\cref@stack@top{\@countstacka}}%
      \cref@stack@pop{\@countstacka}%
      \edef\@tempb{\cref@stack@top{\@countstackb}}%
      \cref@stack@pop{\@countstackb}%
      \ifnum\@tempa<\@tempb\relax%
        \def\cref@result{1}%
      \else%
        \ifnum\@tempa>\@tempb\relax%
          \def\cref@result{2}%
        \else%
          \def\@iterate{\@cref@countercmp}%
        \fi%
      \fi%
    \fi%
  \fi%
  \@iterate}
\def\cref@pagecmp#1#2#3{%
  \begingroup%
  \def\@tempa{#1}%
  \ifx\@tempa\@empty%
    \def\cref@result{1}%
  \else%
    \def\@tempa{#2}%
    \ifx\@tempa\@empty%
      \def\cref@result{2}%
    \else%
      \expandafter\ifx\csname r@cref@#1\endcsname\relax%
        \def\cref@result{2}%
      \else%
        \expandafter\ifx\csname r@cref@#2\endcsname\relax%
          \def\cref@result{1}%
        \else%
          \cref@getpageref{#1}{\@tempa}%
          \cref@getpageref{#2}{\@tempb}%
          \ifnum\@tempa<\@tempb\relax%
            \def\cref@result{1}\relax%
          \else%
            \ifnum\@tempa>\@tempb\relax%
              \def\cref@result{2}\relax%
                \else%
              \def\cref@result{0}\relax%
            \fi%
          \fi%
        \fi%
      \fi%
    \fi%
  \fi%
  \expandafter\endgroup\expandafter%
  \chardef\expandafter#3\expandafter=\cref@result\relax}
\newif\if@cref@inresetlist
\def\cref@isinresetlist#1#2{%
  \begingroup%
    \def\@counter{#1}%
    \def\@elt##1{##1,}%
    \expandafter\ifx\csname cl@#2\endcsname\relax%
      \def\cref@resetstack{,\@nil}%
    \else%
      \edef\cref@resetstack{\csname cl@#2\endcsname\noexpand\@nil}%
    \fi%
    \let\@nextcounter\relax%
    \cref@isstackfull{\cref@resetstack}%
    \@whilesw\if@cref@stackfull\fi{%
      \edef\@nextcounter{\cref@stack@top{\cref@resetstack}}%
      \ifx\@nextcounter\@counter%
        \@cref@stackfullfalse%
      \else%
        \let\@nextcounter\relax%
        \cref@stack@pop{\cref@resetstack}%
        \cref@isstackfull{\cref@resetstack}%
      \fi}%
    \ifx\@nextcounter\relax%
      \def\@next{\@cref@inresetlistfalse}%
    \else%
      \def\@next{\@cref@inresetlisttrue}%
    \fi%
  \expandafter%
  \endgroup%
  \@next}
\def\cref@resetby#1#2{%
  \let#2\relax%
  \def\@tempa{#1}%
  \def\@tempb{subfigure}%
  \ifx\@tempa\@tempb%
    \cref@isinresetlist{#1}{figure}%
    \if@cref@inresetlist%
      \def#2{figure}%
    \fi%
  \fi%
  \def\@tempa{#1}%
  \def\@tempb{subtable}%
  \ifx\@tempa\@tempb%
    \cref@isinresetlist{#1}{table}%
    \if@cref@inresetlist%
      \def#2{table}%
    \fi%
  \fi%
  \@ifundefined{cl@parentequation}{}{%
    \def\@tempa{#1}%
    \def\@tempb{equation}%
    \ifx\@tempa\@tempb%
      \cref@isinresetlist{#1}{parentequation}%
      \if@cref@inresetlist%
        \expandafter\ifnum\c@parentequation=0\else%
          \def#2{parentequation}%
        \fi%
      \fi%
    \fi}%
  \def\@tempa{#1}%
  \def\@tempb{enumii}%
  \ifx\@tempa\@tempb%
    \def#2{enum}%
  \fi%
  \def\@tempb{enumiii}%
  \ifx\@tempa\@tempb%
    \def#2{enum}%
  \fi%
  \def\@tempb{enumiv}%
  \ifx\@tempa\@tempb%
    \def#2{enum}%
  \fi%
  \def\@tempb{enumv}%
  \ifx\@tempa\@tempb%
    \def#2{enum}%
  \fi%
  \def\@tempb{enum}%
  \ifx#2\@tempb%
    \cref@isinresetlist{#1}{enumiv}%
    \if@cref@inresetlist%
      \def#2{enumiv}%
    \else%
      \cref@isinresetlist{#1}{enumiii}%
      \if@cref@inresetlist%
        \def#2{enumiii}%
      \else%
        \cref@isinresetlist{#1}{enumii}%
        \if@cref@inresetlist%
          \def#2{enumii}%
        \else%
          \cref@isinresetlist{#1}{enumi}%
          \if@cref@inresetlist%
            \def#2{enumi}%
          \else%
           \cref@isinresetlist{#1}{part}%
            \if@cref@inresetlist%
              \def#2{part}%
            \else%
              \let#2\relax%
            \fi%
          \fi%
        \fi%
      \fi%
    \fi%
  \fi%
  \ifx#2\relax%
    \cref@isinresetlist{#1}{table}%
    \if@cref@inresetlist%
      \def#2{table}%
    \else%
      \cref@isinresetlist{#1}{subsubsection}%
      \if@cref@inresetlist%
        \def#2{subsubsection}%
      \else%
        \cref@isinresetlist{#1}{subsection}%
        \if@cref@inresetlist%
          \def#2{subsection}%
        \else%
          \cref@isinresetlist{#1}{section}%
          \if@cref@inresetlist%
            \def#2{section}%
          \else%
            \cref@isinresetlist{#1}{chapter}%
            \if@cref@inresetlist%
              \def#2{chapter}%
            \else%
             \cref@isinresetlist{#1}{part}%
              \if@cref@inresetlist%
                \def#2{part}%
              \else%
                \let#2\relax%
              \fi%
            \fi%
          \fi%
        \fi%
      \fi%
    \fi%
  \fi}
\newif\if@cref@refconsecutive%
\def\cref@isrefconsecutive#1#2{%
  \begingroup%
    \countdef\refa@counter=0%
    \countdef\refb@counter=1%
    \cref@getcounter{#1}{\cref@result}%
    \refa@counter=\cref@result%
    \cref@getcounter{#2}{\cref@result}%
    \refb@counter=\cref@result%
    \cref@getprefix{#1}{\refa@prefix}%
    \cref@getprefix{#2}{\refb@prefix}%
    \def\@after{\@cref@refconsecutivefalse}%
    \ifx\refa@prefix\refb@prefix%
      \ifnum\refa@counter=\refb@counter\relax%
        \def\@after{\@cref@refconsecutivetrue}%
      \else%
        \advance\refa@counter 1\relax%
        \ifnum\refa@counter=\refb@counter\relax%
          \def\@after{\@cref@refconsecutivetrue}%
        \fi%
      \fi%
    \fi%
  \expandafter\endgroup\@after}
\def\cref@ispagerefconsecutive#1#2{%
  \begingroup%
  \countdef\refa@counter=0%
  \countdef\refb@counter=1%
  \cref@getpageref{#1}{\cref@result}%
  \refa@counter=\cref@result%
  \cref@getpageref{#2}{\cref@result}%
  \refb@counter=\cref@result%
  \def\@after{\@cref@refconsecutivefalse}%
  \ifnum\refa@counter=\refb@counter\relax%
    \def\@after{\@cref@refconsecutivetrue}%
  \else%
    \advance\refa@counter 1\relax%
    \ifnum\refa@counter=\refb@counter\relax%
      \def\@after{\@cref@refconsecutivetrue}%
    \fi%
  \fi%
  \expandafter\endgroup\@after}
\def\cref@processgroup#1#2{%
  \edef\@nextref{\cref@stack@top{#1}}%
  \expandafter\ifx\csname r@cref@\@nextref\endcsname\relax%
    \def\@grouptype{\@undefined}%
    \def\@groupformat{\@undefined}%
  \else%
    \expandafter\cref@gettype\expandafter{\@nextref}{\@grouptype}%
    \expandafter\expandafter\expandafter\def%
      \expandafter\expandafter\expandafter\@groupformat%
      \expandafter\expandafter\expandafter{%
        \csname cref@\@grouptype @format\endcsname%
        {\@dummya}{\@dummyb}{\@dummyc}}%
  \fi%
  \let\@nexttype\@grouptype%
  \let\@nextformat\@groupformat%
  \@whilesw\ifx\@nextformat\@groupformat\fi{%
    \expandafter\cref@stack@pull\expandafter{\@nextref}{#2}%
    \cref@stack@pop{#1}%
    \cref@isstackempty{#1}%
    \if@cref@stackempty%
      \let\@nexttype\relax%
      \let\@nextformat\relax%
    \else%
      \edef\@nextref{\cref@stack@top{#1}}%
      \ifx\@nextref\@empty%
        \let\@nexttype\@grouptype%
        \let\@nextforamt\@groupformat%
      \else%
        \expandafter\ifx\csname r@cref@\@nextref\endcsname\relax%
          \def\@nexttype{\@undefined}%
          \def\@nextformat{\@undefined}%
        \else%
          \expandafter\cref@gettype\expandafter%
            {\@nextref}{\@nexttype}%
          \def\@tempa{\@undefined}%
          \ifx\@nexttype\@tempa%
            \def\@nextformat{\@undefined}%
          \else%
            \expandafter\expandafter\expandafter\def%
              \expandafter\expandafter\expandafter\@nextformat%
              \expandafter\expandafter\expandafter{%
                \csname cref@\@nexttype @format\endcsname%
                {\@dummya}{\@dummyb}{\@dummyc}}%
          \fi%
        \fi%
      \fi%
    \fi}%
}
\def\cref@processgroupall#1#2{%
  \cref@stack@init{\@tempstack}%
  \edef\@nextref{\cref@stack@top{#1}}%
  \expandafter\ifx\csname r@cref@\@nextref\endcsname\relax%
    \def\@grouptype{\@undefined}%
    \def\@groupformat{\@undefined}%
  \else%
    \expandafter\cref@gettype\expandafter{\@nextref}{\@grouptype}%
    \expandafter\expandafter\expandafter\def%
      \expandafter\expandafter\expandafter\@groupformat%
      \expandafter\expandafter\expandafter{%
        \csname cref@\@grouptype @format\endcsname%
        {\@dummya}{\@dummyb}{\@dummyc}}%
  \fi%
  \let\@lasttype\@grouptype%
  \let\@lastformat\@groupformat%
  \cref@isstackfull{#1}%
  \@whilesw\if@cref@stackfull\fi{%
    \edef\@nextref{\cref@stack@top{#1}}%
    \ifx\@nextref\@empty%
      \ifx\@lastformat\@groupformat%
        \let\@nexttype\@grouptype%
        \let\@nextformat\@groupformat%
      \else%
        \let\@nexttype\relax%
        \let\@nextformat\relax%
      \fi%
    \else%
      \expandafter\ifx\csname r@cref@\@nextref\endcsname\relax%
        \def\@nexttype{\@undefined}%
        \def\@nextformat{\@undefined}%
      \else%
        \expandafter\cref@gettype\expandafter%
          {\@nextref}{\@nexttype}%
        \def\@tempa{\@undefined}%
        \ifx\@nexttype\@tempa%
          \def\@nextformat{\@undefined}%
        \else%
          \expandafter\expandafter\expandafter\def%
            \expandafter\expandafter\expandafter\@nextformat%
            \expandafter\expandafter\expandafter{%
              \csname cref@\@nexttype @format\endcsname%
              {\@dummya}{\@dummyb}{\@dummyc}}%
        \fi%
      \fi%
    \fi%
    \ifx\@nextformat\@groupformat%
      \expandafter\cref@stack@pull\expandafter{\@nextref}{#2}%
    \else%
      \expandafter\cref@stack@pull\expandafter{\@nextref}{\@tempstack}%
    \fi%
    \cref@stack@pop{#1}%
    \let\@lasttype\@nexttype%
    \let\@lastformat\@nextformat%
    \cref@isstackfull{#1}}%
  \let#1\@tempstack}
\def\cref@processconsecutive#1#2#3#4#5{%
  #4=0%
  \edef\@nextref{\cref@stack@top{#1}}%
  \cref@stack@pop{#1}%
  \cref@isstackempty{#1}%
  \if@cref@stackempty%
    \edef#2{\@nextref}%
    \let#3\relax%
    #4=1\relax%
  \else%
    \edef#2{\@nextref}%
    \let#3\relax%
    \edef\@nextref{\cref@stack@top{#1}}%
    #4=1\relax%
    \expandafter\ifx\csname r@cref@#2\endcsname\relax%
      \@cref@refconsecutivefalse%
    \else%
      \ifx\@nextref\@empty%
        \@cref@refconsecutivefalse%
        \@whilesw\ifx\@nextref\@empty\fi{%
          \cref@stack@pop{#1}%
          \cref@isstackempty{#1}%
          \if@cref@stackempty%
            \let\@nextref\relax%
          \else%
            \edef\@nextref{\cref@stack@top{#1}}%
          \fi}%
      \else%
        \expandafter\ifx\csname r@cref@\@nextref\endcsname\relax%
          \@cref@refconsecutivefalse%
        \else%
          \edef\@tempa{{#2}{\@nextref}}%
          \expandafter#5\@tempa%
        \fi%
      \fi%
    \fi%
    \@whilesw\if@cref@refconsecutive\fi{%
      \advance#4 1%
      \let#3\@nextref%
      \cref@stack@pop{#1}%
      \cref@isstackempty{#1}%
      \if@cref@stackempty%
        \@cref@refconsecutivefalse%
      \else%
        \edef\@nextref{\cref@stack@top{#1}}%
        \ifx\@nextref\@empty%
          \@cref@refconsecutivefalse%
          \@whilesw\ifx\@nextref\@empty\fi{%
            \cref@stack@pop{#1}%
            \cref@isstackempty{#1}%
            \if@cref@stackempty%
              \let\@nextref\relax%
            \else%
              \edef\@nextref{\cref@stack@top{#1}}%
            \fi}%
        \else%
          \expandafter\ifx\csname r@cref@\@nextref\endcsname\relax%
            \@cref@refconsecutivefalse%
          \else%
            \edef\@tempa{{#3}{\@nextref}}%
            \expandafter#5\@tempa%
          \fi%
        \fi%
      \fi}%
  \fi}
\DeclareRobustCommand{\cref}[1]{\@cref{cref}{#1}}
\DeclareRobustCommand{\Cref}[1]{\@cref{Cref}{#1}}
\DeclareRobustCommand{\crefrange}[2]{\@setcrefrange{#1}{#2}{cref}{}}
\DeclareRobustCommand{\Crefrange}[2]{\@setcrefrange{#1}{#2}{Cref}{}}
\@ifpackageloaded{hyperref}{\newif\if@crefstarred}{%
  \@ifpackageloaded{varioref}{\newif\if@crefstarred}{}}
\let\if@crefstarred\iffalse%
\def\@cref#1#2{%
  \leavevmode%
  \begingroup%
  \countdef\count@consecutive=0%
  \countdef\count@group=1%
  \count@group=1%
  \def\cref@variant{#1}%
  \newif\if@secondref%
  \cref@stack@init{\@refstack}%
  \edef\@tempa{#2}%
  \expandafter\cref@stack@push\expandafter{\@tempa}{\@refstack}%
  \cref@isstackfull{\@refstack}%
  \@whilesw\if@cref@stackfull\fi{%
    \cref@stack@init{\@refsubstack}%
    \if@cref@sort%
      \cref@processgroupall{\@refstack}{\@refsubstack}%
      \cref@stack@sort{\@refsubstack}{\cref@countercmp}%
    \else%
      \cref@processgroup{\@refstack}{\@refsubstack}%
    \fi%
    \ifnum\count@group=1\relax%
      \advance\count@group 1%
    \else%
      \cref@isstackfull{\@refstack}%
      \if@cref@stackfull%
        \@setcref@middlegroupconjunction%
      \else%
        \ifnum\count@group=2\relax%
          \@setcref@pairgroupconjunction%
        \else%
          \@setcref@lastgroupconjunction%
        \fi%
      \fi%
      \advance\count@group 1%
      \def\cref@variant{cref}%
    \fi%
    \if@cref@compress%
      \cref@processconsecutive%
        {\@refsubstack}{\@beginref}{\@endref}{\count@consecutive}%
        {\cref@isrefconsecutive}%
    \else%
      \edef\@beginref{\cref@stack@top{\@refsubstack}}%
      \cref@stack@pop{\@refsubstack}%
      \@whilesw\ifx\@beginref\@empty\fi{%
        \cref@stack@pop{\@refsubstack}%
        \cref@isstackempty{\@refsubstack}%
        \if@cref@stackempty%
          \let\@beginref\relax%
        \else%
          \edef\@beginref{\cref@stack@top{\@refsubstack}}%
        \fi}%
      \let\@endref\relax%
      \count@consecutive=1\relax%
    \fi%
    \ifnum\count@consecutive=1\relax%
      \cref@isstackfull{\@refsubstack}%
      \if@cref@stackfull%
        \expandafter\@setcref%
          \expandafter{\@beginref}{\cref@variant}{@first}%
      \else%
        \expandafter\@setcref%
          \expandafter{\@beginref}{\cref@variant}{}%
      \fi%
    \else%
      \ifnum\count@consecutive=2\relax%
        \expandafter\@setcref%
          \expandafter{\@beginref}{\cref@variant}{@first}%
        \expandafter\cref@stack@push\expandafter%
          {\@endref,}{\@refsubstack}%
      \else%
        \edef\@tempa{{\@beginref}{\@endref}}%
        \if@cref@stackempty%
          \expandafter\@setcrefrange\@tempa{\cref@variant}{}%
        \else%
          \expandafter\@setcrefrange\@tempa{\cref@variant}{@first}%
        \fi%
      \fi%
    \fi%
    \@secondreftrue%
    \cref@isstackfull{\@refsubstack}%
    \@whilesw\if@cref@stackfull\fi{%
      \if@cref@compress%
        \cref@processconsecutive%
          {\@refsubstack}{\@beginref}{\@endref}{\count@consecutive}%
          {\cref@isrefconsecutive}%
      \else%
        \edef\@beginref{\cref@stack@top{\@refsubstack}}%
        \cref@stack@pop{\@refsubstack}%
        \@whilesw\ifx\@beginref\@empty\fi{%
          \cref@stack@pop{\@refsubstack}%
          \cref@isstackempty{\@refsubstack}%
          \if@cref@stackempty%
            \let\@beginref\relax%
          \else%
            \edef\@beginref{\cref@stack@top{\@refsubstack}}%
          \fi}%
        \let\@endref\relax%
        \count@consecutive=1\relax%
      \fi%
      \cref@isstackempty{\@refsubstack}%
      \if@cref@stackempty%
        \if@secondref%
          \def\@pos{@second}%
        \else%
          \def\@pos{@last}%
        \fi%
      \else%
        \def\@pos{@middle}%
      \fi%
      \ifnum\count@consecutive=1\relax%
        \edef\@tempa{{\@beginref}{cref}{\@pos}}%
        \expandafter\@setcref\@tempa%
      \else%
        \ifnum\count@consecutive=2\relax%
          \expandafter\@setcref\expandafter%
            {\@beginref}{cref}{@middle}%
          \expandafter\cref@stack@push\expandafter%
            {\@endref}{\@refsubstack}%
        \else%
          \edef\@tempa{{\@beginref}{\@endref}{cref}{\@pos}}%
          \expandafter\@setcrefrange\@tempa%
        \fi%
      \fi%
      \@secondreffalse%
      \cref@isstackfull{\@refsubstack}%
    }% end loop over reference substack
    \cref@isstackfull{\@refstack}%
    \if@cref@stackfull%
      \def\@tempa{#1}\def\@tempb{labelcref}%
      \ifx\@tempa\@tempb\relax%
        \protect\G@refundefinedtrue%
        \nfss@text{\reset@font\bfseries\space ??}%
        \@latex@warning{References in label reference on page \thepage
          \space have different types}%
        \@cref@stackfullfalse%
      \fi%
    \fi%
  }% end loop over main reference stack
  \endgroup}
\def\@setcref#1#2#3{%
  \expandafter\ifx\csname r@cref@#1\endcsname\relax%
    \protect\G@refundefinedtrue%
    \nfss@text{\reset@font\bfseries ??}%
    \@latex@warning{Reference `#1' on page \thepage \space undefined}%
  \else%
    \cref@gettype{#1}{\@temptype}%  puts label type in \@temptype
    \cref@getlabel{#1}{\@templabel}%  puts label in \@templabel
    \expandafter\ifx\csname #2@\@temptype @format#3\endcsname\relax%
      \edef\@tempa{#2}\def\@tempb{labelcref}%
      \ifx\@tempa\@tempb\relax%
        \expandafter\@@setcref\expandafter%
          {\csname #2@default@format#3\endcsname}{#1}%
      \else%
        \protect\G@refundefinedtrue%
        \nfss@text{\reset@font\bfseries ??}~\@templabel%
        \@latex@warning{#2 \space reference format for label type
          `\@temptype' undefined}%
      \fi%
    \else%
      \expandafter\@@setcref\expandafter%
        {\csname #2@\@temptype @format#3\endcsname}{#1}%
    \fi%
  \fi}
\def\@@setcref#1#2{\cref@getlabel{#2}{\@templabel}#1{\@templabel}{}{}}
\def\@setcrefrange#1#2#3#4{%
  \begingroup%
    \expandafter\ifx\csname r@cref@#1\endcsname\relax%
      \protect\G@refundefinedtrue%
      \@latex@warning{Reference `#1' on page \thepage \space%
        undefined}%
      \expandafter\ifx\csname r@cref@#2\endcsname\relax%
        \nfss@text{\reset@font\bfseries ??}--%
        \nfss@text{\reset@font\bfseries ??}%
        \@latex@warning{Reference `#2' on page \thepage \space%
          undefined}%
      \else%
        \cref@getlabel{#2}{\@labelb}%
        \nfss@text{\reset@font\bfseries ??}--\@labelb%
      \fi%
    \else%
      \expandafter\ifx\csname r@cref@#2\endcsname\relax%
        \protect\G@refundefinedtrue%
        \cref@getlabel{#1}{\@labela}%
        \@labela--\nfss@text{\reset@font\bfseries ??}%
        \@latex@warning{Reference `#2' on page \thepage %
          \space undefined}%
      \else%
        \cref@gettype{#1}{\@typea}%
        \cref@gettype{#2}{\@typeb}%
        \cref@getlabel{#1}{\@labela}%
        \cref@getlabel{#2}{\@labelb}%
        \edef\@formata{\expandafter\noexpand%
          \csname #3range@\@typea @format#4\endcsname}%
        \edef\@formatb{\expandafter\noexpand%
          \csname #3range@\@typeb @format#4\endcsname}%
        \expandafter\ifx\@formata\relax%
          \edef\@tempa{#3}\def\@tempb{labelcref}%
          \ifx\@tempa\@tempb\relax%
            \expandafter\@@setcrefrange\expandafter%
              {\csname #3range@default@format#4\endcsname}{#1}{#2}%
          \else%
            \protect\G@refundefinedtrue%
            \nfss@text{\reset@font\bfseries ??}~\@labela--\@labelb%
            \@latex@warning{#3\space reference range format for label
              type `\@typea' undefined}%
          \fi%
        \else%
          \ifx\@formata\@formatb%
            \expandafter\@@setcrefrange\expandafter{\@formata}{#1}{#2}%
          \else%
            \protect\G@refundefinedtrue%
            \nfss@text{\reset@font\bfseries ??}~\@labela--\@labelb%
            \@latex@warning{References `#1' and `#2' in reference range
              on page \thepage have different types}%
          \fi%
        \fi%
      \fi%
    \fi%
  \endgroup}
\def\@@setcrefrange#1#2#3{%
  \cref@getlabel{#2}{\@labela}%
  \cref@getlabel{#3}{\@labelb}%
  #1{\@labela}{\@labelb}{}{}{}{}}
\def\@setcref@pairgroupconjunction{\crefpairgroupconjunction}
\def\@setcref@middlegroupconjunction{\crefmiddlegroupconjunction}
\def\@setcref@lastgroupconjunction{\creflastgroupconjunction}
\DeclareRobustCommand{\labelcref}[1]{\@cref{labelcref}{#1}}
\DeclareRobustCommand{\namecref}[1]{%
  \@setnamecref{cref}{#1}{}{}}
\DeclareRobustCommand{\nameCref}[1]{%
  \@setnamecref{Cref}{#1}{}{}}
\DeclareRobustCommand{\lcnamecref}[1]{%
  \@setnamecref{Cref}{#1}{}{\MakeLowercase}}
\DeclareRobustCommand{\namecrefs}[1]{%
  \@setnamecref{cref}{#1}{@plural}{}}
\DeclareRobustCommand{\nameCrefs}[1]{%
  \@setnamecref{Cref}{#1}{@plural}{}}
\DeclareRobustCommand{\lcnamecrefs}[1]{%
  \@setnamecref{Cref}{#1}{@plural}{\MakeLowercase}}
\def\@setnamecref#1#2#3#4{%
  \expandafter\ifx\csname r@cref@#2\endcsname\relax%
    \protect\G@refundefinedtrue%
    \nfss@text{\reset@font\bfseries ??}%
    \@latex@warning{Reference `#1' on page \thepage \space undefined}%
  \else%
    \cref@gettype{#2}{\@tempa}%
    \@ifundefined{#1@\@tempa @name#3}{%
      \protect\G@refundefinedtrue%``
      \nfss@text{\reset@font\bfseries ??}%
      \@latex@warning{Reference name for
        label type `\@tempa' undefined}%
    }{%
      \edef\@tempa{%
        \expandafter\noexpand\csname #1@\@tempa @name#3\endcsname}%
      \expandafter\@@setnamecref\expandafter{\@tempa}{#4}%
    }%
  \fi}
\def\@@setnamecref#1#2{%
  \expandafter\def\expandafter\@tempa\expandafter{#1}%
  \expandafter#2\@tempa}
\DeclareRobustCommand{\cpageref}[1]{%
  \@cpageref{cref}{#1}{\@setcpageref}{\@setcpagerefrange}}
\DeclareRobustCommand{\Cpageref}[1]{%
  \@cpageref{Cref}{#1}{\@setcpageref}{\@setcpagerefrange}}
\DeclareRobustCommand{\cpagerefrange}[2]{%
  \@setcpagerefrange{#1}{#2}{cref}{}}
\DeclareRobustCommand{\Cpagerefrange}[2]{%
  \@setcpagerefrange{#1}{#2}{Cref}{}}
\DeclareRobustCommand{\labelcpageref}[1]{%
  \@cpageref{labelcref}{#1}{\@setcpageref}{\@setcpagerefrange}}
\def\@cpageref#1#2#3#4{%
  \leavevmode%
  \begingroup%
  \countdef\count@consecutive=0%
  \countdef\count@group=1%
  \countdef\@counta=2%
  \countdef\@countb=3%
  \count@group=0%
  \cref@stack@init{\@refstack}%
  \edef\@tempa{#2}%
  \expandafter\cref@stack@push\expandafter{\@tempa}{\@refstack}%
  \if@cref@sort%
    \cref@stack@sort{\@refstack}{\cref@pagecmp}%
  \fi%
  \cref@isstackfull{\@refstack}%
  \@whilesw\if@cref@stackfull\fi{%
    \if@cref@compress%
      \cref@processconsecutive%
        {\@refstack}{\@beginref}{\@endref}{\count@consecutive}%
        {\cref@ispagerefconsecutive}%
    \else%
      \edef\@beginref{\cref@stack@top{\@refstack}}%
      \cref@stack@pop{\@refstack}%
      \@whilesw\ifx\@beginref\@empty\fi{%
        \cref@stack@pop{\@refstack}%
        \cref@isstackempty{\@refstack}%
        \if@cref@stackempty%
          \let\@beginref\relax%
        \else%
          \edef\@beginref{\cref@stack@top{\@refstack}}%
        \fi}%
      \let\@endref\relax%
      \count@consecutive=1\relax%
    \fi%
    \ifx\@endref\relax\else%
      \expandafter\ifx\csname r@cref@\@beginref\endcsname\relax\else%
        \expandafter\ifx\csname r@cref@\@endref\endcsname\relax\else%
          \cref@getpageref{\@beginref}{\@tempa}%
          \cref@getpageref{\@endref}{\@tempb}%
          \ifx\@tempa\@tempb\relax%
            \count@consecutive=1%
            \let\@endref\relax%
          \else%
            \@counta=\@tempa\relax%
            \@countb=\@tempb\relax%
            \advance\@counta 1\relax%
            \ifnum\@counta=\@countb\relax%
              \count@consecutive=2%
            \fi%
          \fi%
        \fi%
      \fi%
    \fi%
    \cref@isstackempty{\@refstack}%
    \if@cref@stackempty%
      \ifcase\count@group\relax%
        \ifnum\count@consecutive=2\relax%
          \def\@pos{@first}%
        \else%
          \def\@pos{}%
        \fi%
      \or%
        \ifnum\count@consecutive=2\relax%
          \def\@pos{@middle}%
        \else%
          \def\@pos{@second}%
        \fi%
      \else%
        \def\@pos{@last}%
      \fi%
    \else%
      \ifnum\count@group=0\relax%
        \def\@pos{@first}%
      \else%
        \def\@pos{@middle}%
      \fi%
    \fi%
    \ifnum\count@consecutive=1\relax%
      \def\@tempa{#3}%
      \edef\@tempb{{\@beginref}{#1}{\@pos}}%
      \expandafter\@tempa\@tempb%
    \else%
      \ifnum\count@consecutive=2\relax%
        \def\@tempa{#3}%
        \edef\@tempb{{\@beginref}{#1}{\@pos}}%
        \expandafter\@tempa\@tempb%
        \expandafter\cref@stack@push\expandafter%
          {\@endref,}{\@refstack}%
      \else%
        \def\@tempa{#4}%
        \edef\@tempb{{\@beginref}{\@endref}{#1}{\@pos}}%
        \expandafter\@tempa\@tempb%
      \fi%
    \fi%
    \advance\count@group 1%
    \cref@isstackfull{\@refstack}%
  }% end loop over reference stack
  \endgroup}
\def\@setcpageref#1#2#3{%
  \expandafter\ifx\csname r@cref@#1\endcsname\relax%
    \protect\G@refundefinedtrue%
    \nfss@text{\reset@font\bfseries ??}%
    \@latex@warning{Reference `#1' on page \thepage \space undefined}%
  \else%
    \cref@getpageref{#1}{\@temppage}%
    \expandafter\ifx\csname #2@page@format#3\endcsname\relax%
      \edef\@tempa{#2}\def\@tempb{labelcref}%
      \ifx\@tempa\@tempb\relax%
        \expandafter\@@setcpageref\expandafter%
          {\csname #2@default@format#3\endcsname}{#1}%
      \else%
        \protect\G@refundefinedtrue%
        \nfss@text{\reset@font\bfseries ??}~\@temppage%
        \@latex@warning{#2 \space reference format for
          page references undefined}%
      \fi%
    \else%
      \expandafter\@@setcpageref\expandafter%
        {\csname #2@page@format#3\endcsname}{#1}%
    \fi%
  \fi}
\def\@@setcpageref#1#2{%
  \cref@getpageref{#2}{\@temppage}#1{\@temppage}{}{}}
\def\@setcpagerefrange#1#2#3#4{%
  \begingroup%
    \expandafter\ifx\csname r@cref@#1\endcsname\relax%
      \protect\G@refundefinedtrue%
      \@latex@warning{Reference `#1' on page \thepage \space%
        undefined}%
      \expandafter\ifx\csname r@cref@#2\endcsname\relax%
        \nfss@text{\reset@font\bfseries ??}--%
        \nfss@text{\reset@font\bfseries ??}%
        \@latex@warning{Reference `#2' on page \thepage \space%
          undefined}%
      \else%
        \cref@getpageref{#2}{\@pageb}%
        \nfss@text{\reset@font\bfseries ??}--\@pageb%
      \fi%
    \else%
      \expandafter\ifx\csname r@cref@#2\endcsname\relax%
        \protect\G@refundefinedtrue%
        \cref@getpageref{#1}{\@pagea}%
        \@pagea--\nfss@text{\reset@font\bfseries ??}%
        \@latex@warning{Reference `#2' on page \thepage %
          \space undefined}%
      \else%
        \cref@getpageref{#1}{\@pagea}%
        \cref@getpageref{#2}{\@pageb}%
        \edef\@format{\expandafter\noexpand%
          \csname #3range@page@format#4\endcsname}%
        \expandafter\ifx\@format\relax%
          \edef\@tempa{#3}\def\@tempb{labelcref}%
          \ifx\@tempa\@tempb\relax%
            \expandafter\@@setcpagerefrange\expandafter%
              {\csname #3range@default@format#4\endcsname}{#1}{#2}%
          \else%
            \protect\G@refundefinedtrue%
            \nfss@text{\reset@font\bfseries ??}~\@pagea--\@pageb%
            \@latex@warning{#3\space reference range format for page
              references undefined}%
          \fi%
        \else%
          \expandafter\@@setcpagerefrange\expandafter{\@format}{#1}{#2}%
        \fi%
      \fi%
    \fi%
  \endgroup}
\def\@@setcpagerefrange#1#2#3{%
  \cref@getpageref{#2}{\@pagea}%
  \cref@getpageref{#3}{\@pageb}%
  #1{\@pagea}{\@pageb}{}{}{}{}}
\cref@stack@init{\cref@label@types}
\newcommand{\crefdefaultlabelformat}[1]{%
  \def\cref@default@label##1##2##3{#1}}
\newcommand{\crefname}[3]{%
  \@crefname{cref}{#1}{#2}{#3}{}}
\newcommand{\Crefname}[3]{%
  \@crefname{Cref}{#1}{#2}{#3}{}}
\newcommand{\creflabelformat}[2]{%
  \expandafter\def\csname cref@#1@label\endcsname##1##2##3{#2}%
  \cref@stack@add{#1}{\cref@label@types}}
\newcommand{\crefrangelabelformat}[2]{%
  \expandafter\def\csname cref@#1@rangelabel\endcsname%
    ##1##2##3##4##5##6{#2}%
  \cref@stack@add{#1}{\cref@label@types}}
\newcommand{\crefalias}[2]{%
  \expandafter\def\csname cref@#1@alias\endcsname{#2}}
\newcommand{\crefname@preamble}[3]{%
  \@crefname{cref}{#1}{#2}{#3}{@preamble}}
\newcommand{\Crefname@preamble}[3]{%
  \@crefname{Cref}{#1}{#2}{#3}{@preamble}}
\def\cref@othervariant#1#2#3{\cref@@othervariant#1\@nil#2#3}
\def\cref@@othervariant#1#2\@nil#3#4{%
  \if#1c%
    \def#3{C#2}%
    \def#4{\MakeUppercase}%
  \else%
    \def#3{c#2}%
    \if@cref@capitalise%
      \def#4{}%
    \else%
      \def#4{\MakeLowercase}%
    \fi%
  \fi}
\def\@crefname#1#2#3#4#5{%
  \expandafter\def\csname #1@#2@name#5\endcsname{#3}%
  \expandafter\def\csname #1@#2@name@plural#5\endcsname{#4}%
  \cref@othervariant{#1}{\@tempc}{\@tempd}%
  \@ifundefined{\@tempc @#2@name#5}{%
    \expandafter\expandafter\expandafter\def%
    \expandafter\expandafter\expandafter\@tempa%
    \expandafter\expandafter\expandafter{%
      \csname#1@#2@name\endcsname}%
    \expandafter\expandafter\expandafter\def%
    \expandafter\expandafter\expandafter\@tempb%
    \expandafter\expandafter\expandafter{%
      \csname#1@#2@name@plural\endcsname}%
    \expandafter\ifx\@tempa\@empty\else%
      \expandafter\expandafter\expandafter\def%
      \expandafter\expandafter\expandafter\@tempa%
      \expandafter\expandafter\expandafter{%
        \expandafter\@tempd\@tempa}%
      \expandafter\expandafter\expandafter\def%
      \expandafter\expandafter\expandafter\@tempb%
      \expandafter\expandafter\expandafter{%
        \expandafter\@tempd\@tempb}%
    \fi%
    \toksdef\@toksa=0%
    \@toksa={%
      \expandafter\def\csname\@tempc @#2@name#5\endcsname}%
    \expandafter\the\expandafter\@toksa\expandafter{\@tempa}%
    \@toksa={%
      \expandafter\def\csname\@tempc @#2@name@plural#5\endcsname}%
    \expandafter\the\expandafter\@toksa\expandafter{\@tempb}%
  }{}%
  \cref@stack@add{#2}{\cref@label@types}}
\def\@crefconstructcomponents#1{%
  \@ifundefined{cref@#1@label}{%
    \let\@templabel\cref@default@label%
  }{%
    \expandafter\let\expandafter\@templabel%
    \csname cref@#1@label\endcsname%
  }%
  \@ifundefined{cref@#1@rangelabel}{%
    \expandafter\def\expandafter\@tempa\expandafter{%
      \@templabel{####1}{####3}{####4}}%
    \expandafter\def\expandafter\@tempb\expandafter{%
      \@templabel{####2}{####5}{####6}}%
    \toksdef\@toksa=0%
    \@toksa={\def\@temprangelabel##1##2##3##4##5##6}%
    \expandafter\expandafter\expandafter\the%
    \expandafter\expandafter\expandafter\@toksa%
    \expandafter\expandafter\expandafter{%
      \expandafter\expandafter\expandafter\crefrangepreconjunction%
      \expandafter\@tempa\expandafter\crefrangeconjunction\@tempb%
      \crefrangepostconjunction}%
  }{%
    \expandafter\let\expandafter\@temprangelabel%
    \csname cref@#1@rangelabel\endcsname%
  }%
  \if@cref@nameinlink%
    \expandafter\def\expandafter\@templabel@first\expandafter{%
      \@templabel{########1}{}{########3}}%
    \expandafter\def\expandafter\@temprangelabel@first\expandafter{%
      \@temprangelabel{########1}{########2}%
        {}{########4}{########5}{########6}}%
  \fi%
  \expandafter\def\expandafter\@templabel\expandafter{%
    \@templabel{########1}{########2}{########3}}%
  \expandafter\def\expandafter\@temprangelabel\expandafter{%
    \@temprangelabel{########1}{########2}{########3}%
    {########4}{########5}{########6}}%
  \if@cref@nameinlink\else%
    \let\@templabel@first\@templabel%
    \let\@temprangelabel@first\@temprangelabel%
  \fi%
  \if@cref@nameinlink%
    \def\@tempa##1##2{##2##1}%
    \expandafter\expandafter\expandafter\def%
    \expandafter\expandafter\expandafter\@tempname%
    \expandafter\expandafter\expandafter{%
      \expandafter\@tempa\expandafter%
        {\csname cref@#1@name\endcsname}{########2}}%
    \expandafter\expandafter\expandafter\def%
    \expandafter\expandafter\expandafter\@tempName%
    \expandafter\expandafter\expandafter{%
      \expandafter\@tempa\expandafter%
        {\csname Cref@#1@name\endcsname}{########2}}%
    \expandafter\expandafter\expandafter\def%
    \expandafter\expandafter\expandafter\@tempnameplural%
    \expandafter\expandafter\expandafter{%
      \expandafter\@tempa\expandafter%
        {\csname cref@#1@name@plural\endcsname}{########2}}%
    \expandafter\expandafter\expandafter\def%
    \expandafter\expandafter\expandafter\@tempNameplural%
    \expandafter\expandafter\expandafter{%
      \expandafter\@tempa\expandafter%
        {\csname Cref@#1@name@plural\endcsname}{########2}}%
    \expandafter\expandafter\expandafter\def%
    \expandafter\expandafter\expandafter\@tempnameplural@range%
    \expandafter\expandafter\expandafter{%
      \expandafter\@tempa\expandafter%
        {\csname cref@#1@name@plural\endcsname}{########3}}%
    \expandafter\expandafter\expandafter\def%
    \expandafter\expandafter\expandafter\@tempNameplural@range%
    \expandafter\expandafter\expandafter{%
      \expandafter\@tempa\expandafter%
        {\csname Cref@#1@name@plural\endcsname}{########3}}%
  \else%
    \expandafter\def\expandafter\@tempname\expandafter{%
      \csname cref@#1@name\endcsname}%
    \expandafter\def\expandafter\@tempName\expandafter{%
      \csname Cref@#1@name\endcsname}%
    \expandafter\def\expandafter\@tempnameplural\expandafter{%
      \csname cref@#1@name@plural\endcsname}%
    \expandafter\def\expandafter\@tempNameplural\expandafter{%
      \csname Cref@#1@name@plural\endcsname}%
    \let\@tempnameplural@range\@tempnameplural%
    \let\@tempNameplural@range\@tempNameplural%
  \fi%
}
\def\@crefdefineformat#1{%
  \begingroup%
    \@crefconstructcomponents{#1}%
    \ifx\@tempname\@empty\relax%
      \expandafter\def\expandafter\@tempfirst\expandafter{\@templabel}%
    \else%
      \expandafter\expandafter\expandafter\def%
      \expandafter\expandafter\expandafter\@tempfirst%
      \expandafter\expandafter\expandafter{%
        \expandafter\@tempname\expandafter\nobreakspace\@templabel@first}%
    \fi%
    \ifx\@tempName\@empty\relax%
      \expandafter\def\expandafter\@tempFirst\expandafter{\@templabel}%
    \else%
      \expandafter\expandafter\expandafter\def%
      \expandafter\expandafter\expandafter\@tempFirst%
      \expandafter\expandafter\expandafter{%
        \expandafter\@tempName\expandafter\nobreakspace\@templabel@first}%
    \fi%
    \expandafter\def\expandafter\@templabel\expandafter{\@templabel}%
    \toksdef\@toksa=0%
    \@toksa={\crefformat{#1}}%
    \expandafter\the\expandafter\@toksa\expandafter{\@tempfirst}%
    \@toksa={\Crefformat{#1}}%
    \expandafter\the\expandafter\@toksa\expandafter{\@tempFirst}%
    \@ifundefined{cref@#1@label}{}{%
      \@toksa={\labelcrefformat{#1}}%
      \expandafter\the\expandafter\@toksa\expandafter{\@templabel}}%
  \endgroup}
\def\@crefrangedefineformat#1{%
  \begingroup%
    \@crefconstructcomponents{#1}%
    \ifx\@tempname\@empty\relax%
      \expandafter\def\expandafter\@tempfirst%
        \expandafter{\@temprangelabel}%
    \else%
      \expandafter\expandafter\expandafter\def%
      \expandafter\expandafter\expandafter\@tempfirst%
      \expandafter\expandafter\expandafter{%
        \expandafter\@tempnameplural@range%
        \expandafter\nobreakspace\@temprangelabel@first}%
    \fi%
    \ifx\@tempName\@empty\relax%
      \expandafter\def\expandafter\@tempFirst%
        \expandafter{\@temprangelabel}%
    \else%
      \expandafter\expandafter\expandafter\def%
      \expandafter\expandafter\expandafter\@tempFirst%
      \expandafter\expandafter\expandafter{%
        \expandafter\@tempNameplural@range%
        \expandafter\nobreakspace\@temprangelabel@first}%
    \fi%
    \expandafter\def\expandafter\@temprangelabel%
      \expandafter{\@temprangelabel}%
    \toksdef\@toksa=0%
    \@toksa={\crefrangeformat{#1}}%
    \expandafter\the\expandafter\@toksa\expandafter{\@tempfirst}%
    \@toksa={\Crefrangeformat{#1}}%
    \expandafter\the\expandafter\@toksa\expandafter{\@tempFirst}%
    \@ifundefined{cref@#1@rangelabel}{%
      \@ifundefined{cref@#1@label}{\let\@tempa\relax}{\def\@tempa{}}}%
      {\def\@tempa{}}%
    \ifx\@tempa\@empty\relax%
      \@toksa={\labelcrefrangeformat{#1}}%
      \expandafter\the\expandafter\@toksa\expandafter{%
        \@temprangelabel}%
    \fi%
  \endgroup}
\def\@crefdefinemultiformat#1{%
  \begingroup%
    \@crefconstructcomponents{#1}%
    \ifx\@tempnameplural\@empty\relax%
      \expandafter\def\expandafter\@tempfirst%
        \expandafter{\@templabel}%
    \else%
      \expandafter\expandafter\expandafter\def%
      \expandafter\expandafter\expandafter\@tempfirst%
      \expandafter\expandafter\expandafter{%
        \expandafter\@tempnameplural%
        \expandafter\nobreakspace\@templabel@first}%
    \fi%
    \ifx\@tempNameplural\@empty\relax%
      \expandafter\def\expandafter\@tempFirst%
        \expandafter{\@templabel}%
    \else%
      \expandafter\expandafter\expandafter\def%
      \expandafter\expandafter\expandafter\@tempFirst%
      \expandafter\expandafter\expandafter{%
        \expandafter\@tempNameplural%
        \expandafter\nobreakspace\@templabel@first}%
    \fi%
    \expandafter\def\expandafter\@tempsecond\expandafter{%
      \expandafter\crefpairconjunction\@templabel}%
    \expandafter\def\expandafter\@tempmiddle\expandafter{%
      \expandafter\crefmiddleconjunction\@templabel}%
    \expandafter\def\expandafter\@templast\expandafter{%
      \expandafter\creflastconjunction\@templabel}%
    \expandafter\def\expandafter\@templabel\expandafter{\@templabel}%
    \toksdef\@toksa=0%
    \toksdef\@toksb=1%
    \@toksb={}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@tempfirst}}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@tempsecond}}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@tempmiddle}}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@templast}}%
    \@toksa={\crefmultiformat{#1}}%
    \expandafter\the\expandafter\@toksa\the\@toksb%
    \@toksb={}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@tempFirst}}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@tempsecond}}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@tempmiddle}}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@templast}}%
    \@toksa={\Crefmultiformat{#1}}%
    \expandafter\the\expandafter\@toksa\the\@toksb%
    \@ifundefined{cref@#1@label}{}{%
      \@toksb={}%
      \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
        \expandafter{\@templabel}}%
      \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
        \expandafter{\@tempsecond}}%
      \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
        \expandafter{\@tempmiddle}}%
      \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
        \expandafter{\@templast}}%
      \@toksa={\labelcrefmultiformat{#1}}%
      \expandafter\the\expandafter\@toksa\the\@toksb}%
  \endgroup}
\def\@crefrangedefinemultiformat#1{%
  \begingroup%
    \@crefconstructcomponents{#1}%
    \ifx\@tempnameplural\@empty\relax%
      \expandafter\def\expandafter\@tempfirst%
        \expandafter{\@temprangelabel}%
    \else%
      \expandafter\expandafter\expandafter\def%
      \expandafter\expandafter\expandafter\@tempfirst%
      \expandafter\expandafter\expandafter{%
        \expandafter\@tempnameplural@range%
        \expandafter\nobreakspace\@temprangelabel@first}%
    \fi%
    \ifx\@tempNameplural\@empty\relax%
      \expandafter\def\expandafter\@tempFirst%
        \expandafter{\@temprangelabel}%
    \else%
      \expandafter\expandafter\expandafter\def%
      \expandafter\expandafter\expandafter\@tempFirst%
      \expandafter\expandafter\expandafter{%
        \expandafter\@tempNameplural@range%
        \expandafter\nobreakspace\@temprangelabel@first}%
    \fi%
    \expandafter\def\expandafter\@tempsecond\expandafter{%
      \expandafter\crefpairconjunction\@temprangelabel}%
    \expandafter\def\expandafter\@tempmiddle\expandafter{%
      \expandafter\crefmiddleconjunction\@temprangelabel}%
    \expandafter\def\expandafter\@templast\expandafter{%
      \expandafter\creflastconjunction\@temprangelabel}%
    \expandafter\def\expandafter\@temprangelabel%
      \expandafter{\@temprangelabel}%
    \toksdef\@toksa=0%
    \toksdef\@toksb=1%
    \@toksb={}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@tempfirst}}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@tempsecond}}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@tempmiddle}}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@templast}}%
    \@toksa={\crefrangemultiformat{#1}}%
    \expandafter\the\expandafter\@toksa\the\@toksb%
    \@toksb={}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@tempFirst}}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@tempsecond}}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@tempmiddle}}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@templast}}%
    \@toksa={\Crefrangemultiformat{#1}}%
    \expandafter\the\expandafter\@toksa\the\@toksb%
    \@ifundefined{cref@#1@rangelabel}{%
      \@ifundefined{cref@#1@label}{\let\@tempa\relax}{\def\@tempa{}}}%
        {\def\@tempa{}}%
    \ifx\@tempa\@empty\relax%
      \@toksb={}%
      \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
        \expandafter{\@temprangelabel}}%
      \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
        \expandafter{\@tempsecond}}%
      \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
        \expandafter{\@tempmiddle}}%
      \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
        \expandafter{\@templast}}%
      \@toksa={\labelcrefrangemultiformat{#1}}%
      \expandafter\the\expandafter\@toksa\the\@toksb%
    \fi%
  \endgroup}
\def\@labelcrefdefinedefaultformats{%
  \begingroup%
    \toksdef\@toksa=0%
    \toksdef\@toksb=1%
    \let\@templabel\cref@default@label%
    \expandafter\def\expandafter\@tempa\expandafter{%
      \@templabel{####1}{####3}{####4}}%
    \expandafter\def\expandafter\@tempb\expandafter{%
      \@templabel{####2}{####5}{####6}}%
    \@toksa={\def\@temprangelabel##1##2##3##4##5##6}%
    \expandafter\expandafter\expandafter\the%
    \expandafter\expandafter\expandafter\@toksa%
    \expandafter\expandafter\expandafter{%
      \expandafter\expandafter\expandafter\crefrangepreconjunction%
      \expandafter\@tempa\expandafter\crefrangeconjunction\@tempb%
      \crefrangepostconjunction}%
    \expandafter\def\expandafter\@templabel\expandafter{%
      \@templabel{########1}{########2}{########3}}%
    \expandafter\def\expandafter\@temprangelabel\expandafter{%
      \@temprangelabel{########1}{########2}{########3}%
      {########4}{########5}{########6}}%
    \expandafter\def\expandafter\@tempsecond\expandafter{%
      \expandafter\crefpairconjunction\@templabel}%
    \expandafter\def\expandafter\@tempmiddle\expandafter{%
      \expandafter\crefmiddleconjunction\@templabel}%
    \expandafter\def\expandafter\@templast\expandafter{%
      \expandafter\creflastconjunction\@templabel}%
    \expandafter\def\expandafter\@temprangesecond\expandafter{%
      \expandafter\crefpairconjunction\@temprangelabel}%
    \expandafter\def\expandafter\@temprangemiddle\expandafter{%
      \expandafter\crefmiddleconjunction\@temprangelabel}%
    \expandafter\def\expandafter\@temprangelast\expandafter{%
      \expandafter\creflastconjunction\@temprangelabel}%
    \expandafter\def\expandafter\@templabel\expandafter{\@templabel}%
    \expandafter\def\expandafter\@temprangelabel%
      \expandafter{\@temprangelabel}%
    \@toksa={\labelcrefformat{default}}%
    \expandafter\the\expandafter\@toksa\expandafter{\@templabel}%
    \@toksa={\labelcrefrangeformat{default}}%
    \expandafter\the\expandafter\@toksa\expandafter{\@temprangelabel}%
    \@toksb={}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@templabel}}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@tempsecond}}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@tempmiddle}}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@templast}}%
    \@toksa={\labelcrefmultiformat{default}}%
    \expandafter\the\expandafter\@toksa\the\@toksb%
    \@toksb={}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@temprangelabel}}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@temprangesecond}}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@temprangemiddle}}%
    \expandafter\cref@append@toks\expandafter\@toksb\expandafter{%
      \expandafter{\@temprangelast}}%
    \@toksa={\labelcrefrangemultiformat{default}}%
    \expandafter\the\expandafter\@toksa\the\@toksb%
  \endgroup}
\def\@crefdefineallformats#1{%
  \@crefdefineformat{#1}%
  \@crefrangedefineformat{#1}%
  \@crefdefinemultiformat{#1}%
  \@crefrangedefinemultiformat{#1}}
\newcommand{\crefformat}[2]{\@crefformat{cref}{#1}{#2}}
\newcommand{\Crefformat}[2]{\@crefformat{Cref}{#1}{#2}}
\newcommand{\crefrangeformat}[2]{\@crefrangeformat{crefrange}{#1}{#2}}
\newcommand{\Crefrangeformat}[2]{\@crefrangeformat{Crefrange}{#1}{#2}}
\newcommand{\crefmultiformat}[5]{%
  \@crefmultiformat{cref}{#1}{#2}{#3}{#4}{#5}}
\newcommand{\Crefmultiformat}[5]{%
  \@crefmultiformat{Cref}{#1}{#2}{#3}{#4}{#5}}
\newcommand{\crefrangemultiformat}[5]{%
  \@crefrangemultiformat{crefrange}{#1}{#2}{#3}{#4}{#5}}
\newcommand{\Crefrangemultiformat}[5]{%
  \@crefrangemultiformat{Crefrange}{#1}{#2}{#3}{#4}{#5}}
\newcommand{\labelcrefformat}[2]{%
  \expandafter\gdef\csname labelcref@#1@format\endcsname##1##2##3{#2}}
\newcommand{\labelcrefrangeformat}[2]{%
  \expandafter\gdef\csname labelcrefrange@#1@format\endcsname%
  ##1##2##3##4##5##6{#2}}
\newcommand{\labelcrefmultiformat}[5]{%
  \expandafter\gdef\csname labelcref@#1@format@first\endcsname%
    ##1##2##3{#2}%
  \expandafter\gdef\csname labelcref@#1@format@second\endcsname%
    ##1##2##3{#3}%
  \expandafter\gdef\csname labelcref@#1@format@middle\endcsname%
    ##1##2##3{#4}%
  \expandafter\gdef\csname labelcref@#1@format@last\endcsname%
    ##1##2##3{#5}}
\newcommand{\labelcrefrangemultiformat}[5]{%
  \expandafter\gdef\csname labelcrefrange@#1@format@first\endcsname%
    ##1##2##3##4##5##6{#2}%
  \expandafter\gdef\csname labelcrefrange@#1@format@second\endcsname%
    ##1##2##3##4##5##6{#3}%
  \expandafter\gdef\csname labelcrefrange@#1@format@middle\endcsname%
    ##1##2##3##4##5##6{#4}%
  \expandafter\gdef\csname labelcrefrange@#1@format@last\endcsname%
    ##1##2##3##4##5##6{#5}}
\def\@crefformat#1#2#3{%
  \begingroup%
    \expandafter\gdef\csname #1@#2@format\endcsname##1##2##3{#3}%
    \cref@othervariant{#1}{\@other}{\@changecase}%
    \@ifundefined{\@other @#2@format}{%
      \toksdef\@toksa=0%
      \@toksa={\def\@tempa##1##2##3}%
      \expandafter\expandafter\expandafter\the%
      \expandafter\expandafter\expandafter\@toksa%
      \expandafter\expandafter\expandafter{%
        \csname#1@#2@format\endcsname{##1}{##2}{##3}}%
      \expandafter\expandafter\expandafter\the%
      \expandafter\expandafter\expandafter\@toksa%
      \expandafter\expandafter\expandafter{%
        \expandafter\@changecase\@tempa{##1}{##2}{##3}}%
      \@toksa={%
        \expandafter\gdef\csname\@other @#2@format\endcsname##1##2##3}%
      \expandafter\the\expandafter\@toksa\expandafter{%
        \@tempa{##1}{##2}{##3}}%
    }{}%
  \endgroup}
\def\@crefrangeformat#1#2#3{%
  \begingroup%
    \expandafter\gdef\csname #1@#2@format\endcsname%
      ##1##2##3##4##5##6{#3}%
    \cref@othervariant{#1}{\@other}{\@changecase}%
    \@ifundefined{\@other @#2@format}{%
      \toksdef\@toksa=0%
      \@toksa={\def\@tempa##1##2##3##4##5##6}%
      \expandafter\expandafter\expandafter\the%
      \expandafter\expandafter\expandafter\@toksa%
      \expandafter\expandafter\expandafter{%
        \csname#1@#2@format\endcsname{##1}{##2}{##3}{##4}{##5}{##6}}%
      \expandafter\expandafter\expandafter\the%
      \expandafter\expandafter\expandafter\@toksa%
      \expandafter\expandafter\expandafter{%
        \expandafter\@changecase\@tempa{##1}{##2}{##3}{##4}{##5}{##6}}%
      \@toksa={\expandafter\gdef%
        \csname\@other @#2@format\endcsname##1##2##3##4##5##6}%
      \expandafter\the\expandafter\@toksa\expandafter{%
        \@tempa{##1}{##2}{##3}{##4}{##5}{##6}}%
    }{}%
  \endgroup}
\def\@crefmultiformat#1#2#3#4#5#6{%
  \begingroup%
    \expandafter\gdef\csname #1@#2@format@first\endcsname##1##2##3{#3}%
    \expandafter\gdef\csname #1@#2@format@second\endcsname##1##2##3{#4}%
    \expandafter\gdef\csname #1@#2@format@middle\endcsname##1##2##3{#5}%
    \expandafter\gdef\csname #1@#2@format@last\endcsname##1##2##3{#6}%
    \cref@othervariant{#1}{\@other}{\@changecase}%
    \@ifundefined{\@other @#2@format@first}{%
      \toksdef\@toksa=0%
      \@toksa={\def\@tempa##1##2##3}%
      \expandafter\expandafter\expandafter\the%
      \expandafter\expandafter\expandafter\@toksa%
      \expandafter\expandafter\expandafter{%
        \csname#1@#2@format@first\endcsname{##1}{##2}{##3}}%
      \expandafter\expandafter\expandafter\the%
      \expandafter\expandafter\expandafter\@toksa%
      \expandafter\expandafter\expandafter{%
        \expandafter\@changecase\@tempa{##1}{##2}{##3}}%
      \@toksa={%
        \expandafter\gdef\csname\@other @#2@format@first\endcsname%
          ##1##2##3}%
      \expandafter\the\expandafter\@toksa\expandafter{%
        \@tempa{##1}{##2}{##3}}%
    }{}%
    \@ifundefined{\@other @#2@format@second}{%
      \@toksa={%
        \expandafter\global\expandafter\let%
        \csname\@other @#2@format@second\endcsname}%
      \expandafter\the\expandafter\@toksa%
        \csname #1@#2@format@second\endcsname%
    }{}%
    \@ifundefined{\@other @#2@format@middle}{%
      \@toksa={%
        \expandafter\global\expandafter\let%
        \csname\@other @#2@format@middle\endcsname}%
      \expandafter\the\expandafter\@toksa%
        \csname #1@#2@format@middle\endcsname%
    }{}%
    \@ifundefined{\@other @#2@format@last}{%
      \@toksa={%
        \expandafter\global\expandafter\let%
        \csname\@other @#2@format@last\endcsname}%
      \expandafter\the\expandafter\@toksa%
        \csname #1@#2@format@last\endcsname%
    }{}%
  \endgroup}
\def\@crefrangemultiformat#1#2#3#4#5#6{%
  \begingroup%
    \expandafter\gdef\csname #1@#2@format@first\endcsname%
      ##1##2##3##4##5##6{#3}%
    \expandafter\gdef\csname #1@#2@format@second\endcsname%
      ##1##2##3##4##5##6{#4}%
    \expandafter\gdef\csname #1@#2@format@middle\endcsname%
      ##1##2##3##4##5##6{#5}%
    \expandafter\gdef\csname #1@#2@format@last\endcsname%
      ##1##2##3##4##5##6{#6}%
    \cref@othervariant{#1}{\@other}{\@changecase}%
    \@ifundefined{\@other @#2@format@first}{%
      \toksdef\@toksa=0%
      \@toksa={\def\@tempa##1##2##3##4##5##6}%
      \expandafter\expandafter\expandafter\the%
      \expandafter\expandafter\expandafter\@toksa%
      \expandafter\expandafter\expandafter{%
        \csname#1@#2@format@first\endcsname%
          {##1}{##2}{##3}{##4}{##5}{##6}}%
      \expandafter\expandafter\expandafter\the%
      \expandafter\expandafter\expandafter\@toksa%
      \expandafter\expandafter\expandafter{%
        \expandafter\@changecase\@tempa{##1}{##2}{##3}{##4}{##5}{##6}}%
      \@toksa={%
        \expandafter\gdef\csname\@other @#2@format@first\endcsname%
          ##1##2##3##4##5##6}%
      \expandafter\the\expandafter\@toksa\expandafter{%
        \@tempa{##1}{##2}{##3}{##4}{##5}{##6}}%
    }{}%
    \@ifundefined{\@other @#2@format@second}{%
      \@toksa={%
        \expandafter\global\expandafter\let%
        \csname\@other @#2@format@second\endcsname}%
      \expandafter\the\expandafter\@toksa%
        \csname #1@#2@format@second\endcsname%
    }{}%
    \@ifundefined{\@other @#2@format@middle}{%
      \@toksa={%
        \expandafter\global\expandafter\let%
        \csname\@other @#2@format@middle\endcsname}%
      \expandafter\the\expandafter\@toksa%
        \csname #1@#2@format@middle\endcsname%
    }{}%
    \@ifundefined{\@other @#2@format@last}{%
      \@toksa={%
        \expandafter\global\expandafter\let%
        \csname\@other @#2@format@last\endcsname}%
      \expandafter\the\expandafter\@toksa%
        \csname #1@#2@format@last\endcsname%
    }{}%
  \endgroup}
\let\if@cref@hyperrefloaded\iffalse
\@ifpackageloaded{hyperref}{%
  \@ifpackagewith{hyperref}{implicit=false}{}{%
    \let\if@cref@hyperrefloaded\iftrue%
    \PackageInfo{cleveref}{`hyperref' support loaded}
    \def\cref@hyperref#1{\expandafter\expandafter\expandafter%
      \@fourthoffive\csname r@#1\endcsname}
    \let\cref@old@H@refstepcounter\H@refstepcounter
    \def\H@refstepcounter#1{%
      \cref@old@H@refstepcounter{#1}%
      \cref@constructprefix{#1}{\cref@result}%
      \@ifundefined{cref@#1@alias}%
        {\def\@tempa{#1}}%
        {\def\@tempa{\csname cref@#1@alias\endcsname}}%
      \protected@xdef\cref@currentlabel{%
        [\@tempa][\arabic{#1}][\cref@result]%
        \csname p@#1\endcsname\csname the#1\endcsname}}
    \let\refstepcounter@noarg\cref@old@refstepcounter%
    \def\refstepcounter@optarg[#1]#2{%
      \cref@old@refstepcounter{#2}%
      \protected@xdef\cref@currentlabel{%
        \expandafter\cref@override@label@type%
          \cref@currentlabel\@nil{#1}}}
    \@ifundefined{appendix}{}{%
      \renewcommand\appendix{%
        \cref@old@appendix%
        \@ifundefined{chapter}{%
          \def\H@refstepcounter##1{%
            \cref@old@H@refstepcounter{##1}%
            \cref@constructprefix{##1}{\cref@result}%
            \ifx\cref@result\@empty%
              \def\cref@result{2147483647}%
            \else%
              \edef\cref@result{2147483647,\cref@result}%
            \fi%
            \def\@tempa{##1}%
            \def\@tempb{section}%
            \ifx\@tempa\@tempb%
              \protected@xdef\cref@currentlabel{%
                [appendix][\arabic{##1}][\cref@result]%
                \csname p@##1\endcsname\csname the##1\endcsname}%
            \else%
              \def\@tempa{##1}%
              \def\@tempb{subsection}%
              \ifx\@tempa\@tempb%
                \protected@xdef\cref@currentlabel{%
                  [subappendix][\arabic{##1}][\cref@result]%
                  \csname p@##1\endcsname\csname the##1\endcsname}%
              \else%
                \def\@tempa{##1}%
                \def\@tempb{subsubsection}%
                \ifx\@tempa\@tempb%
                  \protected@xdef\cref@currentlabel{%
                    [subsubappendix][\arabic{##1}][\cref@result]%
                    \csname p@##1\endcsname\csname the##1\endcsname}%
                \else%
                  \@ifundefined{cref@##1@alias}%
                    {\def\@tempa{##1}}%
                    {\def\@tempa{\csname cref@##1@alias\endcsname}}%
                  \protected@xdef\cref@currentlabel{%
                    [\@tempa][\arabic{##1}][\cref@result]%
                    \csname p@##1\endcsname\csname the##1\endcsname}
                \fi%
              \fi%
            \fi}%
        }{%
          \def\H@refstepcounter##1{%
            \cref@old@H@refstepcounter{##1}%
            \cref@constructprefix{##1}{\cref@result}%
            \ifx\cref@result\@empty%
              \def\cref@result{2147483647}%
            \else%
              \edef\cref@result{2147483647,\cref@result}%
            \fi%
            \def\@tempa{##1}%
            \def\@tempb{chapter}%
            \ifx\@tempa\@tempb%
              \protected@xdef\cref@currentlabel{%
                [appendix][\arabic{##1}][\cref@result]%
                \csname p@##1\endcsname\csname the##1\endcsname}%
            \else%
              \def\@tempa{##1}%
              \def\@tempb{section}%
              \ifx\@tempa\@tempb%
                \protected@xdef\cref@currentlabel{%
                  [subappendix][\arabic{##1}][\cref@result]%
                  \csname p@##1\endcsname\csname the##1\endcsname}%
              \else%
                \def\@tempa{##1}%
                \def\@tempb{subsection}%
                \ifx\@tempa\@tempb%
                  \protected@xdef\cref@currentlabel{%
                    [subsubappendix][\arabic{##1}][\cref@result]%
                    \csname p@##1\endcsname\csname the##1\endcsname}%
                \else%
                  \def\@tempa{##1}%
                  \def\@tempb{subsubsection}%
                  \ifx\@tempa\@tempb%
                    \protected@xdef\cref@currentlabel{%
                      [subsubsubappendix][\arabic{##1}][\cref@result]%
                      \csname p@##1\endcsname\csname the##1\endcsname}%
                  \else%
                    \@ifundefined{cref@##1@alias}%
                      {\def\@tempa{##1}}%
                      {\def\@tempa{\csname cref@##1@alias\endcsname}}%
                    \protected@xdef\cref@currentlabel{%
                      [\@tempa][\arabic{##1}][\cref@result]%
                      \csname p@##1\endcsname\csname the##1\endcsname}
                  \fi%
                \fi%
              \fi%
            \fi}%
        }%
      }%
    }% end of \@ifundefined{appendix}
    \DeclareRobustCommand{\cref}{%
      \@ifstar{\@crefstar{cref}}{\@crefnostar{cref}}}
    \DeclareRobustCommand{\Cref}{%
      \@ifstar{\@crefstar{Cref}}{\@crefnostar{Cref}}}
    \def\@crefnostar#1#2{\@cref{#1}{#2}}
    \def\@crefstar#1#2{%
      \@crefstarredtrue\@cref{#1}{#2}\@crefstarredfalse}
    \DeclareRobustCommand{\crefrange}{%
      \@ifstar{\@crefrangestar{cref}}{\@crefrangenostar{cref}}}
    \DeclareRobustCommand{\Crefrange}{%
      \@ifstar{\@crefrangestar{Cref}}{\@crefrangenostar{Cref}}}
    \def\@crefrangenostar#1#2#3{\@setcrefrange{#2}{#3}{#1}{}}
    \def\@crefrangestar#1#2#3{%
      \@crefstarredtrue\@setcrefrange{#2}{#3}{#1}{}\@crefstarredfalse}
    \DeclareRobustCommand{\cpageref}{%
      \@ifstar{\@cpagerefstar{cref}}{\@cpagerefnostar{cref}}}
    \DeclareRobustCommand{\Cpageref}{%
      \@ifstar{\@cpagerefstar{Cref}}{\@cpagerefnostar{Cref}}}
    \def\@cpagerefnostar#1#2{%
      \@cpageref{#1}{#2}{\@setcpageref}{\@setcpagerefrange}}
    \def\@cpagerefstar#1#2{%
      \@crefstarredtrue%
      \@cpageref{#1}{#2}{\@setcpageref}{\@setcpagerefrange}%
      \@crefstarredfalse}
    \DeclareRobustCommand{\cpagerefrange}{%
      \@ifstar{\@cpagerefrangestar{cref}}{\@cpagerefrangenostar{cref}}}
    \DeclareRobustCommand{\Cpagerefrange}{%
      \@ifstar{\@cpagerefrangestar{Cref}}{\@cpagerefrangenostar{Cref}}}
    \def\@cpagerefrangenostar#1#2#3{\@setcpagerefrange{#2}{#3}{#1}{}}
    \def\@cpagerefrangestar#1#2#3{%
      \@crefstarredtrue%
      \@setcpagerefrange{#2}{#3}{#1}{}%
      \@crefstarredfalse}
    \DeclareRobustCommand{\labelcref}{%
      \@ifstar{\@labelcrefstar}{\@labelcrefnostar}}
    \def\@labelcrefnostar#1{\@cref{labelcref}{#1}}
    \def\@labelcrefstar#1{%
      \@crefstarredtrue%
      \@cref{labelcref}{#1}%
      \@crefstarredfalse}
    \DeclareRobustCommand{\labelcpageref}{%
      \@ifstar{\@labelcpagerefstar}{\@labelcpagerefnostar}}
    \def\@labelcpagerefnostar#1{%
      \@cpageref{labelcref}{#1}{\@setcpageref}{\@setcpagerefrange}}
    \def\@labelcpagerefstar#1{%
      \@crefstarredtrue%
      \@cpageref{labelcref}{#1}{\@setcpageref}{\@setcpagerefrange}%
      \@crefstarredfalse}
    \def\@@setcref#1#2{%
      \cref@getlabel{#2}{\@templabel}%
      \if@crefstarred%
        #1{\@templabel}{}{}%
      \else%
        \edef\@templink{\cref@hyperref{#2}}%
        #1{\@templabel}{\hyper@linkstart{link}{\@templink}}%
          {\hyper@linkend}%
      \fi}
    \def\@@setcrefrange#1#2#3{%
      \cref@getlabel{#2}{\@labela}%
      \cref@getlabel{#3}{\@labelb}%
      \if@crefstarred%
        #1{\@labela}{\@labelb}{}{}{}{}%
      \else%
        \edef\@linka{\cref@hyperref{#2}}%
        \edef\@linkb{\cref@hyperref{#3}}%
        #1{\@labela}{\@labelb}%
          {\hyper@linkstart{link}{\@linka}}{\hyper@linkend}%
          {\hyper@linkstart{link}{\@linkb}}{\hyper@linkend}%
      \fi}%
    \def\@@setcpageref#1#2{%
      \cref@getpageref{#2}{\@temppage}%
      \if@crefstarred%
        #1{\@temppage}{}{}%
      \else%
        \edef\@templink{\cref@hyperref{#2}}%
        #1{\@temppage}{\hyper@linkstart{link}{\@templink}}%
          {\hyper@linkend}%
      \fi}
    \def\@@setcpagerefrange#1#2#3{%
      \cref@getpageref{#2}{\@pagea}%
      \cref@getpageref{#3}{\@pageb}%
      \if@crefstarred%
        #1{\@pagea}{\@pageb}{}{}{}{}%
      \else%
        \edef\@linka{\cref@hyperref{#2}}%
        \edef\@linkb{\cref@hyperref{#3}}%
        #1{\@pagea}{\@pageb}%
          {\hyper@linkstart{link}{\@linka}}{\hyper@linkend}%
          {\hyper@linkstart{link}{\@linkb}}{\hyper@linkend}%
      \fi}%
  }%  end of false case of \@ifpackagewith{hyperref}{implicit=false}
}{% false case of \@ifpackageloaded{hyperref}
  \@ifclassloaded{revtex4}{\let\if@cref@hyperrefloaded\iftrue}{}%
  \@ifclassloaded{revtex4-1}{\let\if@cref@hyperrefloaded\iftrue}{}%
  \if@cref@hyperrefloaded\relax%
    \let\cref@old@H@refstepcounter\H@refstepcounter%
    \def\H@refstepcounter#1{%
      \cref@old@H@refstepcounter{#1}%
      \cref@constructprefix{#1}{\cref@result}%
      \@ifundefined{cref@#1@alias}%
        {\def\@tempa{#1}}%
        {\def\@tempa{\csname cref@#1@alias\endcsname}}%
      \protected@xdef\cref@currentlabel{%
        [\@tempa][\arabic{#1}][\cref@result]%
        \csname p@#1\endcsname\csname the#1\endcsname}}%
  \fi%
  \let\if@cref@hyperrefloaded\iffalse%
}% end of \@ifpackageloaded{hyperref}
\@ifpackageloaded{amsmath}{%
  \AtBeginDocument{
    \let\cref@old@label@in@display\label@in@display
    \def\label@in@display{%
      \@ifnextchar[\label@in@display@optarg\label@in@display@noarg}%]
    \def\label@in@display@noarg#1{\cref@old@label@in@display{{#1}}}
    \def\label@in@display@optarg[#1]#2{%
      \cref@old@label@in@display{[#1]{#2}}}
    \def\ltx@label#1{\cref@label#1}
  }%  end of AtBeginDocument
  \def\measure@#1{%
    \begingroup
        \measuring@true
        \global\eqnshift@\z@
        \global\alignsep@\z@
        \global\let\tag@lengths\@empty
        \global\let\field@lengths\@empty
        \savecounters@
        \global\setbox0\vbox{%
            \let\math@cr@@@\math@cr@@@align@measure
            \everycr{\noalign{\global\tag@false
              \global\let\raise@tag\@empty \global\column@\z@}}%
            \let\label\@gobble@optarg%  <<< cleveref modification
            \global\row@\z@
            \tabskip\z@
            \halign{\span\align@preamble\crcr
                #1%
                \math@cr@@@
                \global\column@\z@
                \add@amps\maxfields@\cr
            }%
        }%
        \restorecounters@
        \ifodd\maxfields@
            \global\advance\maxfields@\@ne
        \fi
        \ifnum\xatlevel@=\tw@
            \ifnum\maxfields@<\thr@@
                \let\xatlevel@\z@
            \fi
        \fi
        \setbox\z@\vbox{%
          \unvbox\z@ \unpenalty \global\setbox\@ne\lastbox
        }%
        \global\totwidth@\wd\@ne
        \if@fleqn \global\advance\totwidth@\@mathmargin \fi
        \global\let\maxcolumn@widths\@empty
        \begingroup
          \let\or\relax
          \loop
            \global\setbox\@ne\hbox{%
              \unhbox\@ne \unskip \global\setbox\thr@@\lastbox
            }%
          \ifhbox\thr@@
           \xdef\maxcolumn@widths{ \or \the\wd\thr@@ \maxcolumn@widths}%
          \repeat
        \endgroup
        \dimen@\displaywidth
        \advance\dimen@-\totwidth@
        \ifcase\xatlevel@
            \global\alignsep@\z@
            \let\minalignsep\z@
            \@tempcntb\z@
            \if@fleqn
                \@tempcnta\@ne
                \global\eqnshift@\@mathmargin
            \else
                \@tempcnta\tw@
                \global\eqnshift@\dimen@
                \global\divide\eqnshift@\@tempcnta
            \fi
        \or
            \@tempcntb\maxfields@
            \divide\@tempcntb\tw@
            \@tempcnta\@tempcntb
            \advance\@tempcntb\m@ne
            \if@fleqn
                \global\eqnshift@\@mathmargin
                \global\alignsep@\dimen@
                \global\divide\alignsep@\@tempcnta
            \else
                \global\advance\@tempcnta\@ne
                \global\eqnshift@\dimen@
                \global\divide\eqnshift@\@tempcnta
                \global\alignsep@\eqnshift@
            \fi
        \or
            \@tempcntb\maxfields@
            \divide\@tempcntb\tw@
            \global\advance\@tempcntb\m@ne
            \global\@tempcnta\@tempcntb
            \global\eqnshift@\z@
            \global\alignsep@\dimen@
            \if@fleqn
                \global\advance\alignsep@\@mathmargin\relax
            \fi
            \global\divide\alignsep@\@tempcntb
        \fi
        \ifdim\alignsep@<\minalignsep\relax
            \global\alignsep@\minalignsep\relax
            \ifdim\eqnshift@>\z@
                \if@fleqn\else
                    \global\eqnshift@\displaywidth
                    \global\advance\eqnshift@-\totwidth@
                    \global\advance\eqnshift@-\@tempcntb\alignsep@
                    \global\divide\eqnshift@\tw@
                \fi
            \fi
        \fi
        \ifdim\eqnshift@<\z@
            \global\eqnshift@\z@
        \fi
        \calc@shift@align
        \global\tagshift@\totwidth@
        \global\advance\tagshift@\@tempcntb\alignsep@
        \if@fleqn
            \ifnum\xatlevel@=\tw@
                \global\advance\tagshift@-\@mathmargin\relax
            \fi
        \else
            \global\advance\tagshift@\eqnshift@
        \fi
        \iftagsleft@ \else
            \global\advance\tagshift@-\displaywidth
        \fi
        \dimen@\minalignsep\relax
        \global\advance\totwidth@\@tempcntb\dimen@
        \ifdim\totwidth@>\displaywidth
            \global\let\displaywidth@\totwidth@
        \else
            \global\let\displaywidth@\displaywidth
        \fi
    \endgroup
  }
  \def\gmeasure@#1{%
    \begingroup
        \measuring@true
        \totwidth@\z@
        \global\let\tag@lengths\@empty
        \savecounters@
        \setbox\@ne\vbox{%
            \everycr{\noalign{\global\tag@false
              \global\let\raise@tag\@empty \global\column@\z@}}%
            \let\label\@gobble%  <<< cleveref modification
            \halign{%
                \setboxz@h{$\m@th\displaystyle{##}$}%
                \ifdim\wdz@>\totwidth@
                    \global\totwidth@\wdz@
                \fi
               &\setboxz@h{\strut@{##}}%
                \savetaglength@
                \crcr
                #1%
                \math@cr@@@
            }%
        }%
        \restorecounters@
        \if@fleqn
            \global\advance\totwidth@\@mathmargin
        \fi
        \iftagsleft@
            \ifdim\totwidth@>\displaywidth
                \global\let\gdisplaywidth@\totwidth@
            \else
                \global\let\gdisplaywidth@\displaywidth
            \fi
        \fi
    \endgroup
}
  \def\multline@#1{%
    \Let@
    \@display@init{\global\advance\row@\@ne \global\dspbrk@lvl\m@ne}%
    \chardef\dspbrk@context\z@
    \restore@math@cr
    \let\tag\tag@in@align
    \global\tag@false \global\let\raise@tag\@empty
    \mmeasure@{#1}%
    \let\tag\gobble@tag \let\label\@gobble@optarg%  <<< cleveref modification
    \tabskip \if@fleqn \@mathmargin \else \z@skip \fi
    \totwidth@\displaywidth
    \if@fleqn
        \advance\totwidth@-\@mathmargin
    \fi
    \halign\bgroup
        \hbox to\totwidth@{%
            \if@fleqn
                \hskip \@centering \relax
            \else
                \hfil
            \fi
            \strut@
            $\m@th\displaystyle{}##\endmultline@math
            \hfil
        }% $
        \crcr
        \if@fleqn
            \hskip-\@mathmargin
            \def\multline@indent{\hskip\@mathmargin}%
        \else
            \hfilneg
            \def\multline@indent{\hskip\multlinegap}%
        \fi
        \iftagsleft@
            \iftag@
                \begingroup
                    \ifshifttag@
                        \rlap{\vbox{%
                                \normalbaselines
                                \hbox{%
                                    \strut@
                                    \make@display@tag
                                }%
                                \vbox to\lineht@{}%
                                \raise@tag
                        }}%
                        \multline@indent
                    \else
                        \setbox\z@\hbox{\make@display@tag}%
                        \dimen@\@mathmargin \advance\dimen@-\wd\z@
                        \ifdim\dimen@<\multlinetaggap
                          \dimen@\multlinetaggap
                        \fi
                        \box\z@ \hskip\dimen@\relax
                    \fi
                \endgroup
            \else
                \multline@indent
            \fi
        \else
            \multline@indent
        \fi
    #1%
  }
  \def\mmeasure@#1{%
    \begingroup
        \measuring@true
        \def\label{%                  <<< cleveref modification
          \@ifnextchar[\label@in@mmeasure@optarg%]
            \label@in@mmeasure@noarg}%
        \def\math@cr@@@{\cr}%
        \let\shoveleft\@iden \let\shoveright\@iden
        \savecounters@
        \global\row@\z@
        \setbox\@ne\vbox{%
            \global\let\df@tag\@empty
            \halign{%
                \setboxz@h{\@lign$\m@th\displaystyle{}##$}%
                \iftagsleft@
                    \ifnum\row@=\@ne
                        \global\totwidth@\wdz@
                        \global\lineht@\ht\z@
                    \fi
                \else
                    \global\totwidth@\wdz@
                    \global\lineht@\dp\z@
                \fi
                \crcr
                #1%
                \crcr
            }%
        }%
        \ifx\df@tag\@empty\else\global\tag@true\fi
        \if@eqnsw\global\tag@true\fi
        \iftag@
            \setboxz@h{%
                \if@eqnsw
                    \stepcounter{equation}%
                    \tagform@\theequation
                \else
                    \df@tag
                \fi
            }%
            \global\tagwidth@\wdz@
            \dimen@\totwidth@
            \advance\dimen@\tagwidth@
            \advance\dimen@\multlinetaggap
            \iftagsleft@\else
                \if@fleqn
                    \advance\dimen@\@mathmargin
                \fi
            \fi
            \ifdim\dimen@>\displaywidth
                \global\shifttag@true
            \else
                \global\shifttag@false
            \fi
        \fi
        \restorecounters@
    \endgroup
  }
  \def\label@in@mmeasure@noarg#1{%
    \begingroup%
      \measuring@false%
      \cref@old@label@in@display{{#1}}%
    \endgroup}
  \def\label@in@mmeasure@optarg[#1]#2{%
    \begingroup%
      \measuring@false%
      \cref@old@label@in@display{[#1]{#2}}%
    \endgroup}
  \let\cref@old@subequations\subequations%
  \let\cref@old@endsubequations\endsubequations%
  \cref@resetby{equation}{\cref@result}%
  \ifx\cref@result\relax\else%
    \@addtoreset{parentequation}{\cref@result}%
  \fi%
  \renewenvironment{subequations}{%
    \@addtoreset{equation}{parentequation}%
    \cref@old@subequations%
  }{%
    \gdef\cl@parentequation{}%
    \cref@old@endsubequations%
    \setcounter{parentequation}{0}%
  }%
  \def\make@df@tag@@#1{%
    \gdef\df@tag{\maketag@@@{#1}\def\@currentlabel{#1}%
      \def\cref@currentlabel{[equation][2147483647][]#1}}}
  \def\make@df@tag@@@#1{%
    \gdef\df@tag{\tagform@{#1}%
      \toks@\@xp{\p@equation{#1}}%
      \edef\@currentlabel{\the\toks@}%
      \edef\cref@currentlabel{[equation][2147483647][]\the\toks@}}}
}{}%  end of \@ifpackageloaded{amsmath}
\@ifpackageloaded{IEEEtrantools}{%
  \PackageInfo{cleveref}{`IEEEtrantools' support loaded}
  \let\cref@orig@@IEEEeqnarray\@@IEEEeqnarray
  \def\@@IEEEeqnarray[#1]#2{%
    \refstepcounter{equation}%
    \addtocounter{equation}{-1}%
    \cref@orig@@IEEEeqnarray[#1]{#2}}
  \let\cref@orig@IEEEeqnarrayXCR\@IEEEeqnarrayXCR
  \def\@IEEEeqnarrayXCR[#1]{%
    \if@eqnsw%
      \if@IEEEissubequation%
        %\addtocounter{equation}{1}%
        \refstepcounter{IEEEsubequation}%
        \addtocounter{IEEEsubequation}{-1}%
      \else%
        \refstepcounter{equation}%
        \addtocounter{equation}{-1}%
      \fi%
    \fi%
  \cref@orig@IEEEeqnarrayXCR[#1]}
  \let\cref@orig@IEEEyessubnumber\IEEEyessubnumber
  \def\IEEEyessubnumber{%
    \if@IEEEeqnarrayISinner%
      \if@IEEElastlinewassubequation\else%
        \setcounter{IEEEsubequation}{0}%
        \refstepcounter{IEEEsubequation}%
      \fi%
    \fi%
    \cref@orig@IEEEyessubnumber}
  \@addtoreset{IEEEsubequation}{equation}%
  \crefalias{IEEEsubequation}{equation}%
}{}% end of \@ifpackageloaded{IEEEtrantools}
  \@ifpackageloaded{amsthm}{%
  \PackageInfo{cleveref}{`amsthm' support loaded}
\let\cref@thmnoarg\@thm
\def\@thm{\@ifnextchar[{\cref@thmoptarg}{\cref@thmnoarg}}%]
\def\cref@thmoptarg[#1]#2#3#4{%
  \ifhmode\unskip\unskip\par\fi%
  \normalfont%
  \trivlist%
  \let\thmheadnl\relax%
  \let\thm@swap\@gobble%
  \thm@notefont{\fontseries\mddefault\upshape}%
  \thm@headpunct{.}% add period after heading
  \thm@headsep 5\p@ plus\p@ minus\p@\relax%
  \thm@space@setup%
  #2% style overrides
  \@topsep \thm@preskip               % used by thm head
  \@topsepadd \thm@postskip           % used by \@endparenv
  \def\@tempa{#3}\ifx\@empty\@tempa%
    \def\@tempa{\@oparg{\@begintheorem{#4}{}}[]}%
  \else%
    \refstepcounter[#1]{#3}%  <<< cleveref modification
    \def\@tempa{\@oparg{\@begintheorem{#4}{\csname the#3\endcsname}}[]}%
  \fi%
  \@tempa}
\def\@ynthm#1[#2]#3{%
  \edef\@tempa{\expandafter\noexpand%
    \csname cref@#1@name@preamble\endcsname}%
  \edef\@tempb{\expandafter\noexpand%
      \csname Cref@#1@name@preamble\endcsname}%
  \def\@tempc{#3}%
  \ifx\@tempc\@empty\relax%
    \expandafter\gdef\@tempa{}%
    \expandafter\gdef\@tempb{}%
  \else%
    \expandafter\expandafter\expandafter\gdef\expandafter%
      \@tempa\expandafter{\MakeLowercase #3}%
    \expandafter\expandafter\expandafter\gdef\expandafter%
      \@tempa\expandafter{\MakeUppercase #3}%
  \fi%
  \cref@stack@add{#1}{\cref@label@types}%
  \ifx\relax#2\relax%
    \def\@tempa{\@oparg{\@xthm{#1}{#3}}[]}%
  \else%
    \@ifundefined{c@#2}{%
      \def\@tempa{\@nocounterr{#2}}%
    }{%
      \@xp\xdef\csname the#1\endcsname{\@xp\@nx\csname the#2\endcsname}%
      \toks@{#3}%
      \@xp\xdef\csname#1\endcsname{%
        \@nx\@thm[#1]{%  <<< new optional argument for theorem name
          \let\@nx\thm@swap%
            \if S\thm@swap\@nx\@firstoftwo\else\@nx\@gobble\fi%
          \@xp\@nx\csname th@\the\thm@style\endcsname}%
            {#2}{\the\toks@}}%
      \let\@tempa\relax%
    }%
  \fi%
  \@tempa}
  \let\@xnthm\cref@old@xnthm
  }{}%  end of \@ifpackageloaded{amsthm}
  \@ifpackageloaded{ntheorem}{%
  \PackageInfo{cleveref}{`ntheorem' support loaded}
  \@ifpackagewith{ntheorem}{thref}{%
    \PackageWarning{cleveref}{`cleveref' supersedes `ntheorem's `thref'
      option}%
    \renewcommand{\thref}{\cref}}{}
  \@ifundefined{theorem@prework}{\let\theorem@prework\relax}{}
  \gdef\@thm#1#2#3{%
    \if@thmmarks%
      \stepcounter{end\InTheoType ctr}%
    \fi%
    \renewcommand{\InTheoType}{#1}%
    \if@thmmarks%
      \stepcounter{curr#1ctr}%
      \setcounter{end#1ctr}{0}%
    \fi%
    \refstepcounter[#1]{#2}%  <<< cleveref modification
    \theorem@prework%
    \thm@topsepadd \theorempostskipamount%
    \ifvmode \advance\thm@topsepadd\partopsep\fi%
    \trivlist%
    \@topsep \theorempreskipamount%
    \@topsepadd \thm@topsepadd%
    \advance\linewidth -\theorem@indent%
    \advance\@totalleftmargin \theorem@indent%
    \parshape \@ne \@totalleftmargin \linewidth%
    \@ifnextchar[{\@ythm{#1}{#2}{#3}}{\@xthm{#1}{#2}{#3}}%]
  }
  }{}%  end of \@ifpackageloaded{ntheorem}
\@ifpackageloaded{varioref}{%
  \PackageInfo{cleveref}{`varioref' support loaded}
  \PackageInfo{cleveref}{`cleveref' supersedes `varioref's %
    \string\labelformat command}
  \def\cref@@vpageref#1[#2]#3{%
    \@cpageref{cref}{#3}%
      {\@setvpageref[#1][\vref@space]}{\@setvpagerefrange[#1]}}
  \def\cref@vref#1#2{%
    \leavevmode%
    \@cref{#1}{#2}\@setcref@space%
    \cref@@vpageref{\reftextcurrent}[]{#2}}
  \def\cref@vrefrange#1#2#3{%
    \@setcrefrange{#2}{#3}{#1}{}\@setcref@space\vpagerefrange{#2}{#3}}
  \def\cref@fullref#1#2{%
    \@cref{#1}{#2}\@setcref@space%
    \@cpageref{cref}{#2}{\@setfullpageref}{\@setfullpagerefrange}}
  \def\cref@vpagerefconjunction#1{%
    \def\@tempa{#1}%
    \def\@tempb{@second}%
    \ifx\@tempa\@tempb\relax%
      \@setcref@pairconjunction%
    \else%
      \def\@tempb{@middle}%
      \ifx\@tempa\@tempb\relax%
        \@setcref@middleconjunction%
      \else%
        \def\@tempb{@last}%
        \ifx\@tempa\@tempb\relax%
          \@setcref@lastconjunction%
        \fi%
      \fi%
    \fi}
  \def\@setcref@space{ }
  \def\@setvpageref[#1][#2]#3#4#5{%
    \cref@vpagerefconjunction{#5}%
    \def\vref@space{}%
    \begingroup%
      \cref@patchreftexts{#5}%
      \@@setvpageref{#1}[#2]{#3}%
    \endgroup}
  \def\@@setvpageref#1[#2]#3{\cref@old@@vpageref{#1}[#2]{#3}}
  \def\@setvpagerefrange[#1]#2#3#4#5{%
    \cref@vpagerefconjunction{#5}%
    \let\vref@space\relax%
    \begingroup%
      \cref@patchreftexts{#5}%
      \@@setvpagerefrange[#1]{#2}{#3}%
    \endgroup}
  \def\@@setvpagerefrange[#1]#2#3{\vpagerefrange[#1]{#2}{#3}}
  \def\@setfullpageref#1#2#3{%
    \cref@vpagerefconjunction{#3}%
    \begingroup%
      \cref@patchreftexts{#3}%
      \@@setfullpageref{#1}%
    \endgroup}
  \def\@@setfullpageref#1{\reftextfaraway{#1}}
  \def\@setfullpagerefrange#1#2#3#4{%
    \cref@vpagerefconjunction{#4}%
    \begingroup%
      \cref@patchreftexts{#4}%
      \@@setfullpagerefrange{#1}{#2}%
    \endgroup}
  \def\@@setfullpagerefrange#1#2{\reftextpagerange{#1}{#2}}
  \def\cref@old@@vpageref#1[#2]#3{%
    \leavevmode%\unskip  <<<
    \global\advance\c@vrcnt\@ne
    \vref@pagenum\@tempa{\the\c@vrcnt @vr}%
    \vref@pagenum\@tempb{\the\c@vrcnt @xvr}%
    %\vref@label{\the\c@vrcnt @xvr}%  <<<
    \ifx\@tempa\@tempb\else
      \vref@err{\noexpand\vref or \noexpand\vpageref at page boundary
                \@tempb-\@tempa\space (may loop)%
                }%
    \fi
    \vrefpagenum\thevpagerefnum{#3}%
    \vref@space
    \ifx\@tempa\thevpagerefnum
      \def\@tempc{#1}%
      \ifx\@tempc\@empty
         \unskip
      \else
         #1%
      \fi
    \else
      #2%
      \is@pos@number\thevpagerefnum
         {%
          \is@pos@number\@tempa
           {\@tempcnta\@tempa
            \advance\@tempcnta\@ne
           }%
           {\@tempcnta\maxdimen}%
          \ifnum \thevpagerefnum =\@tempcnta
           \ifodd\@tempcnta
             \if@twoside
               \reftextfaceafter
             \else
               \reftextafter
             \fi
           \else
             \reftextafter
           \fi
          \else
            \advance\@tempcnta-2
            \ifnum \thevpagerefnum =\@tempcnta
              \ifodd\@tempcnta
                \reftextbefore
              \else
                \if@twoside
                  \reftextfacebefore
                \else
                  \reftextbefore
                \fi
              \fi
            \else
              \reftextfaraway{#3}%
            \fi
          \fi
         }%
         {\reftextfaraway{#3}}%
    \fi
    \vref@label{\the\c@vrcnt @xvr}%  <<<
    \vref@label{\the\c@vrcnt @vr}%
  }
  \let\creftextcurrent\reftextcurrent
  \let\creftextfaceafter\reftextfaceafter
  \let\creftextfacebefore\reftextfacebefore
  \let\creftextafter\reftextafter
  \let\creftextbefore\reftextbefore
  \let\creftextfaraway\reftextfaraway
  \let\creftextpagerange\reftextpagerange
  \def\cref@patchreftexts#1{%
    \cref@patchreftext{reftextcurrent}{#1}%
    \cref@patchreftext{reftextfaceafter}{#1}%
    \cref@patchreftext{reftextfacebefore}{#1}%
    \cref@patchreftext{reftextafter}{#1}%
    \cref@patchreftext{reftextbefore}{#1}}
  \def\cref@patchreftext#1#2{%
    \def\@tempa{#2}%
    \ifx\@tempa\@empty%
      \def\@tempc{}%
      \expandafter\ifx\csname #1\endcsname\@tempc\relax%
        \expandafter\def\csname #1\endcsname{\unskip}%
          %{\advance\count@group -1\reftextcurrent@orig}%
      \else%
        \long\def\@tempc{}%
        \expandafter\ifx\csname #1\endcsname\@tempc\relax%
          \expandafter\def\csname #1\endcsname{\unskip}%
            %{\advance\count@group -1\reftextcurrent@orig}%
        \fi%
      \fi%
    \else%
      \long\def\@tempc{\unskip}%
      \expandafter\ifx\csname #1\endcsname\@tempc\relax%
        \expandafter\expandafter\expandafter\def%
        \expandafter\expandafter\csname #1\endcsname\expandafter{%
          \csname c#1\endcsname}%
      \else%
        \long\def\@tempc{}%
        \expandafter\ifx\csname #1\endcsname\@tempc\relax%
          \expandafter\expandafter\expandafter\def%
          \expandafter\expandafter\csname #1\endcsname\expandafter{%
            \csname c#1\endcsname}%
        \else%
          \def\@tempc{\unskip}%
          \expandafter\ifx\csname #1\endcsname\@tempc\relax%
            \expandafter\expandafter\expandafter\def%
            \expandafter\expandafter\csname #1\endcsname\expandafter{%
              \csname c#1\endcsname}%
          \else%
            \def\@tempc{}%
            \expandafter\ifx\csname #1\endcsname\@tempc\relax%
              \expandafter\expandafter\expandafter\def%
              \expandafter\expandafter\csname #1\endcsname\expandafter{%
                \csname c#1\endcsname}%
            \fi%
          \fi%
        \fi%
      \fi%
    \fi}
  \def\@setcref@pairconjunction{\crefpairconjunction}
  \def\@setcref@middleconjunction{\crefmiddleconjunction}
  \def\@setcref@lastconjunction{\creflastconjunction}
  \AtBeginDocument{%
    \def\@@vpageref#1[#2]#3{\cref@@vpageref{#1}[#2]{#3}}
  }
  \if@cref@hyperrefloaded\relax%  hyperref loaded
    \DeclareRobustCommand{\vref}{%
      \@ifstar{\cref@vrefstar{cref}}{\cref@vref{cref}}}
    \DeclareRobustCommand{\Vref}{%
      \@ifstar{\cref@vrefstar{Cref}}{\cref@vref{Cref}}}
    \DeclareRobustCommand{\vrefrange}{%
      \@ifstar{\cref@vrefrangestar{cref}}{\cref@vrefrange{cref}}}
    \DeclareRobustCommand{\Vrefrange}{%
      \@ifstar{\cref@vrefrangestar{Cref}}{\cref@vrefrange{Cref}}}
    \DeclareRobustCommand{\fullref}{%
      \@ifstar{\cref@fullrefstar{cref}}{\cref@fullref{cref}}}
    \DeclareRobustCommand{\Fullref}{%
      \@ifstar{\cref@fullrefstar{Cref}}{\cref@fullref{Cref}}}
    \def\cref@vrefstar#1#2{%
      \@crefstarredtrue%
      \cref@vref{#1}{#2}%
      \@crefstarredfalse}
    \def\cref@vrefrangestar#1#2#3{%
      \@crefstarredtrue%
      \cref@vrefrange{#1}{#2}{#3}%
      \@crefstarredfalse}
    \def\cref@fullrefstar#1#2{%
      \@crefstarredtrue%
      \cref@fullref{#1}{#2}%
      \@crefstarredfalse}
  \else%
    \DeclareRobustCommand{\vref}{\cref@vref{cref}}
    \DeclareRobustCommand{\Vref}{\cref@vref{Cref}}
    \DeclareRobustCommand{\vrefrange}{\cref@vrefrange{cref}}
    \DeclareRobustCommand{\Vrefrange}{\cref@vrefrange{Cref}}
    \DeclareRobustCommand{\fullref}{\cref@fullref{cref}}
    \DeclareRobustCommand{\Fullref}{\cref@fullref{Cref}}
  \fi%  end of test for hyperref
}{}%  end of \@ifpackageloaded{varioref}
  \@ifpackageloaded{algorithm}{%
  \PackageInfo{cleveref}{`algorithm' support loaded}
  \let\cref@old@ALG@step\ALG@step
  \def\ALG@step{%
    \cref@old@ALG@step%
    \addtocounter{ALG@line}{-1}%
    \refstepcounter[line]{ALG@line}}
  }{}%  end of \@ifpackageloaded{algorithm}
  \@ifpackageloaded{listings}{%
    \PackageInfo{cleveref}{`listings' support loaded}
    \crefalias{lstnumber}{line}%
    \crefalias{lstlisting}{listing}%
  }{}%  end of \@ifpackageloaded{listings}
  \@ifpackageloaded{algorithm2e}{%
    \PackageInfo{cleveref}{`algorithm2e' support loaded}
    \crefalias{algocf}{algorithm}%
    \crefalias{algocfline}{line}%
  }{}%  end of \@ifpackageloaded{listings}
\@ifpackageloaded{subfig}{%
  \PackageInfo{cleveref}{`subfig' support loaded}
  \AtBeginDocument{
    \let\cref@old@refsteponlycounter\refsteponlycounter
    \def\refsteponlycounter{%
      \@ifnextchar[{\refstepcounter@optarg}%
        {\cref@old@refsteponlycounter}%]
    }}
  \def\sf@sub@label(#1){%
    \ifhyperrefloaded
      \protected@edef\@currentlabelname{%
        \expandafter\strip@period #1\relax.\relax\@@@}%
    \fi%
    \let\sf@oldlabel\cref@old@label%
    \let\cref@old@label\sf@@sub@label%
    \cref@label}%
  }{}%  end of \@ifpackageloaded{subfig}
\@ifpackageloaded{caption}{%
  \@ifpackagelater{caption}{2011/08/19}{}{%
    \PackageInfo{cleveref}{`caption' support loaded}
    \let\cref@old@caption@xlabel\caption@xlabel
    \def\caption@xlabel{%
      \let\cref@ORI@label\cref@old@label%
      \let\cref@old@label\cref@old@caption@xlabel%
      \let\caption@ORI@label\cref@ORI@label%
      \cref@label}%
    }% end of \@ifpackagelater
  }{}%  end of \@ifpackageloaded{caption}
\@ifpackageloaded{aliascnt}{%
  \PackageInfo{cleveref}{`aliascnt' support loaded}
  \let\cref@old@newaliascnt\newaliascnt
  \renewcommand*{\newaliascnt}[2]{%
    \cref@old@newaliascnt{#1}{#2}%
    \cref@resetby{#2}{\cref@result}%
    \ifx\cref@result\relax\else%
      \@addtoreset{#1}{\cref@result}%
    \fi}
  }{}%  end of \@ifpackageloaded{aliascnt}
\DeclareOption{poorman}{%
  \PackageInfo{cleveref}{option `poorman' loaded}
  \gdef\cref@poorman@text{}
  \AtBeginDocument{%
    \newwrite\@crefscript%
    \immediate\openout\@crefscript=\jobname.sed}
  \newif\if@cref@switched@language
  \@ifpackageloaded{babel}{%
    \AtBeginDocument{%
      \let\cref@old@select@language\select@language
      \def\select@language{%
        \@cref@switched@languagetrue%
        \cref@writelanguagerules%
        \cref@old@select@language}
      \let\cref@old@foreign@language\foreign@language
      \def\foreign@language{%
        \@cref@switched@languagetrue%
        \cref@writelanguagerules%
        \cref@old@foreign@language}
      \edef\cref@inputlineno{\the\inputlineno}}%
    }{}
  \AtEndDocument{%
    \let\select@language\cref@old@select@language%
    \let\foreign@language\cref@old@foreign@language%
    \cref@writelanguagerules}
  \def\cref@writelanguagerules{%
    \begingroup%
      \if@cref@switched@language%
        \edef\@address{\cref@inputlineno,\the\inputlineno}%
      \else%
        \def\@address{}%
      \fi%
      \expandafter\def\expandafter\cref@poorman@text\expandafter{%
        \crefrangeconjunction}%
      \expandafter\def\expandafter\@tempa\expandafter{%
        \expandafter{\@address}{\string\crefrangeconjunction}}%
      \expandafter\cref@writescript\@tempa%
      \expandafter\def\expandafter\cref@poorman@text\expandafter{%
        \crefrangepreconjunction}%
      \expandafter\def\expandafter\@tempa\expandafter{%
        \expandafter{\@address}{\string\crefrangepreconjunction}}%
      \expandafter\cref@writescript\@tempa%
      \expandafter\def\expandafter\cref@poorman@text\expandafter{%
        \crefrangepostconjunction}%
      \expandafter\def\expandafter\@tempa\expandafter{%
        \expandafter{\@address}{\string\crefrangepostconjunction}}%
      \expandafter\cref@writescript\@tempa%
      \expandafter\def\expandafter\cref@poorman@text\expandafter{%
        \crefpairconjunction}%
      \expandafter\def\expandafter\@tempa\expandafter{%
        \expandafter{\@address}{\string\crefpairconjunction}}%
      \expandafter\cref@writescript\@tempa%
      \expandafter\def\expandafter\cref@poorman@text\expandafter{%
        \crefmiddleconjunction}%
      \expandafter\def\expandafter\@tempa\expandafter{%
        \expandafter{\@address}{\string\crefmiddleconjunction}}%
      \expandafter\cref@writescript\@tempa%
      \expandafter\def\expandafter\cref@poorman@text\expandafter{%
        \creflastconjunction}%
      \expandafter\def\expandafter\@tempa\expandafter{%
        \expandafter{\@address}{\string\creflastconjunction}}%
      \expandafter\cref@writescript\@tempa%
      \expandafter\def\expandafter\cref@poorman@text\expandafter{%
        \crefpairgroupconjunction}%
      \expandafter\def\expandafter\@tempa\expandafter{%
        \expandafter{\@address}{\string\crefpairgroupconjunction}}%
      \expandafter\cref@writescript\@tempa%
      \expandafter\def\expandafter\cref@poorman@text\expandafter{%
        \crefmiddlegroupconjunction}%
      \expandafter\def\expandafter\@tempa\expandafter{%
        \expandafter{\@address}{\string\crefmiddlegroupconjunction}}%
      \expandafter\cref@writescript\@tempa%
      \expandafter\def\expandafter\cref@poorman@text\expandafter{%
        \creflastgroupconjunction}%
      \expandafter\def\expandafter\@tempa\expandafter{%
        \expandafter{\@address}{\string\creflastgroupconjunction}}%
      \expandafter\cref@writescript\@tempa%
      \let\@tempstack\cref@label@types%
      \cref@isstackfull{\@tempstack}%
      \@whilesw\if@cref@stackfull\fi{%
        \edef\@tempa{\cref@stack@top{\@tempstack}}%
        \expandafter\expandafter\expandafter\def%
        \expandafter\expandafter\expandafter\cref@poorman@text%
        \expandafter\expandafter\expandafter{%
          \csname cref@\@tempa @name\endcsname}%
        \edef\@tempa{%
          \string\cref@\expandafter\noexpand\@tempa @name\space}%
        \expandafter\expandafter\expandafter\def%
        \expandafter\expandafter\expandafter\@tempa%
        \expandafter\expandafter\expandafter{%
          \expandafter\expandafter\expandafter{%
            \expandafter\@address\expandafter}%
          \expandafter{\@tempa}}%
        \expandafter\cref@writescript\@tempa%
        \edef\@tempa{\cref@stack@top{\@tempstack}}%
        \expandafter\expandafter\expandafter\def%
        \expandafter\expandafter\expandafter\cref@poorman@text%
        \expandafter\expandafter\expandafter{%
          \csname cref@\@tempa @name@plural\endcsname}%
        \edef\@tempa{%
          \string\cref@\expandafter\noexpand\@tempa%
          @name@plural\space}%
        \expandafter\expandafter\expandafter\def%
        \expandafter\expandafter\expandafter\@tempa%
        \expandafter\expandafter\expandafter{%
          \expandafter\expandafter\expandafter{%
            \expandafter\@address\expandafter}%
          \expandafter{\@tempa}}%
        \expandafter\cref@writescript\@tempa%
        \edef\@tempa{\cref@stack@top{\@tempstack}}%
        \expandafter\expandafter\expandafter\def%
        \expandafter\expandafter\expandafter\cref@poorman@text%
        \expandafter\expandafter\expandafter{%
          \csname Cref@\@tempa @name\endcsname}%
        \edef\@tempa{%
          \string\Cref@\expandafter\noexpand\@tempa @name\space}%
        \expandafter\expandafter\expandafter\def%
        \expandafter\expandafter\expandafter\@tempa%
        \expandafter\expandafter\expandafter{%
          \expandafter\expandafter\expandafter%
          {\expandafter\@address\expandafter}%
          \expandafter{\@tempa}}%
        \expandafter\cref@writescript\@tempa%
        \edef\@tempa{\cref@stack@top{\@tempstack}}%
        \expandafter\expandafter\expandafter\def%
        \expandafter\expandafter\expandafter\cref@poorman@text%
        \expandafter\expandafter\expandafter{%
          \csname Cref@\@tempa @name@plural\endcsname}%
        \edef\@tempa{%
          \string\Cref@\expandafter\noexpand\@tempa%
          @name@plural\space}%
        \expandafter\expandafter\expandafter\def%
        \expandafter\expandafter\expandafter\@tempa%
        \expandafter\expandafter\expandafter{%
          \expandafter\expandafter\expandafter%
          {\expandafter\@address\expandafter}%
          \expandafter{\@tempa}}%
        \expandafter\cref@writescript\@tempa%
        \cref@stack@pop{\@tempstack}%
        \cref@isstackfull{\@tempstack}}%
    \endgroup%
    \edef\cref@inputlineno{\the\inputlineno}}%
  \AtEndDocument{%
    \immediate\closeout\@crefscript%
    \newread\@crefscript%
    \immediate\openin\@crefscript=\jobname.sed%
    \begingroup%
      \newif\if@not@eof%
      \def\@eof{\par }%
      \catcode`.=13 \catcode`*=13
      \catcode`[=13 \catcode`]=13
      \catcode`^=13 \catcode`$=13 %$
      \catcode`\=0 \catcode`<=1 \catcode`>=2
      \catcode`\\=13 \catcode`\{=12 \catcode`\}=12 \catcode`_=12
      \lccode`/=92
      \lccode`~=92\lowercase{\def~{\string/\string/}}%
      \lccode`~=42\lowercase{\def~{\string/\string*}}%
      \lccode`~=46\lowercase{\def~{\string/\string.}}%
      \lccode`~=91\lowercase{\def~{\string/\string[}}%
      \lccode`~=93\lowercase{\def~{\string/\string]}}%
      \lccode`~=94\lowercase{\def~{\string/\string^}}%
      \lccode`~=36\lowercase{\def~{\string/\string$}}% $
      \lccode`~=0 \lccode`/=0 \catcode`~=12
      \def\cref@poorman@text{}%
      \immediate\read\@crefscript to \@tempa%
      \ifx\@tempa\@eof%
        \@not@eoffalse%
      \else%
        \@not@eoftrue%
        \edef\@tempa{\@tempa}%
      \fi%
      \@whilesw\if@not@eof\fi{%
        \expandafter\g@addto@macro\expandafter%
          \cref@poorman@text\expandafter{\@tempa^^J}%
        \immediate\read\@crefscript to \@tempa%
        \ifx\@tempa\@eof%
          \@not@eoffalse%
        \else%
          \@not@eoftrue%
          \edef\@tempa{\@tempa}%
        \fi}%
    \endgroup%
    \immediate\closein\@crefscript%
    \begingroup%
      \lccode`|=92 \lccode`<=123 \lccode`>=125 \lccode`C=67
      \lowercase{\def\@tempa{%[
          s/||label|[[^]]*|]/||label/g}}
      \expandafter\g@addto@macro\expandafter%
        \cref@poorman@text\expandafter{\@tempa^^J}%
      \lowercase{\edef\@tempa{s/||usepackage|(|[.*|]|)|<0,1|><cleveref>//g}}%
      \expandafter\g@addto@macro\expandafter%
        \cref@poorman@text\expandafter{\@tempa^^J}%
      \lowercase{\edef\@tempa{s/||[cC]refformat<.*><.*>//g}}%
      \expandafter\g@addto@macro\expandafter%
        \cref@poorman@text\expandafter{\@tempa^^J}%
      \lowercase{\edef\@tempa{s/||[cC]refrangeformat<.*><.*>//g}}%
      \expandafter\g@addto@macro\expandafter%
        \cref@poorman@text\expandafter{\@tempa^^J}%
      \lowercase{\edef\@tempa{s/||[cC]refmultiformat<.*><.*><.*><.*>//g}}%
      \expandafter\g@addto@macro\expandafter%
        \cref@poorman@text\expandafter{\@tempa^^J}%
      \lowercase{\edef\@tempa{%
          s/||[cC]refrangemultiformat<.*><.*><.*><.*>//g}}%
      \expandafter\g@addto@macro\expandafter%
        \cref@poorman@text\expandafter{\@tempa^^J}%
      \lowercase{\edef\@tempa{s/||[cC]refname<.*><.*>//g}}%
      \expandafter\g@addto@macro\expandafter%
        \cref@poorman@text\expandafter{\@tempa^^J}%
      \lowercase{\edef\@tempa{s/||[cC]reflabelformat<.*><.*>//g}}%
      \expandafter\g@addto@macro\expandafter%
        \cref@poorman@text\expandafter{\@tempa^^J}%
      \lowercase{\edef\@tempa{s/||[cC]refrangelabelformat<.*><.*>//g}}%
      \expandafter\g@addto@macro\expandafter%
        \cref@poorman@text\expandafter{\@tempa^^J}%
      \lowercase{\edef\@tempa{s/||[cC]refdefaultlabelformat<.*>//g}}%
      \expandafter\g@addto@macro\expandafter%
        \cref@poorman@text\expandafter{\@tempa^^J}%
      \lowercase{\edef\@tempa{%
          s/||renewcommand<||crefpairconjunction><.*>//g}}%
      \expandafter\g@addto@macro\expandafter%
        \cref@poorman@text\expandafter{\@tempa^^J}%
      \lowercase{\edef\@tempa{%
          s/||renewcommand<||crefpairgroupconjunction><.*>//g}}%
      \expandafter\g@addto@macro\expandafter%
        \cref@poorman@text\expandafter{\@tempa^^J}%
      \lowercase{\edef\@tempa{%
          s/||renewcommand<||crefmiddleconjunction><.*>//g}}%
      \expandafter\g@addto@macro\expandafter%
        \cref@poorman@text\expandafter{\@tempa^^J}%
      \lowercase{\edef\@tempa{%
          s/||renewcommand<||crefmiddlegroupconjunction><.*>//g}}%
      \expandafter\g@addto@macro\expandafter%
        \cref@poorman@text\expandafter{\@tempa^^J}%
      \lowercase{\edef\@tempa{%
          s/||renewcommand<||creflastconjunction><.*>//g}}%
      \expandafter\g@addto@macro\expandafter%
        \cref@poorman@text\expandafter{\@tempa^^J}%
      \lowercase{\edef\@tempa{%
          s/||renewcommand<||creflastgroupconjunction><.*>//g}}%
      \expandafter\g@addto@macro\expandafter%
        \cref@poorman@text\expandafter{\@tempa^^J}%
      \lowercase{\edef\@tempa{s/||renewcommand<||[cC]ref><.*>//g}}%
      \expandafter\g@addto@macro\expandafter%
        \cref@poorman@text\expandafter{\@tempa^^J}%
      \lowercase{\edef\@tempa{s/||renewcommand<||[cC]refrange><.*>//g}}%
      \expandafter\g@addto@macro\expandafter%
        \cref@poorman@text\expandafter{\@tempa^^J}%
    \endgroup%
    \newwrite\@crefscript%
    \immediate\openout\@crefscript=\jobname.sed%
    \immediate\write\@crefscript{\cref@poorman@text}%
    \immediate\closeout\@crefscript%
  }%  end of \AtEndDocument
  \def\cref@getmeaning#1{\expandafter\@cref@getmeaning\meaning#1\@nil}
  \def\@cref@getmeaning#1->#2\@nil{#2}
  \def\cref@writescript#1#2{%
    \edef\@tempa{\cref@getmeaning{\cref@poorman@text}}%
    \immediate\write\@crefscript{#1 s/#2/\@tempa/g}}
  \if@cref@hyperrefloaded\relax%  hyperref loaded
    \def\@crefnostar#1#2{%
      \gdef\cref@poorman@text{}%
      \@cref{#1}{#2}%
      \def\@tempa##1##2\@nil{%
        \if##1c%
          \cref@writescript{}{\string\cref\string{#2\string}}%
        \else%
          \cref@writescript{}{\string\Cref\string{#2\string}}%
        \fi}%
      \@tempa#1\@nil}
    \def\@crefstar#1#2{%
      \gdef\cref@poorman@text{}%
      \@crefstarredtrue\@cref{#1}{#2}\@crefstarredfalse%
      \def\@tempa##1##2\@nil{%
        \if##1c%
          \cref@writescript{}{\string\cref*\string{#2\string}}%
        \else%
          \cref@writescript{}{\string\Cref*\string{#2\string}}%
        \fi}%
      \@tempa#1\@nil}
    \def\@crefrangenostar#1#2#3{%
      \gdef\cref@poorman@text{}%
      \@setcrefrange{#2}{#3}{#1}{}%
      \def\@tempa##1##2\@nil{%
        \if##1c%
          \cref@writescript{}{%
            \string\crefrange\string{#2\string}\string{#3\string}}%
        \else%
          \cref@writescript{}{%
            \string\Crefrange\string{#2\string}\string{#3\string}}%
        \fi}%
      \@tempa#1\@nil}
    \def\@crefrangestar#1#2#3{%
      \gdef\cref@poorman@text{}%
      \@crefstarredtrue\@setcrefrange{#2}{#3}{#1}{}\@crefstarredfalse%
      \def\@tempa##1##2\@nil{%
        \if##1c%
          \cref@writescript{}{%
            \string\crefrange*\string{#2\string}\string{#3\string}}%
        \else%
          \cref@writescript{}{%
            \string\Crefrange*\string{#2\string}\string{#3\string}}%
        \fi}%
      \@tempa#1\@nil}
    \def\@cpagerefnostar#1#2{%
      \gdef\cref@poorman@text{}%
      \@cpageref{#1}{#2}{\@setcpageref}{\@setcpagerefrange}%
      \def\@tempa##1##2\@nil{%
        \if##1c%
          \cref@writescript{}{\string\cpageref\string{#2\string}}%
        \else%
          \cref@writescript{}{\string\Cpageref\string{#2\string}}%
        \fi}%
      \@tempa#1\@nil}
    \def\@cpagerefstar#1#2{%
      \gdef\cref@poorman@text{}%
      \@crefstarredtrue%
      \@cpageref{#1}{#2}{\@setcpageref}{\@setcpagerefrange}%
      \@crefstarredfalse%
      \def\@tempa##1##2\@nil{%
        \if##1c%
          \cref@writescript{}{\string\cpageref*\string{#2\string}}%
        \else%
          \cref@writescript{}{\string\Cpageref*\string{#2\string}}%
        \fi}%
      \@tempa#1\@nil}
    \def\@cpagerefrangenostar#1#2#3{%
      \gdef\cref@poorman@text{}%
      \@setcpagerefrange{#2}{#3}{#1}{}%
      \def\@tempa##1##2\@nil{%
        \if##1c%
          \cref@writescript{}{%
            \string\cpagerefrange\string{#2\string}\string{#3\string}}%
        \else%
          \cref@writescript{}{%
            \string\Cpagerefrange\string{#2\string}\string{#3\string}}%
        \fi}%
      \@tempa#1\@nil}
    \def\@cpagerefrangestar#1#2#3{%
      \gdef\cref@poorman@text{}%
      \@crefstarredtrue%
      \@setcpagerefrange{#2}{#3}{#1}{}%
      \@crefstarredfalse%
      \def\@tempa##1##2\@nil{%
        \if##1c%
          \cref@writescript{}{%
            \string\cpagerefrange*\string{#2\string}\string{#3\string}}%
        \else%
          \cref@writescript{}{%
            \string\Cpagerefrange*\string{#2\string}\string{#3\string}}%
        \fi}%
      \@tempa#1\@nil}
    \def\@labelcrefnostar#1{%
      \gdef\cref@poorman@text{}%
      \@cref{labelcref}{#1}%
      \cref@writescript{}{\string\labelcref\string{#1\string}}}
    \def\@labelcrefstar#1{%
      \gdef\cref@poorman@text{}%
      \@crefstarredtrue%
      \@cref{labelcref}{#1}%
      \@crefstarredfalse%
      \cref@writescript{}{\string\labelcref*\string{#1\string}}}
    \def\@labelcpagerefnostar#1{%
      \gdef\cref@poorman@text{}%
      \@cpageref{labelcref}{#1}{\@setcpageref}{\@setcpagerefrange}%
      \cref@writescript{}{\string\labelcpageref\string{#1\string}}}
    \def\@labelcpagerefstar#1{%
      \gdef\cref@poorman@text{}%
      \@crefstarredtrue%
      \@cpageref{labelcref}{#1}{\@setcpageref}{\@setcpagerefrange}%
      \@crefstarredfalse%
      \cref@writescript{}{\string\labelcpageref*\string{#1\string}}}
  \else%  hyperref not loaded
    \DeclareRobustCommand{\cref}[1]{%
      \gdef\cref@poorman@text{}%
      \@cref{cref}{#1}%
      \cref@writescript{}{\string\cref\string{#1\string}}}
    \DeclareRobustCommand{\Cref}[1]{%
      \gdef\cref@poorman@text{}%
      \@cref{Cref}{#1}%
      \cref@writescript{}{\string\Cref\string{#1\string}}}
    \DeclareRobustCommand{\crefrange}[2]{%
      \gdef\cref@poorman@text{}%
      \@setcrefrange{#1}{#2}{cref}{}%
      \cref@writescript{}{%
        \string\crefrange\string{#1\string}\string{#2\string}}}
    \DeclareRobustCommand{\Crefrange}[2]{%
      \gdef\cref@poorman@text{}%
      \@setcrefrange{#1}{#2}{Cref}{}%
      \cref@writescript{}{%
        \string\Crefrange\string{#1\string}\string{#2\string}}}
    \DeclareRobustCommand{\cpageref}[1]{%
      \gdef\cref@poorman@text{}%
      \@cpageref{cref}{#1}{\@setcpageref}{\@setcpagerefrange}%
      \cref@writescript{}{\string\cpageref\string{#1\string}}}
    \DeclareRobustCommand{\Cpageref}[1]{%
      \gdef\cref@poorman@text{}%
      \@cpageref{Cref}{#1}{\@setcpageref}{\@setcpagerefrange}%
      \cref@writescript{}{\string\Cpageref\string{#1\string}}}
    \DeclareRobustCommand{\cpagerefrange}[2]{%
      \gdef\cref@poorman@text{}%
      \@setcpagerefrange{#1}{#2}{cref}{}%
      \cref@writescript{}{%
        \string\cpagerefrange\string{#1\string}\string{#2\string}}}
    \DeclareRobustCommand{\Cpagerefrange}[2]{%
      \gdef\cref@poorman@text{}%
      \@setcpagerefrange{#1}{#2}{Cref}{}%
      \cref@writescript{}{%
        \string\Cpagerefrange\string{#1\string}\string{#2\string}}}
    \DeclareRobustCommand{\labelcref}[1]{%
      \gdef\cref@poorman@text{}%
      \@cref{labelcref}{#1}%
      \cref@writescript{}{\string\labelcref\string{#1\string}}}
    \DeclareRobustCommand{\labelcpageref}[1]{%
      \gdef\cref@poorman@text{}%
      \@cpageref{labelcref}{#1}{\@setcpageref}{\@setcpagerefrange}%
      \cref@writescript{}{\string\labelcpageref\string{#1\string}}}
  \fi%  end of test for hyperref
  \DeclareRobustCommand{\namecref}[1]{%
    \gdef\cref@poorman@text{}%
    \@setnamecref{cref}{#1}{}{}%
    \cref@writescript{}{\string\namecref\string{#1\string}}}
  \DeclareRobustCommand{\nameCref}[1]{%
    \gdef\cref@poorman@text{}%
    \@setnamecref{Cref}{#1}{}{}%
    \cref@writescript{}{\string\nameCref\string{#1\string}}}
  \DeclareRobustCommand{\lcnamecref}[1]{%
    \gdef\cref@poorman@text{}%
    \@setnamecref{Cref}{#1}{}{\MakeLowercase}%
    \cref@writescript{}{\string\lcnamecref\string{#1\string}}}
  \DeclareRobustCommand{\namecrefs}[1]{%
    \gdef\cref@poorman@text{}%
    \@setnamecref{cref}{#1}{@plural}{}%
    \cref@writescript{}{\string\namecrefs\string{#1\string}}}
  \DeclareRobustCommand{\nameCrefs}[1]{%
    \gdef\cref@poorman@text{}%
    \@setnamecref{Cref}{#1}{@plural}{}%
    \cref@writescript{}{\string\nameCrefs\string{#1\string}}}
  \DeclareRobustCommand{\lcnamecrefs}[1]{%
    \gdef\cref@poorman@text{}%
    \@setnamecref{Cref}{#1}{@plural}{\MakeLowercase}%
    \cref@writescript{}{\string\lcnamecrefs\string{#1\string}}}
  \def\@setcref@pairgroupconjunction{%
    \crefpairgroupconjunction%
    \expandafter\g@addto@macro\expandafter\cref@poorman@text%
      \expandafter{\crefpairgroupconjunction}}
  \def\@setcref@middlegroupconjunction{%
    \crefmiddlegroupconjunction%
    \expandafter\g@addto@macro\expandafter\cref@poorman@text%
      \expandafter{\crefmiddlegroupconjunction}}
  \def\@setcref@lastgroupconjunction{%
    \creflastgroupconjunction%
    \expandafter\g@addto@macro\expandafter\cref@poorman@text%
      \expandafter{\creflastgroupconjunction}}
  \let\old@@setcref\@@setcref
  \let\old@@setcrefrange\@@setcrefrange
  \let\old@@setcpageref\@@setcpageref
  \let\old@@setcpagerefrange\@@setcpagerefrange
  \if@cref@hyperrefloaded\relax%  hyperref loaded
    \def\@@setcref#1#2{%
      \old@@setcref{#1}{#2}%
      \if@crefstarred%
        \expandafter\g@addto@macro\expandafter\cref@poorman@text%
          \expandafter{#1{\ref*{#2}}{}{}}%
      \else%
        \expandafter\g@addto@macro\expandafter\cref@poorman@text%
          \expandafter{#1{\ref{#2}}{}{}}%
      \fi}
    \def\@@setcrefrange#1#2#3{%
      \old@@setcrefrange{#1}{#2}{#3}%
      \if@crefstarred%
        \expandafter\g@addto@macro\expandafter\cref@poorman@text%
          \expandafter{#1{\ref*{#2}}{\ref*{#3}}{}{}{}{}}%
      \else%
        \expandafter\g@addto@macro\expandafter\cref@poorman@text%
          \expandafter{#1{\ref{#2}}{\ref{#3}}{}{}{}{}}%
      \fi}
    \def\@@setcpageref#1#2{%
      \old@@setcpageref{#1}{#2}%
      \if@crefstarred%
        \expandafter\g@addto@macro\expandafter\cref@poorman@text%
          \expandafter{#1{\pageref*{#2}}{}{}}%
      \else%
        \expandafter\g@addto@macro\expandafter\cref@poorman@text%
          \expandafter{#1{\pageref{#2}}{}{}}%
      \fi}
    \def\@@setcpagerefrange#1#2#3{%
      \old@@setcpagerefrange{#1}{#2}{#3}%
      \if@crefstarred%
        \expandafter\g@addto@macro\expandafter\cref@poorman@text%
          \expandafter{#1{\pageref*{#2}}{\pageref*{#3}}{}{}{}{}}%
      \else%
        \expandafter\g@addto@macro\expandafter\cref@poorman@text%
          \expandafter{#1{\pageref{#2}}{\pageref{#3}}{}{}{}{}}%
      \fi}
  \else%  hyperref not loaded
    \def\@@setcref#1#2{%
      \old@@setcref{#1}{#2}%
      \expandafter\g@addto@macro\expandafter{%
        \expandafter\cref@poorman@text\expandafter}%
        \expandafter{#1{\ref{#2}}{}{}}}
    \def\@@setcrefrange#1#2#3{%
      \old@@setcrefrange{#1}{#2}{#3}%
      \expandafter\g@addto@macro%
        \expandafter{\expandafter\cref@poorman@text\expandafter}%
        \expandafter{#1{\ref{#2}}{\ref{#3}}{}{}{}{}}}
    \def\@@setcpageref#1#2{%
      \old@@setcpageref{#1}{#2}%
      \expandafter\g@addto@macro\expandafter{%
        \expandafter\cref@poorman@text\expandafter}%
        \expandafter{#1{\pageref{#2}}{}{}}}
    \def\@@setcpagerefrange#1#2#3{%
      \old@@setcpagerefrange{#1}{#2}{#3}%
      \expandafter\g@addto@macro%
        \expandafter{\expandafter\cref@poorman@text\expandafter}%
        \expandafter{#1{\pageref{#2}}{\pageref{#3}}{}{}{}{}}}
  \fi%  end of hyperref test
  \let\old@@setnamecref\@@setnamecref
  \def\@@setnamecref#1#2{%
    \old@@setnamecref{#1}{#2}%
    \expandafter\def\expandafter\@tempa\expandafter{#1}%
    \def\@tempb{#2}%
    \expandafter\expandafter\expandafter\g@addto@macro%
      \expandafter\expandafter\expandafter{%
      \expandafter\expandafter\expandafter\cref@poorman@text%
      \expandafter\expandafter\expandafter}%
      \expandafter\expandafter\expandafter{\expandafter\@tempb\@tempa}}
  \@ifpackageloaded{varioref}{%
    \AtBeginDocument{%
      \def\@@vpageref#1[#2]#3{%
        \gdef\cref@poorman@text{}%
        \cref@@vpageref{#1}[#2]{#3}%
        \cref@writescript{}{\string\vpageref\string{#3\string}}}
      \let\old@cref@vref\cref@vref
      \def\cref@vref#1#2{%
        \gdef\cref@poorman@text{}%
        \old@cref@vref{#1}{#2}%
        \def\@tempa##1##2\@nil{%
          \if##1c%
            \if@crefstarred%
              \cref@writescript{}{\string\vref*\string{#2\string}}%
            \else%
              \cref@writescript{}{\string\vref\string{#2\string}}%
            \fi%
          \else%
            \if@crefstarred%
              \cref@writescript{}{\string\Vref*\string{#2\string}}%
            \else%
              \cref@writescript{}{\string\Vref\string{#2\string}}%
            \fi%
          \fi}%
        \@tempa#1\@nil}
      \let\old@cref@fullref\cref@fullref
      \def\cref@fullref#1#2{%
        \gdef\cref@poorman@text{}%
        \old@cref@fullref{#1}{#2}%
        \def\@tempa##1##2\@nil{%
          \if##1c%
            \if@crefstarred%
              \cref@writescript{}{\string\fullref*\string{#2\string}}%
            \else%
              \cref@writescript{}{\string\fullref\string{#2\string}}%
            \fi%
          \else%
            \if@crefstarred%
              \cref@writescript{}{\string\Fullref*\string{#2\string}}%
            \else%
              \cref@writescript{}{\string\Fullref\string{#2\string}}%
            \fi%
          \fi}%
        \@tempa#1\@nil}
      \let\old@cref@vrefrange\cref@vrefrange
      \def\cref@vrefrange#1#2#3{%
        \gdef\cref@poorman@text{}%
        \old@cref@vrefrange{#1}{#2}{#3}%
        \def\@tempa##1##2\@nil{%
          \if##1c%
            \if@crefstarred%
              \cref@writescript{}{%
                \string\vrefrange*\string{#2\string}\string{#3\string}}%
            \else%
              \cref@writescript{}{%
                \string\vrefrange\string{#2\string}\string{#3\string}}%
            \fi%
          \else%
            \if@crefstarred%
              \cref@writescript{}{%
                \string\Vrefrange*\string{#2\string}\string{#3\string}}%
            \else%
              \cref@writescript{}{%
                \string\Vrefrange\string{#2\string}\string{#3\string}}%
            \fi%
          \fi}%
        \@tempa#1\@nil}
      \def\@@setvpageref#1[#2]#3{%
        \cref@old@@vpageref{#1}[#2]{#3}%
        \g@addto@macro\cref@poorman@text{\vpageref{#3}}}
      \def\@@setvpagerefrange[#1]#2#3{%
        \vpagerefrange[#1]{#2}{#3}%
        \g@addto@macro\cref@poorman@text{\vpagerefrange{#2}{#3}}}
      \def\@@setfullpageref#1{%
        \reftextfaraway{#1}%
        \g@addto@macro\cref@poorman@text{\reftextfaraway{#1}}}
      \def\@@setfullpagerefrange#1#2{%
        \reftextpagerange{#1}{#2}%
        \g@addto@macro\cref@poorman@text{\reftextpagerange{#1}{#2}}}
      \def\@setcref@space{ % space here is deliberate
        \g@addto@macro\cref@poorman@text{ }}
      \def\@setcref@pairconjunction{%
        \crefpairconjunction%
        \expandafter\g@addto@macro\expandafter\cref@poorman@text%
          \expandafter{\crefpairconjunction}}
      \def\@setcref@middleconjunction{%
        \crefmiddleconjunction%
        \expandafter\g@addto@macro\expandafter\cref@poorman@text%
          \expandafter{\crefmiddleconjunction}}
      \def\@setcref@lastconjunction{%
        \creflastconjunction%
        \expandafter\g@addto@macro\expandafter\cref@poorman@text%
          \expandafter{\creflastconjunction}}
    }% end of \AtBeginDocument
  }{}% end of \@ifpackageloaded{varioref}
}%  end of poorman option
\newif\if@cref@sort
\newif\if@cref@compress
\@cref@sorttrue
\@cref@compresstrue
\DeclareOption{sort}{%
  \PackageInfo{cleveref}{sorting but not compressing references}
  \@cref@sorttrue
  \@cref@compressfalse}
\DeclareOption{compress}{%
  \PackageInfo{cleveref}{compressing but not sorting references}
  \@cref@sortfalse
  \@cref@compresstrue}
\DeclareOption{sort&compress}{%
  \PackageInfo{cleveref}{sorting and compressing references}
  \@cref@sorttrue
  \@cref@compresstrue}
\DeclareOption{nosort}{%
  \PackageInfo{cleveref}{neither sorting nor compressing references}
  \@cref@sortfalse
  \@cref@compressfalse}
\newif\if@cref@capitalise
\@cref@capitalisefalse
\DeclareOption{capitalise}{%
  \PackageInfo{cleveref}{always capitalise cross-reference names}
  \@cref@capitalisetrue}
\DeclareOption{capitalize}{%
  \PackageInfo{cleveref}{always capitalise cross-reference names}
  \@cref@capitalisetrue}
\newif\if@cref@nameinlink
\@cref@nameinlinkfalse
\DeclareOption{nameinlink}{%
  \PackageInfo{cleveref}{include cross-reference names in hyperlinks}
  \@cref@nameinlinktrue}
\newif\if@cref@abbrev
\@cref@abbrevtrue
\DeclareOption{noabbrev}{%
  \PackageInfo{cleveref}{no abbreviation of names}
  \@cref@abbrevfalse}
\def\cref@addto#1#2{%
  \@temptokena{#2}%
  \ifx#1\undefined%
    \edef#1{\the\@temptokena}%
  \else%
    \toks@\expandafter{#1}%
    \edef#1{\the\toks@\the\@temptokena}%
  \fi%
  \@temptokena{}\toks@\@temptokena%
}
\@onlypreamble\cref@addto
\DeclareOption{english}{%
  \PackageInfo{cleveref}{loaded `english' language definitions}
  \AtBeginDocument{%
    \def\crefrangeconjunction@preamble{ to\nobreakspace}%
    \def\crefrangepreconjunction@preamble{}%
    \def\crefrangepostconjunction@preamble{}%
    \def\crefpairconjunction@preamble{ and\nobreakspace}%
    \def\crefmiddleconjunction@preamble{, }%
    \def\creflastconjunction@preamble{ and\nobreakspace}%
    \def\crefpairgroupconjunction@preamble{ and\nobreakspace}%
    \def\crefmiddlegroupconjunction@preamble{, }%
    \def\creflastgroupconjunction@preamble{, and\nobreakspace}%
 %
    \Crefname@preamble{equation}{Equation}{Equations}%
    \Crefname@preamble{figure}{Figure}{Figures}%
    \Crefname@preamble{table}{Table}{Tables}%
    \Crefname@preamble{page}{Page}{Pages}%
    \Crefname@preamble{part}{Part}{Parts}%
    \Crefname@preamble{chapter}{Chapter}{Chapters}%
    \Crefname@preamble{section}{Section}{Sections}%
    \Crefname@preamble{appendix}{Appendix}{Appendices}%
    \Crefname@preamble{enumi}{Item}{Items}%
    \Crefname@preamble{footnote}{Footnote}{Footnotes}%
    \Crefname@preamble{theorem}{Theorem}{Theorems}%
    \Crefname@preamble{lemma}{Lemma}{Lemmas}%
    \Crefname@preamble{corollary}{Corollary}{Corollaries}%
    \Crefname@preamble{proposition}{Proposition}{Propositions}%
    \Crefname@preamble{definition}{Definition}{Definitions}%
    \Crefname@preamble{result}{Result}{Results}%
    \Crefname@preamble{example}{Example}{Examples}%
    \Crefname@preamble{remark}{Remark}{Remarks}%
    \Crefname@preamble{note}{Note}{Notes}%
    \Crefname@preamble{algorithm}{Algorithm}{Algorithms}%
    \Crefname@preamble{listing}{Listing}{Listings}%
    \Crefname@preamble{line}{Line}{Lines}%
 %
    \if@cref@capitalise%  capitalise set
      \if@cref@abbrev%
        \crefname@preamble{equation}{Eq.}{Eqs.}%
        \crefname@preamble{figure}{Fig.}{Figs.}%
      \else%
        \crefname@preamble{equation}{Equation}{Equations}%
        \crefname@preamble{figure}{Figure}{Figures}%
      \fi%
      \crefname@preamble{page}{Page}{Pages}%
      \crefname@preamble{table}{Table}{Tables}%
      \crefname@preamble{part}{Part}{Parts}%
      \crefname@preamble{chapter}{Chapter}{Chapters}%
      \crefname@preamble{section}{Section}{Sections}%
      \crefname@preamble{appendix}{Appendix}{Appendices}%
      \crefname@preamble{enumi}{Item}{Items}%
      \crefname@preamble{footnote}{Footnote}{Footnotes}%
      \crefname@preamble{theorem}{Theorem}{Theorems}%
      \crefname@preamble{lemma}{Lemma}{Lemmas}%
      \crefname@preamble{corollary}{Corollary}{Corollaries}%
      \crefname@preamble{proposition}{Proposition}{Propositions}%
      \crefname@preamble{definition}{Definition}{Definitions}%
      \crefname@preamble{result}{Result}{Results}%
      \crefname@preamble{example}{Example}{Examples}%
      \crefname@preamble{remark}{Remark}{Remarks}%
      \crefname@preamble{note}{Note}{Notes}%
      \crefname@preamble{algorithm}{Algorithm}{Algorithms}%
      \crefname@preamble{listing}{Listing}{Listings}%
      \crefname@preamble{line}{Line}{Lines}%
 %
    \else%  capitalise unset
      \if@cref@abbrev%
        \crefname@preamble{equation}{eq.}{eqs.}%
        \crefname@preamble{figure}{fig.}{figs.}%
      \else%
        \crefname@preamble{equation}{equation}{equations}%
        \crefname@preamble{figure}{figure}{figures}%
      \fi%
      \crefname@preamble{page}{page}{pages}%
      \crefname@preamble{table}{table}{tables}%
      \crefname@preamble{part}{part}{parts}%
      \crefname@preamble{chapter}{chapter}{chapters}%
      \crefname@preamble{section}{section}{sections}%
      \crefname@preamble{appendix}{appendix}{appendices}%
      \crefname@preamble{enumi}{item}{items}%
      \crefname@preamble{footnote}{footnote}{footnotes}%
      \crefname@preamble{theorem}{theorem}{theorems}%
      \crefname@preamble{lemma}{lemma}{lemmas}%
      \crefname@preamble{corollary}{corollary}{corollaries}%
      \crefname@preamble{proposition}{proposition}{propositions}%
      \crefname@preamble{definition}{definition}{definitions}%
      \crefname@preamble{result}{result}{results}%
      \crefname@preamble{example}{example}{examples}%
      \crefname@preamble{remark}{remark}{remarks}%
      \crefname@preamble{note}{note}{notes}%
      \crefname@preamble{algorithm}{algorithm}{algorithms}%
      \crefname@preamble{listing}{listing}{listings}%
      \crefname@preamble{line}{line}{lines}%
    \fi%
    \def\cref@language{english}%
    \cref@addto\extrasenglish{%
      \renewcommand{\crefrangeconjunction}{ to\nobreakspace}%
      \renewcommand\crefrangepreconjunction{}%
      \renewcommand\crefrangepostconjunction{}%
      \renewcommand{\crefpairconjunction}{ and\nobreakspace}%
      \renewcommand{\crefmiddleconjunction}{, }%
      \renewcommand{\creflastconjunction}{ and\nobreakspace}%
      \renewcommand{\crefpairgroupconjunction}{ and\nobreakspace}%
      \renewcommand{\crefmiddlegroupconjunction}{, }%
      \renewcommand{\creflastgroupconjunction}{, and\nobreakspace}%
 %
      \Crefname{equation}{Equation}{Equations}%
      \Crefname{figure}{Figure}{Figures}%
      \Crefname{subfigure}{Figure}{Figures}%
      \Crefname{table}{Table}{Tables}%
      \Crefname{subtable}{Table}{Tables}%
      \Crefname{page}{Page}{Pages}%
      \Crefname{part}{Part}{Parts}%
      \Crefname{chapter}{Chapter}{Chapters}%
      \Crefname{section}{Section}{Sections}%
      \Crefname{subsection}{Section}{Sections}%
      \Crefname{subsubsection}{Section}{Sections}%
      \Crefname{appendix}{Appendix}{Appendices}%
      \Crefname{subappendix}{Appendix}{Appendices}%
      \Crefname{subsubappendix}{Appendix}{Appendices}%
      \Crefname{subsubsubappendix}{Appendix}{Appendices}%
      \Crefname{enumi}{Item}{Items}%
      \Crefname{enumii}{Item}{Items}%
      \Crefname{enumiii}{Item}{Items}%
      \Crefname{enumiv}{Item}{Items}%
      \Crefname{enumv}{Item}{Items}%
      \Crefname{footnote}{Footnote}{Footnotes}%
      \Crefname{theorem}{Theorem}{Theorems}%
      \Crefname{lemma}{Lemma}{Lemmas}%
      \Crefname{corollary}{Corollary}{Corollaries}%
      \Crefname{proposition}{Proposition}{Propositions}%
      \Crefname{definition}{Definition}{Definitions}%
      \Crefname{result}{Result}{Results}%
      \Crefname{example}{Example}{Examples}%
      \Crefname{remark}{Remark}{Remarks}%
      \Crefname{note}{Note}{Notes}%
      \Crefname{algorithm}{Algorithm}{Algorithms}%
      \Crefname{listing}{Listing}{Listings}%
      \Crefname{line}{Line}{Lines}%
 %
      \if@cref@capitalise%  capitalise set
        \if@cref@abbrev%
          \crefname{equation}{Eq.}{Eqs.}%
          \crefname{figure}{Fig.}{Figs.}%
          \crefname{subfigure}{Fig.}{Figs.}%
        \else%
          \crefname{equation}{Equation}{Equations}%
          \crefname{figure}{Figure}{Figures}%
          \crefname{subfigure}{Figure}{Figures}%
        \fi%
        \crefname{page}{Page}{Pages}%
        \crefname{table}{Table}{Tables}%
        \crefname{subtable}{Table}{Tables}%
        \crefname{part}{Part}{Parts}%
        \crefname{chapter}{Chapter}{Chapters}%
        \crefname{section}{Section}{Sections}%
        \crefname{subsection}{Section}{Sections}%
        \crefname{subsubsection}{Section}{Sections}%
        \crefname{appendix}{Appendix}{Appendices}%
        \crefname{subappendix}{Appendix}{Appendices}%
        \crefname{subsubappendix}{Appendix}{Appendices}%
        \crefname{subsubsubappendix}{Appendix}{Appendices}%
        \crefname{enumi}{Item}{Items}%
        \crefname{enumii}{Item}{Items}%
        \crefname{enumiii}{Item}{Items}%
        \crefname{enumiv}{Item}{Items}%
        \crefname{enumv}{Item}{Items}%
        \crefname{footnote}{Footnote}{Footnotes}%
        \crefname{theorem}{Theorem}{Theorems}%
        \crefname{lemma}{Lemma}{Lemmas}%
        \crefname{corollary}{Corollary}{Corollaries}%
        \crefname{proposition}{Proposition}{Propositions}%
        \crefname{definition}{Definition}{Definitions}%
        \crefname{result}{Result}{Results}%
        \crefname{example}{Example}{Examples}%
        \crefname{remark}{Remark}{Remarks}%
        \crefname{note}{Note}{Notes}%
        \crefname{algorithm}{Algorithm}{Algorithms}%
        \crefname{listing}{Listing}{Listings}%
        \crefname{line}{Line}{Lines}%
 %
      \else%  capitalise unset
        \if@cref@abbrev%
          \crefname{equation}{eq.}{eqs.}%
          \crefname{figure}{fig.}{figs.}%
          \crefname{subfigure}{fig.}{figs.}%
        \else%
          \crefname{equation}{equation}{equations}%
          \crefname{figure}{figure}{figures}%
          \crefname{subfigure}{figure}{figures}%
        \fi%
        \crefname{table}{table}{tables}%
        \crefname{subtable}{table}{tables}%
        \crefname{page}{page}{pages}%
        \crefname{part}{part}{parts}%
        \crefname{chapter}{chapter}{chapters}%
        \crefname{section}{section}{sections}%
        \crefname{subsection}{section}{sections}%
        \crefname{subsubsection}{section}{sections}%
        \crefname{appendix}{appendix}{appendices}%
        \crefname{subappendix}{appendix}{appendices}%
        \crefname{subsubappendix}{appendix}{appendices}%
        \crefname{subsubsubappendix}{appendix}{appendices}%
        \crefname{enumi}{item}{items}%
        \crefname{enumii}{item}{items}%
        \crefname{enumiii}{item}{items}%
        \crefname{enumiv}{item}{items}%
        \crefname{enumv}{item}{items}%
        \crefname{footnote}{footnote}{footnotes}%
        \crefname{theorem}{theorem}{theorems}%
        \crefname{lemma}{lemma}{lemmas}%
        \crefname{corollary}{corollary}{corollaries}%
        \crefname{proposition}{proposition}{propositions}%
        \crefname{definition}{definition}{definitions}%
        \crefname{result}{result}{results}%
        \crefname{example}{example}{examples}%
        \crefname{remark}{remark}{remarks}%
        \crefname{note}{note}{notes}%
        \crefname{algorithm}{algorithm}{algorithms}%
        \crefname{listing}{listing}{listings}%
        \crefname{line}{line}{lines}%
      \fi%
    }}}
\DeclareOption{german}{%
  \PackageInfo{cleveref}{loaded `german' language definitions}
  \AtBeginDocument{%
    \def\crefrangeconjunction@preamble{ bis\nobreakspace}%
    \def\crefrangepreconjunction@preamble{}%
    \def\crefrangepostconjunction@preamble{}%
    \def\crefpairconjunction@preamble{ und\nobreakspace}%
    \def\crefmiddleconjunction@preamble{, }%
    \def\creflastconjunction@preamble{ und\nobreakspace}%
    \def\crefpairgroupconjunction@preamble{ und\nobreakspace}%
    \def\crefmiddlegroupconjunction@preamble{, }%
    \def\creflastgroupconjunction@preamble{ und\nobreakspace}%
 %
    \Crefname@preamble{equation}{Gleichung}{Gleichungen}%
    \Crefname@preamble{figure}{Abbildung}{Abbildungen}%
    \Crefname@preamble{table}{Tabelle}{Tabellen}%
    \Crefname@preamble{page}{Seite}{Seiten}%
    \Crefname@preamble{part}{Teil}{Teile}%
    \Crefname@preamble{chapter}{Kapitel}{Kapitel}%
    \Crefname@preamble{section}{Abschnitt}{Abschnitte}%
    \Crefname@preamble{appendix}{Anhang}{Anh\"ange}%
    \Crefname@preamble{enumi}{Punkt}{Punkte}%
    \Crefname@preamble{footnote}{Fu\ss note}{Fu\ss noten}%
    \Crefname@preamble{theorem}{Theorem}{Theoreme}%
    \Crefname@preamble{lemma}{Lemma}{Lemmata}%
    \Crefname@preamble{corollary}{Korollar}{Korollare}%
    \Crefname@preamble{proposition}{Satz}{S\"atze}%
    \Crefname@preamble{definition}{Definition}{Definitionen}%
    \Crefname@preamble{result}{Ergebnis}{Ergebnisse}%
    \Crefname@preamble{example}{Beispiel}{Beispiele}%
    \Crefname@preamble{remark}{Bemerkung}{Bemerkungen}%
    \Crefname@preamble{note}{Anmerkung}{Anmerkungen}%
    \Crefname@preamble{algorithm}{Algorithmus}{Algorithmen}%
    \Crefname@preamble{listing}{Listing}{Listings}%
    \Crefname@preamble{line}{Zeile}{Zeilen}%
 %
    \crefname@preamble{equation}{Gleichung}{Gleichungen}%
    \crefname@preamble{figure}{Abbildung}{Abbildungen}%
    \crefname@preamble{table}{Tabelle}{Tabellen}%
    \crefname@preamble{page}{Seite}{Seiten}%
    \crefname@preamble{part}{Teil}{Teile}%
    \crefname@preamble{chapter}{Kapitel}{Kapitel}%
    \crefname@preamble{section}{Abschnitt}{Abschnitte}%
    \crefname@preamble{appendix}{Anhang}{Anh\"ange}%
    \crefname@preamble{enumi}{Punkt}{Punkte}%
    \crefname@preamble{footnote}{Fu\ss note}{Fu\ss noten}%
    \crefname@preamble{theorem}{Theorem}{Theoreme}%
    \crefname@preamble{lemma}{Lemma}{Lemmata}%
    \crefname@preamble{corollary}{Korollar}{Korollare}%
    \crefname@preamble{proposition}{Satz}{S\"atze}%
    \crefname@preamble{definition}{Definition}{Definitionen}%
    \crefname@preamble{result}{Ergebnis}{Ergebnisse}%
    \crefname@preamble{example}{Beispiel}{Beispiele}%
    \crefname@preamble{remark}{Bemerkung}{Bemerkungen}%
    \crefname@preamble{note}{Anmerkung}{Anmerkungen}%
    \crefname@preamble{algorithm}{Algorithmus}{Algorithmen}%
    \crefname@preamble{listing}{Listing}{Listings}%
    \crefname@preamble{line}{Zeile}{Zeilen}%
    \def\cref@language{german}%
    \cref@addto\extrasgerman{%
      \renewcommand{\crefrangeconjunction}{ bis\nobreakspace}%
      \renewcommand\crefrangepreconjunction{}%
      \renewcommand\crefrangepostconjunction{}%
      \renewcommand{\crefpairconjunction}{ und\nobreakspace}%
      \renewcommand{\crefmiddleconjunction}{, }%
      \renewcommand{\creflastconjunction}{ und\nobreakspace}%
      \renewcommand{\crefpairgroupconjunction}{ und\nobreakspace}%
      \renewcommand{\crefmiddlegroupconjunction}{, }%
      \renewcommand{\creflastgroupconjunction}{ und\nobreakspace}%
 %
      \Crefname{equation}{Gleichung}{Gleichungen}%
      \Crefname{figure}{Abbildung}{Abbildungen}%
      \Crefname{subfigure}{Abbildung}{Abbildungen}%
      \Crefname{table}{Tabelle}{Tabellen}%
      \Crefname{subtable}{Tabelle}{Tabellen}%
      \Crefname{page}{Seite}{Seiten}%
      \Crefname{part}{Teil}{Teile}%
      \Crefname{chapter}{Kapitel}{Kapitel}%
      \Crefname{section}{Abschnitt}{Abschnitte}%
      \Crefname{subsection}{Abschnitt}{Abschnitte}%
      \Crefname{subsubsection}{Abschnitt}{Abschnitte}%
      \Crefname{appendix}{Anhang}{Anh\"ange}%
      \Crefname{subappendix}{Anhang}{Anh\"ange}%
      \Crefname{subsubappendix}{Anhang}{Anh\"ange}%
      \Crefname{subsubsubappendix}{Anhang}{Anh\"ange}%
      \Crefname{enumi}{Punkt}{Punkte}%
      \Crefname{enumii}{Punkt}{Punkte}%
      \Crefname{enumiii}{Punkt}{Punkte}%
      \Crefname{enumiv}{Punkt}{Punkte}%
      \Crefname{enumv}{Punkt}{Punkte}%
      \Crefname{footnote}{Fu\ss note}{Fu\ss noten}%
      \Crefname{theorem}{Theorem}{Theoreme}%
      \Crefname{lemma}{Lemma}{Lemmata}%
      \Crefname{corollary}{Korollar}{Korollare}%
      \Crefname{proposition}{Satz}{S\"atze}%
      \Crefname{definition}{Definition}{Definitionen}%
      \Crefname{result}{Ergebnis}{Ergebnisse}%
      \Crefname{example}{Beispiel}{Beispiele}%
      \Crefname{remark}{Bemerkung}{Bemerkungen}%
      \Crefname{note}{Anmerkung}{Anmerkungen}%
      \Crefname{algorithm}{Algorithmus}{Algorithmen}%
      \Crefname{listing}{Listing}{Listings}%
      \Crefname{line}{Zeile}{Zeilen}%
 %
      \crefname{equation}{Gleichung}{Gleichungen}%
      \crefname{figure}{Abbildung}{Abbildungen}%
      \crefname{subfigure}{Abbildung}{Abbildungen}%
      \crefname{table}{Tabelle}{Tabellen}%
      \crefname{subtable}{Tabelle}{Tabellen}%
      \crefname{page}{Seite}{Seiten}%
      \crefname{part}{Teil}{Teile}%
      \crefname{chapter}{Kapitel}{Kapitel}%
      \crefname{section}{Abschnitt}{Abschnitte}%
      \crefname{subsection}{Abschnitt}{Abschnitte}%
      \crefname{subsubsection}{Abschnitt}{Abschnitte}%
      \crefname{appendix}{Anhang}{Anh\"ange}%
      \crefname{subappendix}{Anhang}{Anh\"ange}%
      \crefname{subsubappendix}{Anhang}{Anh\"ange}%
      \crefname{subsubsubappendix}{Anhang}{Anh\"ange}%
      \crefname{enumi}{Punkt}{Punkte}%
      \crefname{enumii}{Punkt}{Punkte}%
      \crefname{enumiii}{Punkt}{Punkte}%
      \crefname{enumiv}{Punkt}{Punkte}%
      \crefname{enumv}{Punkt}{Punkte}%
      \crefname{footnote}{Fu\ss note}{Fu\ss noten}%
      \crefname{theorem}{Theorem}{Theoreme}%
      \crefname{lemma}{Lemma}{Lemmata}%
      \crefname{corollary}{Korollar}{Korollare}%
      \crefname{proposition}{Satz}{S\"atze}%
      \crefname{definition}{Definition}{Definitionen}%
      \crefname{result}{Ergebnis}{Ergebnisse}%
      \crefname{example}{Beispiel}{Beispiele}%
      \crefname{remark}{Bemerkung}{Bemerkungen}%
      \crefname{note}{Anmerkung}{Anmerkungen}%
      \crefname{algorithm}{Algorithmus}{Algorithmen}%
      \crefname{listing}{Listing}{Listings}%
      \crefname{line}{Zeile}{Zeilen}%
    }}}
\DeclareOption{ngerman}{%
  \PackageInfo{cleveref}{loaded `ngerman' language definitions}
  \ExecuteOptions{german}
  \def\cref@language{ngerman}
  \AtBeginDocument{%
    \cref@addto\extrasngerman{%
      \renewcommand{\crefrangeconjunction}{ bis\nobreakspace}%
      \renewcommand\crefrangepreconjunction{}%
      \renewcommand\crefrangepostconjunction{}%
      \renewcommand{\crefpairconjunction}{ und\nobreakspace}%
      \renewcommand{\crefmiddleconjunction}{, }%
      \renewcommand{\creflastconjunction}{ und\nobreakspace}%
      \renewcommand{\crefpairgroupconjunction}{ und\nobreakspace}%
      \renewcommand{\crefmiddlegroupconjunction}{, }%
      \renewcommand{\creflastgroupconjunction}{ und\nobreakspace}%
 %
      \Crefname{equation}{Gleichung}{Gleichungen}%
      \Crefname{figure}{Abbildung}{Abbildungen}%
      \Crefname{subfigure}{Abbildung}{Abbildungen}%
      \Crefname{table}{Tabelle}{Tabellen}%
      \Crefname{subtable}{Tabelle}{Tabellen}%
      \Crefname{page}{Seite}{Seiten}%
      \Crefname{part}{Teil}{Teile}%
      \Crefname{chapter}{Kapitel}{Kapitel}%
      \Crefname{section}{Abschnitt}{Abschnitte}%
      \Crefname{subsection}{Abschnitt}{Abschnitte}%
      \Crefname{subsubsection}{Abschnitt}{Abschnitte}%
      \Crefname{appendix}{Anhang}{Anh\"ange}%
      \Crefname{subappendix}{Anhang}{Anh\"ange}%
      \Crefname{subsubappendix}{Anhang}{Anh\"ange}%
      \Crefname{subsubsubappendix}{Anhang}{Anh\"ange}%
      \Crefname{enumi}{Punkt}{Punkte}%
      \Crefname{enumii}{Punkt}{Punkte}%
      \Crefname{enumiii}{Punkt}{Punkte}%
      \Crefname{enumiv}{Punkt}{Punkte}%
      \Crefname{enumv}{Punkt}{Punkte}%
      \Crefname{footnote}{Fu\ss note}{Fu\ss noten}%
      \Crefname{theorem}{Theorem}{Theoreme}%
      \Crefname{lemma}{Lemma}{Lemmata}%
      \Crefname{corollary}{Korollar}{Korollare}%
      \Crefname{proposition}{Satz}{S\"atze}%
      \Crefname{definition}{Definition}{Definitionen}%
      \Crefname{result}{Ergebnis}{Ergebnisse}%
      \Crefname{example}{Beispiel}{Beispiele}%
      \Crefname{remark}{Bemerkung}{Bemerkungen}%
      \Crefname{note}{Anmerkung}{Anmerkungen}%
      \Crefname{algorithm}{Algorithmus}{Algorithmen}%
      \Crefname{listing}{Listing}{Listings}%
      \Crefname{line}{Zeile}{Zeilen}%
 %
      \crefname{equation}{Gleichung}{Gleichungen}%
      \crefname{figure}{Abbildung}{Abbildungen}%
      \crefname{subfigure}{Abbildung}{Abbildungen}%
      \crefname{table}{Tabelle}{Tabellen}%
      \crefname{subtable}{Tabelle}{Tabellen}%
      \crefname{page}{Seite}{Seiten}%
      \crefname{part}{Teil}{Teile}%
      \crefname{chapter}{Kapitel}{Kapitel}%
      \crefname{section}{Abschnitt}{Abschnitte}%
      \crefname{subsection}{Abschnitt}{Abschnitte}%
      \crefname{subsubsection}{Abschnitt}{Abschnitte}%
      \crefname{appendix}{Anhang}{Anh\"ange}%
      \crefname{subappendix}{Anhang}{Anh\"ange}%
      \crefname{subsubappendix}{Anhang}{Anh\"ange}%
      \crefname{subsubsubappendix}{Anhang}{Anh\"ange}%
      \crefname{enumi}{Punkt}{Punkte}%
      \crefname{enumii}{Punkt}{Punkte}%
      \crefname{enumiii}{Punkt}{Punkte}%
      \crefname{enumiv}{Punkt}{Punkte}%
      \crefname{enumv}{Punkt}{Punkte}%
      \crefname{footnote}{Fu\ss note}{Fu\ss noten}%
      \crefname{theorem}{Theorem}{Theoreme}%
      \crefname{lemma}{Lemma}{Lemmata}%
      \crefname{corollary}{Korollar}{Korollare}%
      \crefname{proposition}{Satz}{S\"atze}%
      \crefname{definition}{Definition}{Definitionen}%
      \crefname{result}{Ergebnis}{Ergebnisse}%
      \crefname{example}{Beispiel}{Beispiele}%
      \crefname{remark}{Bemerkung}{Bemerkungen}%
      \crefname{note}{Anmerkung}{Anmerkungen}%
      \crefname{algorithm}{Algorithmus}{Algorithmen}%
      \crefname{listing}{Listing}{Listings}%
      \crefname{line}{Zeile}{Zeilen}%
    }}}
\DeclareOption{dutch}{%
  \PackageInfo{cleveref}{loaded `dutch' language definitions}
  \AtBeginDocument{%
    \def\crefrangeconjunction@preamble{ tot\nobreakspace}%
    \def\crefrangepreconjunction@preamble{}%
    \def\crefrangepostconjunction@preamble{}%
    \def\crefpairconjunction@preamble{ en\nobreakspace}%
    \def\crefmiddleconjunction@preamble{, }%
    \def\creflastconjunction@preamble{ en\nobreakspace}%
    \def\crefpairgroupconjunction@preamble{ en\nobreakspace}%
    \def\crefmiddlegroupconjunction@preamble{, }%
    \def\creflastgroupconjunction@preamble{ en\nobreakspace}%
 %
    \Crefname@preamble{equation}{Vergel\ij{}king}{Vergel\ij{}kingen}%
    \Crefname@preamble{figure}{Figuur}{Figuren}%
    \Crefname@preamble{table}{Tabel}{Tabellen}%
    \Crefname@preamble{page}{Pagina}{Pagina's}%
    \Crefname@preamble{part}{Deel}{Delen}%
    \Crefname@preamble{chapter}{Hoofdstuk}{Hoofdstuken}%
    \Crefname@preamble{section}{Paragraaf}{Paragrafen}%
    \Crefname@preamble{appendix}{Appendix}{Appendices}%
    \Crefname@preamble{enumi}{Punt}{Punten}%
    \Crefname@preamble{footnote}{Voetnote}{Voetnoten}%
    \Crefname@preamble{lemma}{Lemma}{Lemma's}%
    \Crefname@preamble{corollary}{Corollarium}{Corollaria}%
    \Crefname@preamble{proposition}{Bewering}{Beweringen}%
    \Crefname@preamble{definition}{Definitie}{Definities}%
    \Crefname@preamble{result}{Resultaat}{Resultaten}%
    \Crefname@preamble{example}{Voorbeeld}{Voorbeelden}%
    \Crefname@preamble{remark}{Opmerking}{Opmerkingen}%
    \Crefname@preamble{note}{Aantekening}{Aantekeningen}%
    \Crefname@preamble{algorithm}{Algoritme}{Algoritmen}%
    \Crefname@preamble{listing}{Listing}{Listings}%
    \Crefname@preamble{line}{Lijn}{Lijnen}%
 %
    \if@cref@capitalise%  capitalise set
      \if@cref@abbrev%
        \crefname@preamble{equation}{Verg.}{Verg's.}%
        \crefname@preamble{figure}{Fig.}{Fig's.}%
      \else%
        \crefname@preamble{equation}{Vergel\ij{}king}{Vergel\ij{}kingen}%
        \crefname@preamble{figure}{Figuur}{Figuren}%
      \fi%
      \crefname@preamble{page}{Pagina}{Pagina's}%
      \crefname@preamble{table}{Tabel}{Tabellen}%
      \crefname@preamble{part}{Deel}{Delen}%
      \crefname@preamble{chapter}{Hoofdstuk}{Hoofdstukken}%
      \crefname@preamble{section}{Paragraaf}{Paragrafen}%
      \crefname@preamble{appendix}{Appendix}{Appendices}%
      \crefname@preamble{enumi}{Punt}{Punten}%
      \crefname@preamble{footnote}{Voetnote}{Voetnoten}%
      \crefname@preamble{theorem}{Theorema}{Theorema's}%
      \crefname@preamble{lemma}{Lemma}{Lemma's}%
      \crefname@preamble{corollary}{Corollarium}{Corollaria}%
      \crefname@preamble{proposition}{Bewering}{Beweringen}%
      \crefname@preamble{definition}{Definitie}{Definities}%
      \crefname@preamble{result}{Resultaat}{Resultaten}%
      \crefname@preamble{example}{Voorbeeld}{Voorbeelden}%
      \crefname@preamble{remark}{Opmerking}{Opmerkingen}%
      \crefname@preamble{note}{Aantekening}{Aantekeningen}%
      \crefname@preamble{algorithm}{Algoritme}{Algoritmen}%
      \crefname@preamble{listing}{Listing}{Listings}%
      \crefname@preamble{line}{Lijn}{Lijnen}%
 %
    \else%  capitalise unset
      \if@cref@abbrev%
        \crefname@preamble{equation}{verg.}{verg's.}%
        \crefname@preamble{figure}{fig.}{fig's.}%
      \else%
        \crefname@preamble{equation}{vergel\ij{}king}{vergel\ij{}kingen}%
        \crefname@preamble{figure}{figuur}{figuren}%
      \fi%
      \crefname@preamble{page}{pagina}{pagina's}%
      \crefname@preamble{table}{tabel}{tabellen}%
      \crefname@preamble{part}{deel}{delen}%
      \crefname@preamble{chapter}{hoofdstuk}{hoofdstukken}%
      \crefname@preamble{section}{paragraaf}{paragrafen}%
      \crefname@preamble{appendix}{appendix}{appendices}%
      \crefname@preamble{enumi}{punt}{punten}%
      \crefname@preamble{footnote}{voetnote}{voetnoten}%
      \crefname@preamble{theorem}{theorema}{theorema's}%
      \crefname@preamble{lemma}{lemma}{lemma's}%
      \crefname@preamble{corollary}{corollarium}{corollaria}%
      \crefname@preamble{proposition}{bewering}{beweringen}%
      \crefname@preamble{definition}{definitie}{definities}%
      \crefname@preamble{result}{resultaat}{resultaten}%
      \crefname@preamble{example}{voorbeeld}{voorbeelden}%
      \crefname@preamble{remark}{opmerking}{opmerkingen}%
      \crefname@preamble{note}{aantekening}{aantekeningen}%
      \crefname@preamble{algorithm}{algoritme}{algoritmen}%
      \crefname@preamble{listing}{listing}{listings}%
      \crefname@preamble{line}{lijn}{lijnen}%
    \fi%
    \def\cref@language{dutch}%
    \cref@addto\extrasdutch{%
      \renewcommand{\crefrangeconjunction}{ tot\nobreakspace}%
      \renewcommand\crefrangepreconjunction{}%
      \renewcommand\crefrangepostconjunction{}%
      \renewcommand{\crefpairconjunction}{ en\nobreakspace}%
      \renewcommand{\crefmiddleconjunction}{, }%
      \renewcommand{\creflastconjunction}{ en\nobreakspace}%
      \renewcommand{\crefpairgroupconjunction}{ en\nobreakspace}%
      \renewcommand{\crefmiddlegroupconjunction}{, }%
      \renewcommand{\creflastgroupconjunction}{ en\nobreakspace}%
 %
      \Crefname{equation}{Vergel\ij{}king}{Vergel\ij{}kingen}%
      \Crefname{figure}{Figuur}{Figuren}%
      \Crefname{subfigure}{Figuur}{Figuren}%
      \Crefname{table}{Tabel}{Tabellen}%
      \Crefname{subtable}{Tabel}{Tabellen}%
      \Crefname{page}{Pagina}{Pagina's}%
      \Crefname{part}{Deel}{Delen}%
      \Crefname{chapter}{Hoofdstuk}{Hoofdstuken}%
      \Crefname{section}{Paragraaf}{Paragrafen}%
      \Crefname{subsection}{Paragraaf}{Paragrafen}%
      \Crefname{subsubsection}{Paragraaf}{Paragrafen}%
      \Crefname{appendix}{Appendix}{Appendices}%
      \Crefname{subappendix}{Appendix}{Appendices}%
      \Crefname{subsubappendix}{Appendix}{Appendices}%
      \Crefname{subsubsubappendix}{Appendix}{Appendices}%
      \Crefname{enumi}{Punt}{Punten}%
      \Crefname{enumii}{Punt}{Punten}%
      \Crefname{enumiii}{Punt}{Punten}%
      \Crefname{enumiv}{Punt}{Punten}%
      \Crefname{enumv}{Punt}{Punten}%
      \Crefname{footnote}{Voetnote}{Voetnoten}%
      \Crefname{theorem}{Theorema}{Theorema's}%
      \Crefname{lemma}{Lemma}{Lemma's}%
      \Crefname{corollary}{Corollarium}{Corollaria}%
      \Crefname{proposition}{Bewering}{Beweringen}%
      \Crefname{definition}{Definitie}{Definities}%
      \Crefname{result}{Resultaat}{Resultaten}%
      \Crefname{example}{Voorbeeld}{Voorbeelden}%
      \Crefname{remark}{Opmerking}{Opmerkingen}%
      \Crefname{note}{Aantekening}{Aantekeningen}%
      \Crefname{algorithm}{Algoritme}{Algoritmen}%
      \Crefname{listing}{Listing}{Listings}%
      \Crefname{line}{Lijn}{Lijnen}%
 %
      \if@cref@capitalise%  capitalise set
        \if@cref@abbrev%
          \crefname{equation}{Verg.}{Verg's.}%
          \crefname{figure}{Fig.}{Fig's.}%
          \crefname{subfigure}{Fig.}{Fig's.}%
        \else%
          \crefname{equation}{Vergel\ij{}king}{Vergel\ij{}kingen}%
          \crefname{figure}{Figuur}{Figuren}%
          \crefname{subfigure}{Figuur}{Figuren}%
        \fi%
        \crefname{table}{Tabel}{Tabellen}%
        \crefname{subtable}{Tabel}{Tabellen}%
        \crefname{page}{Pagina}{Pagina's}%
        \crefname{part}{Deel}{Delen}%
        \crefname{chapter}{Hoofdstuk}{Hoofdstukken}%
        \crefname{section}{Paragraaf}{Paragrafen}%
        \crefname{appendix}{Appendix}{Appendices}%
        \crefname{enumi}{Punt}{Punten}%
        \crefname{footnote}{Voetnote}{Voetnoten}%
        \crefname{theorem}{Theorema}{Theorema's}%
        \crefname{lemma}{Lemma}{Lemma's}%
        \crefname{corollary}{Corollarium}{Corollaria}%
        \crefname{proposition}{Bewering}{Beweringen}%
        \crefname{definition}{Definitie}{Definities}%
        \crefname{result}{Resultaat}{Resultaten}%
        \crefname{example}{Voorbeeld}{Voorbeelden}%
        \crefname{remark}{Opmerking}{Opmerkingen}%
        \crefname{note}{Aantekening}{Aantekeningen}%
        \crefname{algorithm}{Algoritme}{Algoritmen}%
        \crefname{listing}{Listing}{Listings}%
        \crefname{line}{Lijn}{Lijnen}%
 %
      \else%  capitalise unset
        \if@cref@abbrev%
          \crefname{equation}{verg.}{verg's.}%
          \crefname{figure}{fig.}{fig's.}%
          \crefname{subfigure}{fig.}{fig's.}%
        \else%
          \crefname{equation}{vergel\ij{}king}{vergel\ij{}kingen}%
          \crefname{figure}{figuur}{figuren}%
          \crefname{subfigure}{figuur}{figuren}%
        \fi%
        \crefname{table}{tabel}{tabellen}%
        \crefname{subtable}{tabel}{tabellen}%
        \crefname{page}{pagina}{pagina's}%
        \crefname{part}{deel}{delen}%
        \crefname{chapter}{hoofdstuk}{hoofdstukken}%
        \crefname{section}{paragraaf}{paragrafen}%
        \crefname{appendix}{appendix}{appendices}%
        \crefname{enumi}{punt}{punten}%
        \crefname{footnote}{voetnote}{voetnoten}%
        \crefname{theorem}{theorema}{theorema's}%
        \crefname{lemma}{lemma}{lemma's}%
        \crefname{corollary}{corollarium}{corollaria}%
        \crefname{proposition}{bewering}{beweringen}%
        \crefname{definition}{definitie}{definities}%
        \crefname{result}{resultaat}{resultaten}%
        \crefname{example}{voorbeeld}{voorbeelden}%
        \crefname{remark}{opmerking}{opmerkingen}%
        \crefname{note}{aantekening}{aantekeningen}%
        \crefname{algorithm}{algoritme}{algoritmen}%
        \crefname{listing}{listing}{listings}%
        \crefname{line}{lijn}{lijnen}%
      \fi%
    }}}
\DeclareOption{french}{%
  \PackageInfo{cleveref}{loaded `french' language definitions}
  \AtBeginDocument{%
    \def\crefrangeconjunction@preamble{ \`a\nobreakspace}%
    \def\crefrangepreconjunction@preamble{}%
    \def\crefrangepostconjunction@preamble{}%
    \def\crefpairconjunction@preamble{ et\nobreakspace}%
    \def\crefmiddleconjunction@preamble{, }%
    \def\creflastconjunction@preamble{ et\nobreakspace}%
    \def\crefpairgroupconjunction@preamble{ et\nobreakspace}%
    \def\crefmiddlegroupconjunction@preamble{, }%
    \def\creflastgroupconjunction@preamble{, et\nobreakspace}%
 %
    \Crefname@preamble{equation}{{\'E}quation}{{\'E}quations}%
    \Crefname@preamble{figure}{Figure}{Figures}%
    \Crefname@preamble{table}{Tableau}{Tableaux}%
    \Crefname@preamble{page}{Page}{Pages}%
    \Crefname@preamble{part}{Partie}{Parties}%
    \Crefname@preamble{chapter}{Chapitre}{Chapitres}%
    \Crefname@preamble{section}{Section}{Sections}%
    \Crefname@preamble{appendix}{Annexe}{Annexes}%
    \Crefname@preamble{enumi}{Point}{Points}%
    \Crefname@preamble{footnote}{Note}{Notes}%
    \Crefname@preamble{theorem}{Th\'eor\`eme}{Th\'eor\`emes}%
    \Crefname@preamble{lemma}{Lemme}{Lemmes}%
    \Crefname@preamble{corollary}{Corollaire}{Corollaires}%
    \Crefname@preamble{proposition}{Proposition}{Propositions}%
    \Crefname@preamble{definition}{D\'efinition}{D\'efinitions}%
    \Crefname@preamble{result}{R\'esultat}{R\'esultats}%
    \Crefname@preamble{example}{Exemple}{Exemples}%
    \Crefname@preamble{remark}{Remarque}{Remarques}%
    \Crefname@preamble{algorithm}{Algorithme}{Algorithmes}%
    \Crefname@preamble{listing}{Liste}{Listes}%
    \Crefname@preamble{line}{Ligne}{Lignes}%
 %
    \if@cref@capitalise%  capitalise set
      \crefname@preamble{equation}{{\'E}quation}{{\'E}quations}%
      \crefname@preamble{figure}{Figure}{Figures}%
      \crefname@preamble{table}{Tableau}{Tableaux}%
      \crefname@preamble{page}{Page}{Pages}%
      \crefname@preamble{part}{Partie}{Parties}%
      \crefname@preamble{chapter}{Chapitre}{Chapitres}%
      \crefname@preamble{section}{Section}{Sections}%
      \crefname@preamble{appendix}{Annexe}{Annexes}%
      \crefname@preamble{enumi}{Point}{Points}%
      \crefname@preamble{footnote}{Note}{Notes}%
      \crefname@preamble{theorem}{Th\'eor\`eme}{Th\'eor\`emes}%
      \crefname@preamble{lemma}{Lemme}{Lemmes}%
      \crefname@preamble{corollary}{Corollaire}{Corollaires}%
      \crefname@preamble{proposition}{Proposition}{Propositions}%
      \crefname@preamble{definition}{D\'efinition}{D\'efinitions}%
      \crefname@preamble{result}{R\'esultat}{R\'esultats}%
      \crefname@preamble{example}{Exemple}{Exemples}%
      \crefname@preamble{remark}{Remarque}{Remarques}%
      \crefname@preamble{note}{Commentaire}{Commentaires}%
      \crefname@preamble{algorithm}{Algorithme}{Algorithmes}%
      \crefname@preamble{listing}{Liste}{Listes}%
      \crefname@preamble{line}{Ligne}{Lignes}%
 %
    \else%  capitalise unset
      \crefname@preamble{equation}{{\'e}quation}{{\'e}quations}%
      \crefname@preamble{figure}{figure}{figures}%
      \crefname@preamble{table}{tableau}{tableaux}%
      \crefname@preamble{page}{page}{pages}%
      \crefname@preamble{part}{partie}{parties}%
      \crefname@preamble{chapter}{chapitre}{chapitres}%
      \crefname@preamble{section}{section}{sections}%
      \crefname@preamble{appendix}{annexe}{annexes}%
      \crefname@preamble{enumi}{point}{points}%
      \crefname@preamble{footnote}{note}{notes}%
      \crefname@preamble{theorem}{th\'eor\`eme}{th\'eor\`emes}%
      \crefname@preamble{lemma}{lemme}{lemmes}%
      \crefname@preamble{corollary}{corollaire}{corollaires}%
      \crefname@preamble{proposition}{proposition}{propositions}%
      \crefname@preamble{definition}{d\'efinition}{d\'efinitions}%
      \crefname@preamble{result}{r\'esultat}{r\'esultats}%
      \crefname@preamble{example}{exemple}{exemples}%
      \crefname@preamble{remark}{remarque}{remarques}%
      \crefname@preamble{note}{commentaire}{commentaires}%
      \crefname@preamble{algorithm}{algorithme}{algorithmes}%
      \crefname@preamble{listing}{liste}{listes}%
      \crefname@preamble{line}{ligne}{lignes}%
    \fi%
    \def\cref@language{french}%
    \cref@addto\extrasfrench{%
      \renewcommand{\crefrangeconjunction}{ \`a\nobreakspace}%
      \renewcommand\crefrangepreconjunction{}%
      \renewcommand\crefrangepostconjunction{}%
      \renewcommand{\crefpairconjunction}{ et\nobreakspace}%
      \renewcommand{\crefmiddleconjunction}{, }%
      \renewcommand{\creflastconjunction}{ et\nobreakspace}%
      \renewcommand{\crefpairgroupconjunction}{ et\nobreakspace}%
      \renewcommand{\crefmiddlegroupconjunction}{, }%
      \renewcommand{\creflastgroupconjunction}{ et\nobreakspace}%
 %
      \Crefname{equation}{{\'E}quation}{{\'E}quations}%
      \Crefname{figure}{Figure}{Figures}%
      \Crefname{subfigure}{Figure}{Figures}%
      \Crefname{table}{Tableau}{Tableaux}%
      \Crefname{subtable}{Tableau}{Tableaux}%
      \Crefname{page}{Page}{Pages}%
      \Crefname{part}{Partie}{Parties}%
      \Crefname{chapter}{Chapitre}{Chapitres}%
      \Crefname{section}{Section}{Sections}%
      \Crefname{subsection}{Section}{Sections}%
      \Crefname{subsubsection}{Section}{Sections}%
      \Crefname{appendix}{Annexe}{Annexes}%
      \Crefname{subappendix}{Annexe}{Annexes}%
      \Crefname{subsubappendix}{Annexe}{Annexes}%
      \Crefname{subsubsubappendix}{Annexe}{Annexes}%
      \Crefname{enumi}{Point}{Points}%
      \Crefname{enumii}{Point}{Points}%
      \Crefname{enumiii}{Point}{Points}%
      \Crefname{enumiv}{Point}{Points}%
      \Crefname{enumv}{Point}{Points}%
      \Crefname{footnote}{Note}{Notes}%
      \Crefname{theorem}{Th\'eor\`eme}{Th\'eor\`emes}%
      \Crefname{lemma}{Lemme}{Lemmes}%
      \Crefname{corollary}{Corollaire}{Corollaires}%
      \Crefname{proposition}{Proposition}{Propositions}%
      \Crefname{definition}{D\'efinition}{D\'efinitions}%
      \Crefname{result}{R\'esultat}{R\'esultats}%
      \Crefname{example}{Exemple}{Exemples}%
      \Crefname{remark}{Remarque}{Remarques}%
      \Crefname{note}{Commentaire}{Commentaires}%
      \Crefname{algorithm}{Algorithme}{Algorithmes}%
      \Crefname{listing}{Liste}{Listes}%
      \Crefname{line}{Ligne}{Lignes}%
 %
      \if@cref@capitalise%  capitalise set
        \crefname{equation}{{\'E}quation}{{\'E}quations}%
        \crefname{figure}{Figure}{Figures}%
        \crefname{subfigure}{Figure}{Figures}%
        \crefname{table}{Tableau}{Tableaux}%
        \crefname{subtable}{Tableau}{Tableaux}%
        \crefname{page}{Page}{Pages}%
        \crefname{part}{Partie}{Parties}%
        \crefname{chapter}{Chapitre}{Chapitres}%
        \crefname{section}{Section}{Sections}%
        \crefname{subsection}{Section}{Sections}%
        \crefname{subsubsection}{Section}{Sections}%
        \crefname{appendix}{Annexe}{Annexes}%
        \crefname{subappendix}{Annexe}{Annexes}%
        \crefname{subsubappendix}{Annexe}{Annexes}%
        \crefname{subsubsubappendix}{Annexe}{Annexes}%
        \crefname{enumi}{Point}{Points}%
        \crefname{enumii}{Point}{Points}%
        \crefname{enumiii}{Point}{Points}%
        \crefname{enumiv}{Point}{Points}%
        \crefname{enumv}{Point}{Points}%
        \crefname{footnote}{Note}{Notes}%
        \crefname{theorem}{Th\'eor\`eme}{Th\'eor\`emes}%
        \crefname{lemma}{Lemme}{Lemmes}%
        \crefname{corollary}{Corollaire}{Corollaires}%
        \crefname{proposition}{Proposition}{Propositions}%
        \crefname{definition}{D\'efinition}{D\'efinitions}%
        \crefname{result}{R\'esultat}{R\'esultats}%
        \crefname{example}{Exemple}{Exemples}%
        \crefname{remark}{Remarque}{Remarques}%
        \crefname{note}{Commentaire}{Commentaires}%
        \crefname{algorithm}{Algorithme}{Algorithmes}%
        \crefname{listing}{Liste}{Listes}%
        \crefname{line}{Ligne}{Lignes}%
 %
      \else%  capitalise unset
        \crefname{equation}{{\'e}quation}{{\'e}quations}%
        \crefname{figure}{figure}{figures}%
        \crefname{subfigure}{figure}{figures}%
        \crefname{table}{tableau}{tableaux}%
        \crefname{subtable}{tableau}{tableaux}%
        \crefname{page}{page}{pages}%
        \crefname{part}{partie}{parties}%
        \crefname{chapter}{chapitre}{chapitres}%
        \crefname{section}{section}{sections}%
        \crefname{subsection}{section}{sections}%
        \crefname{subsubsection}{section}{sections}%
        \crefname{appendix}{annexe}{annexes}%
        \crefname{subappendix}{annexe}{annexes}%
        \crefname{subsubappendix}{annexe}{annexes}%
        \crefname{subsubsubappendix}{annexe}{annexes}%
        \crefname{enumi}{point}{points}%
        \crefname{enumii}{point}{points}%
        \crefname{enumiii}{point}{points}%
        \crefname{enumiv}{point}{points}%
        \crefname{enumv}{point}{points}%
        \crefname{footnote}{note}{notes}%
        \crefname{theorem}{th\'eor\`eme}{th\'eor\`emes}%
        \crefname{lemma}{lemme}{lemmes}%
        \crefname{corollary}{corollaire}{corollaires}%
        \crefname{proposition}{proposition}{propositions}%
        \crefname{definition}{d\'efinition}{d\'efinitions}%
        \crefname{result}{r\'esultat}{r\'esultats}%
        \crefname{example}{exemple}{exemples}%
        \crefname{remark}{remarque}{remarques}%
        \crefname{note}{commentaire}{commentaires}%
        \crefname{algorithm}{algorithme}{algorithmes}%
        \crefname{listing}{liste}{listes}%
        \crefname{line}{ligne}{lignes}%
      \fi%
    }}}
\DeclareOption{spanish}{%
  \PackageInfo{cleveref}{loaded `spanish' language definitions}
  \AtBeginDocument{%
    \def\crefrangeconjunction@preamble{ a\nobreakspace}%
    \def\crefrangepreconjunction@preamble{}%
    \def\crefrangepostconjunction@preamble{}%
    \def\crefpairconjunction@preamble{ y\nobreakspace}%
    \def\crefmiddleconjunction@preamble{, }%
    \def\creflastconjunction@preamble{ y\nobreakspace}%
    \def\crefpairgroupconjunction@preamble{ y\nobreakspace}%
    \def\crefmiddlegroupconjunction@preamble{, }%
    \def\creflastgroupconjunction@preamble{ y\nobreakspace}%
 %
    \Crefname@preamble{equation}{Ecuaci\'on}{Ecuaciones}%
    \Crefname@preamble{figure}{Figura}{Figuras}%
    \Crefname@preamble{table}{Cuadro}{Cuadros}%
    \Crefname@preamble{page}{P\'agina}{P\'aginas}%
    \Crefname@preamble{part}{Parte}{Partes}%
    \Crefname@preamble{chapter}{Cap\'itulo}{Cap\'itulos}%
    \Crefname@preamble{section}{Apartado}{Apartados}%
    \Crefname@preamble{appendix}{Ap\'endice}{Ap\'endices}%
    \Crefname@preamble{enumi}{Punto}{Puntos}%
    \Crefname@preamble{footnote}{Nota}{Notas}%
    \Crefname@preamble{theorem}{Teorema}{Teoremas}%
    \Crefname@preamble{lemma}{Lema}{Lemas}%
    \Crefname@preamble{corollary}{Corolario}{Corolarios}%
    \Crefname@preamble{proposition}{Proposici\'on}{Proposiciones}%
    \Crefname@preamble{definition}{Definici\'on}{Definiciones}%
    \Crefname@preamble{result}{Resultado}{Resultados}%
    \Crefname@preamble{example}{Ejemplo}{Ejemplos}%
    \Crefname@preamble{remark}{Observaci\'on}{Observaciones}%
    \Crefname@preamble{note}{Nota}{Notas}%
    \Crefname@preamble{algorithm}{Algoritmo}{Algoritmos}%
    \Crefname@preamble{listing}{Listado}{Listados}%
    \Crefname@preamble{line}{L\'inea}{L\'ineas}%
 %
    \if@cref@capitalise%  capitalise set
      \crefname@preamble{equation}{Ecuaci\'on}{Ecuaciones}%
      \crefname@preamble{figure}{Figura}{Figuras}%
      \crefname@preamble{table}{Cuadro}{Cuadros}%
      \crefname@preamble{page}{P\'agina}{P\'aginas}%
      \crefname@preamble{part}{Parte}{Partes}%
      \crefname@preamble{chapter}{Cap\'itulo}{Cap\'itulos}%
      \crefname@preamble{section}{Apartado}{Apartados}%
      \crefname@preamble{appendix}{Ap\'endice}{Ap\'endices}%
      \crefname@preamble{enumi}{Punto}{Puntos}%
      \crefname@preamble{footnote}{Nota}{Notas}%
      \crefname@preamble{theorem}{Teorema}{Teoremas}%
      \crefname@preamble{lemma}{Lema}{Lemas}%
      \crefname@preamble{corollary}{Corolario}{Corolarios}%
      \crefname@preamble{proposition}{Proposici\'on}{Proposiciones}%
      \crefname@preamble{definition}{Definici\'on}{Definiciones}%
      \crefname@preamble{result}{Resultado}{Resultados}%
      \crefname@preamble{example}{Ejemplo}{Ejemplos}%
      \crefname@preamble{remark}{Observaci\'on}{Observaciones}%
      \crefname@preamble{note}{Nota}{Notas}%
      \crefname@preamble{algorithm}{Algoritmo}{Algoritmos}%
      \crefname@preamble{listing}{Listado}{Listados}%
      \crefname@preamble{line}{L\'inea}{L\'ineas}%
 %
    \else%  capitalise unset
      \crefname@preamble{equation}{ecuaci\'on}{ecuaciones}%
      \crefname@preamble{figure}{figura}{figuras}%
      \crefname@preamble{table}{cuadro}{cuadros}%
      \crefname@preamble{page}{p\'agina}{p\'aginas}%
      \crefname@preamble{part}{parte}{partes}%
      \crefname@preamble{chapter}{cap\'itulo}{cap\'itulos}%
      \crefname@preamble{section}{apartado}{apartados}%
      \crefname@preamble{appendix}{ap\'endice}{ap\'endices}%
      \crefname@preamble{enumi}{punto}{puntos}%
      \crefname@preamble{footnote}{nota}{notas}%
      \crefname@preamble{theorem}{teorema}{teoremas}%
      \crefname@preamble{lemma}{lema}{lemas}%
      \crefname@preamble{corollary}{corolario}{corolarios}%
      \crefname@preamble{proposition}{proposici\'on}{proposiciones}%
      \crefname@preamble{definition}{definici\'on}{definiciones}%
      \crefname@preamble{result}{resultado}{resultados}%
      \crefname@preamble{example}{ejemplo}{ejemplos}%
      \crefname@preamble{remark}{observaci\'on}{observaciones}%
      \crefname@preamble{note}{nota}{notas}%
      \crefname@preamble{algorithm}{algoritmo}{algoritmos}%
      \crefname@preamble{listing}{listado}{listados}%
      \crefname@preamble{line}{l\'inea}{l\'ineas}%
    \fi%
    \def\cref@language{spanish}%
    \cref@addto\extrasspanish{%
      \renewcommand{\crefrangeconjunction}{ a\nobreakspace}%
      \renewcommand{\crefrangepreconjunction}{}%
      \renewcommand{\crefrangepostconjunction}{}%
      \renewcommand{\crefpairconjunction}{ y\nobreakspace}%
      \renewcommand{\crefmiddleconjunction}{, }%
      \renewcommand{\creflastconjunction}{ y\nobreakspace}%
      \renewcommand{\crefpairgroupconjunction}{ y\nobreakspace}%
      \renewcommand{\crefmiddlegroupconjunction}{, }%
      \renewcommand{\creflastgroupconjunction}{ y\nobreakspace}%
 %
      \Crefname{equation}{Ecuaci\'on}{Ecuaciones}%
      \Crefname{figure}{Figura}{Figuras}%
      \Crefname{subfigure}{Figura}{Figuras}%
      \Crefname{table}{Cuadro}{Cuadros}%
      \Crefname{subtable}{Cuadro}{Cuadros}%
      \Crefname{page}{P\'agina}{P\'aginas}%
      \Crefname{part}{Parte}{Partes}%
      \Crefname{chapter}{Cap\'itulo}{Cap\'itulos}%
      \Crefname{section}{Apartado}{Apartados}%
      \Crefname{subsection}{Apartado}{Apartados}%
      \Crefname{subsubsection}{Apartado}{Apartados}%
      \Crefname{appendix}{Ap\'endice}{Ap\'endices}%
      \Crefname{subappendix}{Ap\'endice}{Ap\'endices}%
      \Crefname{subsubappendix}{Ap\'endice}{Ap\'endices}%
      \Crefname{subsubsubappendix}{Ap\'endice}{Ap\'endices}%
      \Crefname{enumi}{Punto}{Puntos}%
      \Crefname{enumii}{Punto}{Puntos}%
      \Crefname{enumiii}{Punto}{Puntos}%
      \Crefname{enumiv}{Punto}{Puntos}%
      \Crefname{enumv}{Punto}{Puntos}%
      \Crefname{footnote}{Nota}{Notas}%
      \Crefname{theorem}{Teorema}{Teoremas}%
      \Crefname{lemma}{Lema}{Lemas}%
      \Crefname{corollary}{Corolario}{Corolarios}%
      \Crefname{proposition}{Proposici\'on}{Proposiciones}%
      \Crefname{definition}{Definici\'on}{Definiciones}%
      \Crefname{result}{Resultado}{Resultados}%
      \Crefname{example}{Ejemplo}{Ejemplos}%
      \Crefname{remark}{Observaci\'on}{Observaci\'on}%
      \Crefname{note}{Nota}{Notas}%
      \Crefname{algorithm}{Algoritmo}{Algoritmos}%
      \Crefname{listing}{Listado}{Listados}%
      \Crefname{line}{L\'inea}{L\'ineas}%
 %
      \if@cref@capitalise%  capitalise set
        \crefname{equation}{Ecuaci\'on}{Ecuaciones}%
        \crefname{figure}{Figura}{Figuras}%
        \crefname{subfigure}{Figura}{Figuras}%
        \crefname{table}{Cuadro}{Cuadros}%
        \crefname{subtable}{Cuadro}{Cuadros}%
        \crefname{page}{P\'agina}{P\'aginas}%
        \crefname{part}{Parte}{Partes}%
        \crefname{chapter}{Cap\'itulo}{Cap\'itulos}%
        \crefname{section}{Apartado}{Apartados}%
        \crefname{subsection}{Apartado}{Apartados}%
        \crefname{subsubsection}{Apartado}{Apartados}%
        \crefname{appendix}{Ap\'endice}{Ap\'endices}%
        \crefname{subappendix}{Ap\'endice}{Ap\'endices}%
        \crefname{subsubappendix}{Ap\'endice}{Ap\'endices}%
        \crefname{subsubsubappendix}{Ap\'endice}{Ap\'endices}%
        \crefname{enumi}{Punto}{Puntos}%
        \crefname{enumii}{Punto}{Puntos}%
        \crefname{enumiii}{Punto}{Puntos}%
        \crefname{enumiv}{Punto}{Puntos}%
        \crefname{enumv}{Punto}{Puntos}%
        \crefname{footnote}{Nota}{Notas}%
        \crefname{theorem}{Teorema}{Teoremas}%
        \crefname{lemma}{Lema}{Lemas}%
        \crefname{corollary}{Corolario}{Corolarios}%
        \crefname{proposition}{Proposici\'on}{Proposiciones}%
        \crefname{definition}{Definici\'on}{Definiciones}%
        \crefname{result}{Resultado}{Resultados}%
        \crefname{example}{Ejemplo}{Ejemplos}%
        \crefname{remark}{Observaci\'on}{Observaci\'ones}%
        \crefname{note}{Nota}{Notas}%
        \crefname{algorithm}{Algoritmo}{Algoritmos}%
        \crefname{listing}{Listado}{Listados}%
        \crefname{line}{L\'inea}{L\'ineas}%
 %
      \else%  capitalise unset
        \crefname{equation}{ecuaci\'on}{ecuaciones}%
        \crefname{figure}{figura}{figuras}%
        \crefname{subfigure}{figura}{figuras}%
        \crefname{table}{cuadro}{cuadros}%
        \crefname{subtable}{cuadro}{cuadros}%
        \crefname{page}{p\'agina}{p\'aginas}%
        \crefname{part}{parte}{partes}%
        \crefname{chapter}{cap\'itulo}{cap\'itulos}%
        \crefname{section}{apartado}{apartados}%
        \crefname{subsection}{apartado}{apartados}%
        \crefname{subsubsection}{apartado}{apartados}%
        \crefname{appendix}{ap\'endice}{ap\'endices}%
        \crefname{subappendix}{ap\'endice}{ap\'endices}%
        \crefname{subsubappendix}{ap\'endice}{ap\'endices}%
        \crefname{subsubsubappendix}{ap\'endice}{ap\'endices}%
        \crefname{enumi}{punto}{puntos}%
        \crefname{enumii}{punto}{puntos}%
        \crefname{enumiii}{punto}{puntos}%
        \crefname{enumiv}{punto}{puntos}%
        \crefname{enumv}{punto}{puntos}%
        \crefname{footnote}{nota}{notas}%
        \crefname{theorem}{teorema}{teoremas}%
        \crefname{lemma}{lema}{lemas}%
        \crefname{corollary}{corolario}{corolarios}%
        \crefname{proposition}{proposici\'on}{proposiciones}%
        \crefname{definition}{definici\'on}{definiciones}%
        \crefname{result}{resultado}{resultados}%
        \crefname{example}{ejemplo}{ejemplos}%
        \crefname{remark}{observaci\'on}{observaci\'ones}%
        \crefname{note}{nota}{notas}%
        \crefname{algorithm}{algoritmo}{algoritmos}%
        \crefname{listing}{listado}{listados}%
        \crefname{line}{l\'inea}{l\'ineas}%
      \fi%
    }}}
\DeclareOption{italian}{%
  \PackageInfo{cleveref}{loaded `italian' language definitions}
  \AtBeginDocument{%
    \def\crefrangeconjunction@preamble{ a\nobreakspace}%
    \def\crefrangepreconjunction@preamble{da\nobreakspace}%
    \def\crefrangepostconjunction@preamble{}%
    \def\crefpairconjunction@preamble{ e\nobreakspace}%
    \def\crefmiddleconjunction@preamble{, }%
    \def\creflastconjunction@preamble{ e\nobreakspace}%
    \def\crefpairgroupconjunction@preamble{ e\nobreakspace}%
    \def\crefmiddlegroupconjunction@preamble{, }%
    \def\creflastgroupconjunction@preamble{ e\nobreakspace}%
 %
    \Crefname@preamble{equation}{Equazione}{Equazioni}%
    \Crefname@preamble{figure}{Figura}{Figure}%
    \Crefname@preamble{table}{Tabella}{Tabelle}%
    \Crefname@preamble{page}{Pagina}{Pagine}%
    \Crefname@preamble{part}{Parte}{Parti}%
    \Crefname@preamble{chapter}{Capitolo}{Capitoli}%
    \Crefname@preamble{section}{Sezione}{Sezioni}%
    \Crefname@preamble{appendix}{Appendice}{Appendici}%
    \Crefname@preamble{enumi}{Voce}{Voci}%
    \Crefname@preamble{footnote}{Nota}{Note}%
    \Crefname@preamble{theorem}{Teorema}{Teoremi}%
    \Crefname@preamble{lemma}{Lemma}{Lemmi}%
    \Crefname@preamble{corollary}{Corollario}{Corollari}%
    \Crefname@preamble{proposition}{Proposizione}{Proposizioni}%
    \Crefname@preamble{definition}{Definizioni}{Definizioni}%
    \Crefname@preamble{result}{Risultato}{Risultati}%
    \Crefname@preamble{example}{esempio}{esempi}%
    \Crefname@preamble{remark}{Osservazione}{Osservazioni}%
    \Crefname@preamble{note}{Nota}{Note}%
    \Crefname@preamble{algorithm}{Algoritmo}{Algoritmi}%
    \Crefname@preamble{listing}{Elenco}{Elenchi}%
    \Crefname@preamble{line}{Linea}{Linee}%
 %
    \if@cref@capitalise%  capitalise set
      \if@cref@abbrev%
        \crefname@preamble{equation}{Eq.}{Eq.}%
        \crefname@preamble{figure}{Fig.}{Fig.}%
      \else%
        \crefname@preamble{equation}{Equazione}{Equazioni}%
        \crefname@preamble{figure}{Figura}{Figure}%
      \fi%
      \crefname@preamble{table}{Tabella}{Tabelle}%
      \crefname@preamble{page}{Pagina}{Pagine}%
      \crefname@preamble{part}{Parte}{Parti}%
      \crefname@preamble{chapter}{Capitolo}{Capitoli}%
      \crefname@preamble{section}{Sezione}{Sezioni}%
      \crefname@preamble{appendix}{Appendice}{Appendici}%
      \crefname@preamble{enumi}{Voce}{Voci}%
      \crefname@preamble{footnote}{Nota}{Note}%
      \crefname@preamble{theorem}{Teorema}{Teoremi}%
      \crefname@preamble{lemma}{Lemma}{Lemmi}%
      \crefname@preamble{corollary}{Corollario}{Corollari}%
      \crefname@preamble{proposition}{Proposizione}{Proposizioni}%
      \crefname@preamble{definition}{Definizione}{Definizioni}%
      \crefname@preamble{result}{Risultato}{Risultati}%
      \crefname@preamble{example}{Esempio}{Esempi}%
      \crefname@preamble{remark}{Osservazione}{Osservazioni}%
      \crefname@preamble{note}{Nota}{Note}%
      \crefname@preamble{algorithm}{Algoritmo}{Algoritmi}%
      \crefname@preamble{listing}{Elenco}{Elenchi}%
      \crefname@preamble{line}{Linea}{Linee}%
 %
    \else%  capitalise unset
      \if@cref@abbrev%
        \crefname@preamble{equation}{eq.}{eq.}%
        \crefname@preamble{figure}{fig.}{fig.}%
      \else%
        \crefname@preamble{equation}{equazione}{equazioni}%
        \crefname@preamble{figure}{figura}{figure}%
      \fi%
      \crefname@preamble{table}{tabella}{tabelle}%
      \crefname@preamble{page}{pagina}{pagine}%
      \crefname@preamble{part}{parte}{parti}%
      \crefname@preamble{chapter}{capitolo}{capitoli}%
      \crefname@preamble{section}{sezione}{sezioni}%
      \crefname@preamble{appendix}{appendice}{appendici}%
      \crefname@preamble{enumi}{voce}{voci}%
      \crefname@preamble{footnote}{nota}{note}%
      \crefname@preamble{theorem}{teorema}{teoremi}%
      \crefname@preamble{lemma}{lemma}{lemmi}%
      \crefname@preamble{corollary}{corollario}{corollari}%
      \crefname@preamble{proposition}{proposizione}{proposizioni}%
      \crefname@preamble{definition}{definizione}{definizioni}%
      \crefname@preamble{result}{risultato}{risultati}%
      \crefname@preamble{example}{esempio}{esempi}%
      \crefname@preamble{remark}{osservazione}{osservazioni}%
      \crefname@preamble{note}{nota}{note}%
      \crefname@preamble{algorithm}{algoritmo}{algoritmi}%
      \crefname@preamble{listing}{elenco}{elenchi}%
      \crefname@preamble{line}{linea}{linee}%
    \fi%
    \def\cref@language{italian}%
    \cref@addto\extrasitalian{%
      \renewcommand{\crefrangeconjunction}{ a\nobreakspace}%
      \renewcommand\crefrangepreconjunction{da\nobreakspace}%
      \renewcommand\crefrangepostconjunction{}%
      \renewcommand{\crefpairconjunction}{ e\nobreakspace}%
      \renewcommand{\crefmiddleconjunction}{, }%
      \renewcommand{\creflastconjunction}{ e\nobreakspace}%
      \renewcommand{\crefpairgroupconjunction}{ e\nobreakspace}%
      \renewcommand{\crefmiddlegroupconjunction}{, }%
      \renewcommand{\creflastgroupconjunction}{ e\nobreakspace}%
 %
      \Crefname{equation}{Equazione}{Equazioni}%
      \Crefname{figure}{Figura}{Figure}%
      \Crefname{subfigure}{Figura}{Figure}%
      \Crefname{table}{Tabella}{Tabelle}%
      \Crefname{subtable}{Tabella}{Tabelle}%
      \Crefname{page}{Pagina}{Pagine}%
      \Crefname{part}{Parte}{Parti}%
      \Crefname{chapter}{Capitolo}{Capitoli}%
      \Crefname{section}{Sezione}{Sezioni}%
      \Crefname{subsection}{Sezione}{Sezioni}%
      \Crefname{subsubsection}{Sezione}{Sezioni}%
      \Crefname{appendix}{Appendice}{Appendici}%
      \Crefname{subappendix}{Appendice}{Appendici}%
      \Crefname{subsubappendix}{Appendice}{Appendici}%
      \Crefname{subsubsubappendix}{Appendice}{Appendici}%
      \Crefname{enumi}{Voce}{Voci}%
      \Crefname{enumii}{Voce}{Voci}%
      \Crefname{enumiii}{Voce}{Voci}%
      \Crefname{enumiv}{Voce}{Voci}%
      \Crefname{enumv}{Voce}{Voci}%
      \Crefname{footnote}{Nota}{Note}%
      \Crefname{theorem}{Teorema}{Teoremi}%
      \Crefname{lemma}{Lemma}{Lemmi}%
      \Crefname{corollary}{Corollario}{Corollari}%
      \Crefname{proposition}{Proposizione}{Proposizioni}%
      \Crefname{definition}{Definizione}{Definizione}%
      \Crefname{result}{Risultato}{Risultati}%
      \Crefname{example}{esempio}{esempi}%
      \Crefname{remark}{Osservazione}{Osservazioni}%
      \Crefname{note}{Nota}{Note}%
      \Crefname{algorithm}{Algoritmo}{Algoritmi}%
      \Crefname{listing}{Elenco}{Elenchi}%
      \Crefname{line}{Linea}{Linee}%
 %
      \if@cref@capitalise%  capitalise set
        \if@cref@abbrev%
          \crefname{equation}{Eq.}{Eq.}%
          \crefname{figure}{Fig.}{Fig.}%
          \crefname{subfigure}{Fig.}{Fig.}%
        \else%
          \crefname{equation}{Equazione}{Equazioni}%
          \crefname{figure}{Figura}{Figure}%
          \crefname{figure}{Figura}{Figure}%
        \fi%
        \crefname{table}{Tabella}{Tabelle}%
        \crefname{page}{Pagina}{Pagine}%
        \crefname{subtable}{Tabella}{Tabelle}%
        \crefname{part}{Parte}{Parti}%
        \crefname{chapter}{Capitolo}{Capitoli}%
        \crefname{section}{Sezione}{Sezioni}%
        \crefname{subsection}{Sezione}{Sezioni}%
        \crefname{subsubsection}{Sezione}{Sezioni}%
        \crefname{appendix}{Appendice}{Appendici}%
        \crefname{subappendix}{Appendice}{Appendici}%
        \crefname{subsubappendix}{Appendice}{Appendici}%
        \crefname{subsubsubappendix}{Appendice}{Appendici}%
        \crefname{enumi}{Voce}{Voci}%
        \crefname{enumii}{Voce}{Voci}%
        \crefname{enumiii}{Voce}{Voci}%
        \crefname{enumiv}{Voce}{Voci}%
        \crefname{enumv}{Voce}{Voci}%
        \crefname{footnote}{Nota}{Note}%
        \crefname{theorem}{Teorema}{Teoremi}%
        \crefname{lemma}{Lemma}{Lemmi}%
        \crefname{corollary}{Corollario}{Corollari}%
        \crefname{proposition}{Proposizione}{Proposizioni}%
        \crefname{definition}{Definizione}{Definizione}%
        \crefname{result}{Risultato}{Risultati}%
        \crefname{example}{Esempio}{Esempi}%
        \crefname{remark}{Osservazione}{Osservazioni}%
        \crefname{note}{Nota}{Note}%
        \crefname{algorithm}{Algoritmo}{Algoritmi}%
        \crefname{listing}{Elenco}{Elenchi}%
        \crefname{line}{Linea}{Linee}%
 %
      \else%  capitalise unset
        \if@cref@abbrev%
          \crefname{equation}{eq.}{eq.}%
          \crefname{figure}{fig.}{fig.}%
          \crefname{subfigure}{fig.}{fig.}%
        \else%
          \crefname{equation}{equazione}{equazioni}%
          \crefname{figure}{figura}{figure}%
          \crefname{figure}{figura}{figure}%
        \fi%
        \crefname{table}{tabella}{tabelle}%
        \crefname{page}{pagina}{pagine}%
        \crefname{subtable}{tabella}{tabelle}%
        \crefname{part}{parte}{parti}%
        \crefname{chapter}{capitolo}{capitoli}%
        \crefname{section}{sezione}{sezioni}%
        \crefname{subsection}{sezione}{sezioni}%
        \crefname{subsubsection}{sezione}{sezioni}%
        \crefname{appendix}{appendice}{appendici}%
        \crefname{subappendix}{appendice}{appendici}%
        \crefname{subsubappendix}{appendice}{appendici}%
        \crefname{subsubsubappendix}{appendice}{appendici}%
        \crefname{enumi}{voce}{voci}%
        \crefname{enumii}{voce}{voci}%
        \crefname{enumiii}{voce}{voci}%
        \crefname{enumiv}{voce}{voci}%
        \crefname{enumv}{voce}{voci}%
        \crefname{footnote}{nota}{note}%
        \crefname{theorem}{teorema}{teoremi}%
        \crefname{lemma}{lemma}{lemmi}%
        \crefname{corollary}{corollario}{corollari}%
        \crefname{proposition}{proposizione}{proposizioni}%
        \crefname{definition}{definizione}{definizione}%
        \crefname{result}{risultato}{risultati}%
        \crefname{example}{esempio}{esempi}%
        \crefname{remark}{osservazione}{osservazioni}%
        \crefname{note}{nota}{note}%
        \crefname{algorithm}{algoritmo}{algoritmi}%
        \crefname{listing}{elenco}{elenchi}%
        \crefname{line}{linea}{linee}%
      \fi%
    }}}
\DeclareOption{russian}{%
  \PackageInfo{cleveref}{loaded `russian' language definitions}
  \AtBeginDocument{%
    \def\crefrangeconjunction@preamble{--}%
    \def\crefrangepreconjunction@preamble{}%
    \def\crefrangepostconjunction@preamble{}%
    \def\crefpairconjunction@preamble{ \cyri\nobreakspace}%
    \def\crefmiddleconjunction@preamble{, }%
    \def\creflastconjunction@preamble{ \cyri\nobreakspace}%
    \def\crefpairgroupconjunction@preamble{ \cyri\nobreakspace}%
    \def\crefmiddlegroupconjunction@preamble{, }%
    \def\creflastgroupconjunction@preamble%
      {, \cyra\ \cyrt\cyra\cyrk\cyrzh\cyre\nobreakspace}%
 %
      \Crefname@preamble{equation}%
      {\CYRF\cyro\cyrr\cyrm\cyru\cyrl\cyra}%
      {\CYRF\cyro\cyrr\cyrm\cyru\cyrl\cyrery}%
    \Crefname@preamble{figure}%
      {\CYRR\cyri\cyrs\cyru\cyrn\cyro\cyrk}%
      {\CYRR\cyri\cyrs\cyru\cyrn\cyrk\cyri}%
    \Crefname@preamble{table}%
      {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyra}%
      {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyrery}%
    \Crefname@preamble{enumi}%
      {\CYRP\cyru\cyrn\cyrk\cyrt}%
      {\CYRP\cyru\cyrn\cyrk\cyrt\cyrery}%
    \Crefname@preamble{chapter}%
      {\CYRG\cyrl\cyra\cyrv\cyra}%
      {\CYRG\cyrl\cyra\cyrv\cyrery}%
    \Crefname@preamble{section}%
      {\CYRR\cyra\cyrz\cyrd\cyre\cyrl}%
      {\CYRR\cyra\cyrz\cyrd\cyre\cyrl\cyrery}%
    \Crefname@preamble{appendix}%
      {\CYRP\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyre}%
      {\CYRP\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyrya}%
    \Crefname@preamble{footnote}%
      {\CYRS\cyrn\cyro\cyrs\cyrk\cyra}%
      {\CYRS\cyrn\cyro\cyrs\cyrk\cyri}%
    \Crefname@preamble{theorem}%
      {\CYRT\cyre\cyro\cyrr\cyre\cyrm\cyra}%
      {\CYRT\cyre\cyro\cyrr\cyre\cyrm\cyrery}%
    \Crefname@preamble{lemma}%
      {\CYRL\cyre\cyrm\cyrm\cyra}%
      {\CYRL\cyre\cyrm\cyrm\cyrery}%
    \Crefname@preamble{corollary}%
      {\CYRV\cyrery\cyrv\cyro\cyrd}%
      {\CYRV\cyrery\cyrv\cyro\cyrd\cyrery}%
    \Crefname@preamble{proposition}%
      {\CYRU\cyrt\cyrv\cyre\cyrr\cyrzh\cyrd\cyre\cyrn\cyri\cyre}%
      {\CYRU\cyrt\cyrv\cyre\cyrr\cyrzh\cyrd\cyre\cyrn\cyri\cyrya}%
    \Crefname@preamble{definition}%
      {\CYRO\cyrp\cyrr\cyre\cyrd\cyre\cyrl\cyre\cyrn\cyri\cyre}%
      {\CYRO\cyrp\cyrr\cyre\cyrd\cyre\cyrl\cyre\cyrn\cyri\cyrya}%
    \Crefname@preamble{result}%
      {\CYRR\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt}%
      {\CYRR\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt\cyrery}%
    \Crefname@preamble{example}%
      {\CYRP\cyrr\cyri\cyrm\cyre\cyrr}%
      {\CYRP\cyrr\cyri\cyrm\cyre\cyrr\cyrery}%
    \Crefname@preamble{remark}%
      {\CYRP\cyrr\cyri\cyrm\cyre\cyrch\cyra\cyrn\cyri\cyre}%
      {\CYRP\cyrr\cyri\cyrm\cyre\cyrch\cyra\cyrn\cyri\cyrya}%
    \Crefname@preamble{note}%
      {\CYRZ\cyra\cyrm\cyre\cyrt\cyrk\cyra}%
      {\CYRZ\cyra\cyrm\cyre\cyrt\cyrk\cyri}%
    \Crefname@preamble{algorithm}%
      {\CYRA\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm}%
      {\CYRA\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm\cyrery}%
    \Crefname@preamble{listing}%
      {\CYRL\cyri\cyrs\cyrt\cyri\cyrn\cyrg}%
      {\CYRL\cyri\cyrs\cyrt\cyri\cyrn\cyrg\cyri}%
    \Crefname@preamble{line}%
      {\CYRS\cyrt\cyrr\cyro\cyrk\cyra}%
      {\CYRS\cyrt\cyrr\cyro\cyrk\cyri}%
    \Crefname@preamble{page}%
      {\CYRS\cyrt\cyrr\cyra\cyrn\cyri\cyrc\cyra}%
      {\CYRS\cyrt\cyrr\cyra\cyrn\cyri\cyrc\cyrery}%
    \Crefname@preamble{part}%
      {\CYRCH\cyra\cyrs\cyrt\cyrsftsn}%
      {\CYRCH\cyra\cyrs\cyrt\cyri}%
 %
    \if@cref@capitalise%  capitalise set
      \if@cref@abbrev%  abbrev set
        \crefname@preamble{equation}%
          {\CYRF-\cyrl.}%
          {\CYRF-\cyrl.}%
        \crefname@preamble{figure}%
          {\CYRR\cyri\cyrs.}%
          {\CYRR\cyri\cyrs.}%
        \crefname@preamble{table}%
          {\CYRT\cyra\cyrb\cyrl.}%
          {\CYRT\cyra\cyrb\cyrl.}%
        \crefname@preamble{enumi}%
          {\CYRP.}%
          {\CYRP.\cyrp.}%
      \else%
        \crefname@preamble{equation}%
          {\CYRF\cyro\cyrr\cyrm\cyru\cyrl\cyra}%
          {\CYRF\cyro\cyrr\cyrm\cyru\cyrl\cyrery}%
        \crefname@preamble{figure}%
          {\CYRR\cyri\cyrs\cyru\cyrn\cyro\cyrk}%
          {\CYRR\cyri\cyrs\cyru\cyrn\cyrk\cyri}%
        \crefname@preamble{table}%
          {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyra}%
          {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyrery}%
        \crefname@preamble{enumi}%
          {\CYRP\cyru\cyrn\cyrk\cyrt}%
          {\CYRP\cyru\cyrn\cyrk\cyrt\cyrery}%
      \fi%
      \crefname@preamble{chapter}%
        {\CYRG\cyrl\cyra\cyrv\cyra}%
        {\CYRG\cyrl\cyra\cyrv\cyrery}%
      \crefname@preamble{section}%
        {\CYRR\cyra\cyrz\cyrd\cyre\cyrl}%
        {\CYRR\cyra\cyrz\cyrd\cyre\cyrl\cyrery}%
      \crefname@preamble{appendix}%
        {\CYRP\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyre}%
        {\CYRP\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyrya}%
      \crefname@preamble{footnote}%
        {\CYRS\cyrn\cyro\cyrs\cyrk\cyra}%
        {\CYRS\cyrn\cyro\cyrs\cyrk\cyri}%
      \crefname@preamble{theorem}%
        {\CYRT\cyre\cyro\cyrr\cyre\cyrm\cyra}%
        {\CYRT\cyre\cyro\cyrr\cyre\cyrm\cyrery}%
      \crefname@preamble{lemma}%
        {\CYRL\cyre\cyrm\cyrm\cyra}%
        {\CYRL\cyre\cyrm\cyrm\cyrery}%
      \crefname@preamble{corollary}%
        {\CYRV\cyrery\cyrv\cyro\cyrd}%
        {\CYRV\cyrery\cyrv\cyro\cyrd\cyrery}%
      \crefname@preamble{proposition}%
        {\CYRU\cyrt\cyrv\cyre\cyrr\cyrzh\cyrd\cyre\cyrn\cyri\cyre}%
        {\CYRU\cyrt\cyrv\cyre\cyrr\cyrzh\cyrd\cyre\cyrn\cyri\cyrya}%
      \crefname@preamble{definition}%
        {\CYRO\cyrp\cyrr\cyre\cyrd\cyre\cyrl\cyre\cyrn\cyri\cyre}%
        {\CYRO\cyrp\cyrr\cyre\cyrd\cyre\cyrl\cyre\cyrn\cyri\cyrya}%
      \crefname@preamble{result}%
        {\CYRR\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt}%
        {\CYRR\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt\cyrery}%
      \crefname@preamble{example}%
        {\CYRP\cyrr\cyri\cyrm\cyre\cyrr}%
        {\CYRP\cyrr\cyri\cyrm\cyre\cyrr\cyrery}%
      \crefname@preamble{remark}%
        {\CYRP\cyrr\cyri\cyrm\cyre\cyrch\cyra\cyrn\cyri\cyre}%
        {\CYRP\cyrr\cyri\cyrm\cyre\cyrch\cyra\cyrn\cyri\cyrya}%
      \crefname@preamble{note}%
        {\CYRZ\cyra\cyrm\cyre\cyrt\cyrk\cyra}%
        {\CYRZ\cyra\cyrm\cyre\cyrt\cyrk\cyri}%
      \crefname@preamble{algorithm}%
        {\CYRA\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm}%
        {\CYRA\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm\cyrery}%
      \crefname@preamble{listing}%
        {\CYRL\cyri\cyrs\cyrt\cyri\cyrn\cyrg}%
        {\CYRL\cyri\cyrs\cyrt\cyri\cyrn\cyrg\cyri}%
      \crefname@preamble{line}%
        {\CYRS\cyrt\cyrr\cyro\cyrk\cyra}%
        {\CYRS\cyrt\cyrr\cyro\cyrk\cyri}%
      \crefname@preamble{page}%
        {\CYRS\cyrt\cyrr\cyra\cyrn\cyri\cyrc\cyra}%
        {\CYRS\cyrt\cyrr\cyra\cyrn\cyri\cyrc\cyrery}%
      \crefname@preamble{part}%
        {\CYRCH\cyra\cyrs\cyrt\cyrsftsn}%
        {\CYRCH\cyra\cyrs\cyrt\cyri}%
 %
    \else%  capitalise unset
      \if@cref@abbrev%  abbrev set
        \crefname@preamble{equation}%
          {\cyrf-\cyrl.}%
          {\cyrf-\cyrl.}%
        \crefname@preamble{figure}%
          {\cyrr\cyri\cyrs.}%
          {\cyrr\cyri\cyrs.}%
        \crefname@preamble{table}%
          {\cyrt\cyra\cyrb\cyrl.}%
          {\cyrt\cyra\cyrb\cyrl.}%
        \crefname@preamble{enumi}%
          {\cyrp.}%
          {\cyrp.\cyrp.}%
        \crefname@preamble{chapter}%
          {\cyrg\cyrl\cyra\cyrv.}%
          {\cyrg\cyrl\cyra\cyrv.}%
        \crefname@preamble{section}%
          {\cyrr\cyra\cyrz\cyrd.}%
          {\cyrr\cyra\cyrz\cyrd\cyre\cyrl.}%
        \crefname@preamble{appendix}%
          {\cyrp\cyrr\cyri\cyrl\cyro\cyrzh.}%
          {\cyrp\cyrr\cyri\cyrl\cyro\cyrzh.}%
        \crefname@preamble{footnote}%
          {\cyrs\cyrn\cyro\cyrs\cyrk.}%
          {\cyrs\cyrn\cyro\cyrs\cyrk.}%
        \crefname@preamble{theorem}%
          {\cyrt\cyre\cyro\cyrr\cyre\cyrm.}%
          {\cyrt\cyre\cyro\cyrr\cyre\cyrm.}%
        \crefname@preamble{lemma}%
          {\cyrl\cyre\cyrm\cyrm.}%
          {\cyrl\cyre\cyrm\cyrm.}%
        \crefname@preamble{corollary}%
          {\cyrv\cyrery\cyrv\cyro\cyrd}%
          {\cyrv\cyrery\cyrv\cyro\cyrd.}%
        \crefname@preamble{proposition}%
          {\cyru\cyrt\cyrv\cyre\cyrr\cyrzh\cyrd.}%
          {\cyru\cyrt\cyrv\cyre\cyrr\cyrzh\cyrd.}%
        \crefname@preamble{definition}%
          {\cyro\cyrp\cyrr\cyre\cyrd\cyre\cyrl\cyre\cyrn.}%
          {\cyro\cyrp\cyrr\cyre\cyrd\cyre\cyrl\cyre\cyrn.}%
        \crefname@preamble{result}%
          {\cyrr\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt.}%
          {\cyrr\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt.}%
        \crefname@preamble{example}%
          {\cyrp\cyrr\cyri\cyrm.}%
          {\cyrp\cyrr\cyri\cyrm\cyre\cyrr.}%
        \crefname@preamble{remark}%
          {\cyrp\cyrr\cyri\cyrm\cyre\cyrch.}%
          {\cyrp\cyrr\cyri\cyrm\cyre\cyrch.}%
        \crefname@preamble{note}%
          {\cyrz\cyra\cyrm\cyre\cyrt\cyrk.}%
          {\cyrz\cyra\cyrm\cyre\cyrt\cyrk.}%
        \crefname@preamble{algorithm}%
          {\cyra\cyrl\cyrg.}%
          {\cyra\cyrl\cyrg.}%
        \crefname@preamble{listing}%
          {\cyrl\cyri\cyrs\cyrt\cyri\cyrn.}%
          {\cyrl\cyri\cyrs\cyrt\cyri\cyrn\cyrg.}%
        \crefname@preamble{line}%
          {\cyrs\cyrt\cyrr\cyrk.}%
          {\cyrs\cyrt\cyrr\cyrk.}%
      \else%  abbrev unset
        \crefname@preamble{equation}%
          {\cyrf\cyro\cyrr\cyrm\cyru\cyrl\cyra}%
          {\cyrf\cyro\cyrr\cyrm\cyru\cyrl\cyrery}%
        \crefname@preamble{figure}%
          {\cyrr\cyri\cyrs\cyru\cyrn\cyro\cyrk}%
          {\cyrr\cyri\cyrs\cyru\cyrn\cyrk\cyri}%
        \crefname@preamble{table}%
          {\cyrt\cyra\cyrb\cyrl\cyri\cyrc\cyra}%
          {\cyrt\cyra\cyrb\cyrl\cyri\cyrc\cyrery}%
        \crefname@preamble{enumi}%
          {\cyrp\cyru\cyrn\cyrk\cyrt}%
          {\cyrp\cyru\cyrn\cyrk\cyrt\cyrery}%
        \crefname@preamble{chapter}%
          {\cyrg\cyrl\cyra\cyrv\cyra}%
          {\cyrg\cyrl\cyra\cyrv\cyrery}%
        \crefname@preamble{section}%
          {\cyrr\cyra\cyrz\cyrd\cyre\cyrl}%
          {\cyrr\cyra\cyrz\cyrd\cyre\cyrl\cyrery}%
        \crefname@preamble{appendix}%
          {\cyrp\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyre}%
          {\cyrp\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyrya}%
        \crefname@preamble{footnote}%
          {\cyrs\cyrn\cyro\cyrs\cyrk\cyra}%
          {\cyrs\cyrn\cyro\cyrs\cyrk\cyri}%
        \crefname@preamble{theorem}%
          {\cyrt\cyre\cyro\cyrr\cyre\cyrm\cyra}%
          {\cyrt\cyre\cyro\cyrr\cyre\cyrm\cyrery}%
        \crefname@preamble{lemma}%
          {\cyrl\cyre\cyrm\cyrm\cyra}%
          {\cyrl\cyre\cyrm\cyrm\cyrery}%
        \crefname@preamble{corollary}%
          {\cyrv\cyrery\cyrv\cyro\cyrd}%
          {\cyrv\cyrery\cyrv\cyro\cyrd\cyrery}%
        \crefname@preamble{proposition}%
          {\cyru\cyrt\cyrv\cyre\cyrr\cyrzh\cyrd\cyre\cyrn\cyri\cyre}%
          {\cyru\cyrt\cyrv\cyre\cyrr\cyrzh\cyrd\cyre\cyrn\cyri\cyrya}%
        \crefname@preamble{definition}%
          {\cyro\cyrp\cyrr\cyre\cyrd\cyre\cyrl\cyre\cyrn\cyri\cyre}%
          {\cyro\cyrp\cyrr\cyre\cyrd\cyre\cyrl\cyre\cyrn\cyri\cyrya}%
        \crefname@preamble{result}%
          {\cyrr\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt}%
          {\cyrr\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt\cyrery}%
        \crefname@preamble{example}%
          {\cyrp\cyrr\cyri\cyrm\cyre\cyrr}%
          {\cyrp\cyrr\cyri\cyrm\cyre\cyrr\cyrery}%
        \crefname@preamble{remark}%
          {\cyrp\cyrr\cyri\cyrm\cyre\cyrch\cyra\cyrn\cyri\cyre}%
          {\cyrp\cyrr\cyri\cyrm\cyre\cyrch\cyra\cyrn\cyri\cyrya}%
        \crefname@preamble{note}%
          {\cyrz\cyra\cyrm\cyre\cyrt\cyrk\cyra}%
          {\cyrz\cyra\cyrm\cyre\cyrt\cyrk\cyri}%
        \crefname@preamble{algorithm}%
          {\cyra\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm}%
          {\cyra\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm\cyrery}%
        \crefname@preamble{listing}%
          {\cyrl\cyri\cyrs\cyrt\cyri\cyrn\cyrg}%
          {\cyrl\cyri\cyrs\cyrt\cyri\cyrn\cyrg\cyri}%
        \crefname@preamble{line}%
          {\cyrs\cyrt\cyrr\cyro\cyrk\cyra}%
          {\cyrs\cyrt\cyrr\cyro\cyrk\cyri}%
      \fi%
      \crefname@preamble{page}%
        {\cyrs\cyrt\cyrr\cyra\cyrn\cyri\cyrc\cyre}%
        {\cyrs\cyrt\cyrr\cyra\cyrn\cyri\cyrc\cyra\cyrh}%
      \crefname@preamble{part}%
        {\cyrch\cyra\cyrs\cyrt\cyrsftsn}%
        {\cyrch\cyra\cyrs\cyrt\cyri}%
    \fi%
    \def\cref@language{russian}%
    \cref@addto\extrasrussian{%
      \renewcommand{\crefrangeconjunction}{--}%
      \renewcommand\crefrangepreconjunction{}%
      \renewcommand\crefrangepostconjunction{}%
      \renewcommand{\crefpairconjunction}{ \cyri\nobreakspace}%
      \renewcommand{\crefmiddleconjunction}{, }%
      \renewcommand{\creflastconjunction}{ \cyri\nobreakspace}%
      \renewcommand{\crefpairgroupconjunction}{ \cyri\nobreakspace}%
      \renewcommand{\crefmiddlegroupconjunction}{, }%
      \renewcommand{\creflastgroupconjunction}%
        {, \cyra\ \cyrt\cyra\cyrk\cyrzh\cyre\nobreakspace}%
 %
        \Crefname{page}%
        {\CYRS\cyrt\cyrr\cyra\cyrn\cyri\cyrc\cyra}%
        {\CYRS\cyrt\cyrr\cyra\cyrn\cyri\cyrc\cyrery}%
      \Crefname{equation}%
        {\CYRF\cyro\cyrr\cyrm\cyru\cyrl\cyra}%
        {\CYRF\cyro\cyrr\cyrm\cyru\cyrl\cyrery}%
      \Crefname{figure}%
        {\CYRR\cyri\cyrs\cyru\cyrn\cyro\cyrk}%
        {\CYRR\cyri\cyrs\cyru\cyrn\cyrk\cyri}%
      \Crefname{subfigure}%
        {\CYRR\cyri\cyrs\cyru\cyrn\cyro\cyrk}%
        {\CYRR\cyri\cyrs\cyru\cyrn\cyrk\cyri}%
      \Crefname{table}%
        {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyra}%
        {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyrery}%
      \Crefname{subtable}%
        {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyra}%
        {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyrery}%
      \Crefname{part}%
        {\CYRCH\cyra\cyrs\cyrt\cyrsftsn}%
        {\CYRCH\cyra\cyrs\cyrt\cyri}%
      \Crefname{chapter}%
        {\CYRG\cyrl\cyra\cyrv\cyra}%
        {\CYRG\cyrl\cyra\cyrv\cyrery}%
      \Crefname{section}%
        {\CYRR\cyra\cyrz\cyrd\cyre\cyrl}%
        {\CYRR\cyra\cyrz\cyrd\cyre\cyrl\cyrery}%
      \Crefname{subsection}%
        {\CYRR\cyra\cyrz\cyrd\cyre\cyrl}%
        {\CYRR\cyra\cyrz\cyrd\cyre\cyrl\cyrery}%
      \Crefname{subsubsection}%
        {\CYRR\cyra\cyrz\cyrd\cyre\cyrl}%
        {\CYRR\cyra\cyrz\cyrd\cyre\cyrl\cyrery}%
      \Crefname{appendix}%
        {\CYRP\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyre}%
        {\CYRP\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyrya}%
      \Crefname{subappendix}%
        {\CYRP\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyre}%
        {\CYRP\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyrya}
      \Crefname{subsubappendix}%
        {\CYRP\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyre}%
        {\CYRP\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyrya}
      \Crefname{subsubsubappendix}%
        {\CYRP\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyre}%
        {\CYRP\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyrya}
      \Crefname{enumi}%
        {\CYRP\cyru\cyrn\cyrk\cyrt}%
        {\CYRP\cyru\cyrn\cyrk\cyrt\cyrery}%
      \Crefname{enumii}%
        {\CYRP\cyru\cyrn\cyrk\cyrt}%
        {\CYRP\cyru\cyrn\cyrk\cyrt\cyrery}%
      \Crefname{enumiii}%
        {\CYRP\cyru\cyrn\cyrk\cyrt}%
        {\CYRP\cyru\cyrn\cyrk\cyrt\cyrery}%
      \Crefname{enumiv}%
        {\CYRP\cyru\cyrn\cyrk\cyrt}%
        {\CYRP\cyru\cyrn\cyrk\cyrt\cyrery}%
      \Crefname{enumv}%
        {\CYRP\cyru\cyrn\cyrk\cyrt}%
        {\CYRP\cyru\cyrn\cyrk\cyrt\cyrery}%
      \Crefname{footnote}%
        {\CYRS\cyrn\cyro\cyrs\cyrk\cyra}%
        {\CYRS\cyrn\cyro\cyrs\cyrk\cyri}%
      \Crefname{theorem}%
        {\CYRT\cyre\cyro\cyrr\cyre\cyrm\cyra}%
        {\CYRT\cyre\cyro\cyrr\cyre\cyrm\cyrery}%
      \Crefname{lemma}%
        {\CYRL\cyre\cyrm\cyrm\cyra}%
        {\CYRL\cyre\cyrm\cyrm\cyrery}%
      \Crefname{corollary}%
        {\CYRV\cyrery\cyrv\cyro\cyrd}%
        {\CYRV\cyrery\cyrv\cyro\cyrd\cyrery}%
      \Crefname{proposition}%
        {\CYRU\cyrt\cyrv\cyre\cyrr\cyrzh\cyrd\cyre\cyrn\cyri\cyre}%
        {\CYRU\cyrt\cyrv\cyre\cyrr\cyrzh\cyrd\cyre\cyrn\cyri\cyrya}%
      \Crefname{definition}%
        {\CYRO\cyrp\cyrr\cyre\cyrd\cyre\cyrl\cyre\cyrn\cyri\cyre}%
        {\CYRO\cyrp\cyrr\cyre\cyrd\cyre\cyrl\cyre\cyrn\cyri\cyrya}%
      \Crefname{result}%
        {\CYRR\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt}%
        {\CYRR\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt\cyrery}%
      \Crefname{example}%
        {\CYRP\cyrr\cyri\cyrm\cyre\cyrr}%
        {\CYRP\cyrr\cyri\cyrm\cyre\cyrr\cyrery}%
      \Crefname{remark}%
        {\CYRP\cyrr\cyri\cyrm\cyre\cyrch\cyra\cyrn\cyri\cyre}%
        {\CYRP\cyrr\cyri\cyrm\cyre\cyrch\cyra\cyrn\cyri\cyrya}%
      \Crefname{note}%
        {\CYRZ\cyra\cyrm\cyre\cyrt\cyrk\cyra}%
        {\CYRZ\cyra\cyrm\cyre\cyrt\cyrk\cyri}%
      \Crefname{algorithm}%
        {\CYRA\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm}%
        {\CYRA\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm\cyrery}%
      \Crefname{listing}%
        {\CYRL\cyri\cyrs\cyrt\cyri\cyrn\cyrg}%
        {\CYRL\cyri\cyrs\cyrt\cyri\cyrn\cyrg\cyri}%
      \Crefname{line}%
        {\CYRS\cyrt\cyrr\cyro\cyrk\cyra}%
        {\CYRS\cyrt\cyrr\cyro\cyrk\cyri}%
 %
      \if@cref@capitalise%  capitalise set
        \if@cref@abbrev%  abbrev set
          \crefname{equation}%
            {\CYRF-\cyrl.}%
            {\CYRF-\cyrl.}%
          \crefname{figure}%
            {\CYRR\cyri\cyrs.}%
            {\CYRR\cyri\cyrs.}%
          \crefname{subfigure}%
            {\CYRR\cyri\cyrs.}%
            {\CYRR\cyri\cyrs.}%
          \crefname{table}%
            {\CYRT\cyra\cyrb\cyrl.}%
            {\CYRT\cyra\cyrb\cyrl.}%
          \crefname{subtable}%
            {\CYRT\cyra\cyrb\cyrl.}%
            {\CYRT\cyra\cyrb\cyrl.}%
          \crefname{enumi}%
            {\CYRP.}%
            {\CYRP.\cyrp.}%
          \crefname{enumii}%
            {\CYRP.}%
            {\CYRP.\cyrp.}%
          \crefname{enumiii}%
            {\CYRP.}%
            {\CYRP.\cyrp.}%
          \crefname{enumiv}%
            {\CYRP.}%
            {\CYRP.\cyrp.}%
          \crefname{enumv}%
            {\CYRP.}%
            {\CYRP.\cyrp.}%
        \else%  abbrev unset
          \crefname{equation}%
            {\CYRF\cyro\cyrr\cyrm\cyru\cyrl\cyra}%
            {\CYRF\cyro\cyrr\cyrm\cyru\cyrl\cyrery}%
          \crefname{figure}%
            {\CYRR\cyri\cyrs\cyru\cyrn\cyro\cyrk}%
            {\CYRR\cyri\cyrs\cyru\cyrn\cyrk\cyri}%
          \crefname{subfigure}%
            {\CYRR\cyri\cyrs\cyru\cyrn\cyro\cyrk}%
            {\CYRR\cyri\cyrs\cyru\cyrn\cyrk\cyri}%
          \crefname{table}%
            {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyra}%
            {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyrery}%
          \crefname{subtable}%
            {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyra}%
            {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyrery}%
          \crefname{enumi}%
            {\CYRP\cyru\cyrn\cyrk\cyrt}%
            {\CYRP\cyru\cyrn\cyrk\cyrt\cyrery}%
          \crefname{enumii}%
            {\CYRP\cyru\cyrn\cyrk\cyrt}%
            {\CYRP\cyru\cyrn\cyrk\cyrt\cyrery}%
          \crefname{enumiii}%
            {\CYRP\cyru\cyrn\cyrk\cyrt}%
            {\CYRP\cyru\cyrn\cyrk\cyrt\cyrery}%
          \crefname{enumiv}%
            {\CYRP\cyru\cyrn\cyrk\cyrt}%
            {\CYRP\cyru\cyrn\cyrk\cyrt\cyrery}%
          \crefname{enumv}%
            {\CYRP\cyru\cyrn\cyrk\cyrt}%
            {\CYRP\cyru\cyrn\cyrk\cyrt\cyrery}%
        \fi%
        \crefname{page}%
          {\CYRS\cyrt\cyrr\cyra\cyrn\cyri\cyrc\cyra}%
          {\CYRS\cyrt\cyrr\cyra\cyrn\cyri\cyrc\cyrery}%
        \crefname{part}%
          {\CYRCH\cyra\cyrs\cyrt\cyrsftsn}%
          {\CYRCH\cyra\cyrs\cyrt\cyri}%
        \crefname{chapter}%
          {\CYRG\cyrl\cyra\cyrv\cyra}%
          {\CYRG\cyrl\cyra\cyrv\cyrery}%
        \crefname{section}%
          {\CYRR\cyra\cyrz\cyrd\cyre\cyrl}%
          {\CYRR\cyra\cyrz\cyrd\cyre\cyrl\cyrery}%
        \crefname{subsection}%
          {\CYRR\cyra\cyrz\cyrd\cyre\cyrl}%
          {\CYRR\cyra\cyrz\cyrd\cyre\cyrl\cyrery}%
        \crefname{subsubsection}%
          {\CYRR\cyra\cyrz\cyrd\cyre\cyrl}%
          {\CYRR\cyra\cyrz\cyrd\cyre\cyrl\cyrery}%
        \crefname{appendix}%
          {\CYRP\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyre}%
          {\CYRP\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyrya}%
        \crefname{subappendix}%
          {\CYRP\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyre}%
          {\CYRP\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyrya}%
        \crefname{subsubappendix}%
          {\CYRP\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyre}%
          {\CYRP\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyrya}%
        \crefname{subsubsubappendix}%
          {\CYRP\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyre}%
          {\CYRP\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyrya}%
        \crefname{footnote}%
          {\CYRS\cyrn\cyro\cyrs\cyrk\cyra}%
          {\CYRS\cyrn\cyro\cyrs\cyrk\cyri}%
        \crefname{theorem}%
          {\CYRT\cyre\cyro\cyrr\cyre\cyrm\cyra}%
          {\CYRT\cyre\cyro\cyrr\cyre\cyrm\cyrery}%
        \crefname{lemma}%
          {\CYRL\cyre\cyrm\cyrm\cyra}%
          {\CYRL\cyre\cyrm\cyrm\cyrery}%
        \crefname{corollary}%
          {\CYRV\cyrery\cyrv\cyro\cyrd}%
          {\CYRV\cyrery\cyrv\cyro\cyrd\cyrery}%
        \crefname{proposition}%
          {\CYRU\cyrt\cyrv\cyre\cyrr\cyrzh\cyrd\cyre\cyrn\cyri\cyre}%
          {\CYRU\cyrt\cyrv\cyre\cyrr\cyrzh\cyrd\cyre\cyrn\cyri\cyrya}%
        \crefname{definition}%
          {\CYRO\cyrp\cyrr\cyre\cyrd\cyre\cyrl\cyre\cyrn\cyri\cyre}%
          {\CYRO\cyrp\cyrr\cyre\cyrd\cyre\cyrl\cyre\cyrn\cyri\cyrya}%
        \crefname{result}%
          {\CYRR\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt}%
          {\CYRR\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt\cyrery}%
        \crefname{example}%
          {\CYRP\cyrr\cyri\cyrm\cyre\cyrr}%
          {\CYRP\cyrr\cyri\cyrm\cyre\cyrr\cyrery}%
        \crefname{remark}%
          {\CYRP\cyrr\cyri\cyrm\cyre\cyrch\cyra\cyrn\cyri\cyre}%
          {\CYRP\cyrr\cyri\cyrm\cyre\cyrch\cyra\cyrn\cyri\cyrya}%
        \crefname{note}%
          {\CYRZ\cyra\cyrm\cyre\cyrt\cyrk\cyra}%
          {\CYRZ\cyra\cyrm\cyre\cyrt\cyrk\cyri}%
        \crefname{algorithm}%
          {\CYRA\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm}%
          {\CYRA\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm\cyrery}%
        \crefname{listing}%
          {\CYRL\cyri\cyrs\cyrt\cyri\cyrn\cyrg}%
          {\CYRL\cyri\cyrs\cyrt\cyri\cyrn\cyrg\cyri}%
        \crefname{line}%
          {\CYRS\cyrt\cyrr\cyro\cyrk\cyra}%
          {\CYRS\cyrt\cyrr\cyro\cyrk\cyri}%
 %
      \else%  capitalise unset
        \if@cref@abbrev%  abbrev set
          \crefname{equation}%
            {\cyrf-\cyrl.}%
            {\cyrf-\cyrl.}%
          \crefname{chapter}%
            {\cyrg\cyrl\cyra\cyrv.}%
            {\cyrg\cyrl\cyra\cyrv.}%
          \crefname{section}%
            {\cyrr\cyra\cyrz\cyrd.}%
            {\cyrr\cyra\cyrz\cyrd\cyre\cyrl.}%
          \crefname{subsection}%
            {\cyrr\cyra\cyrz\cyrd.}%
            {\cyrr\cyra\cyrz\cyrd\cyre\cyrl.}%
          \crefname{subsubsection}%
            {\cyrr\cyra\cyrz\cyrd.}%
            {\cyrr\cyra\cyrz\cyrd\cyre\cyrl.}%
          \crefname{appendix}%
            {\cyrp\cyrr\cyri\cyrl\cyro\cyrzh.}%
            {\cyrp\cyrr\cyri\cyrl\cyro\cyrzh.}%
          \crefname{subappendix}%
            {\cyrp\cyrr\cyri\cyrl\cyro\cyrzh.}%
            {\cyrp\cyrr\cyri\cyrl\cyro\cyrzh.}%
          \crefname{subsubappendix}%
            {\cyrp\cyrr\cyri\cyrl\cyro\cyrzh.}%
            {\cyrp\cyrr\cyri\cyrl\cyro\cyrzh.}%
          \crefname{subsubsubappendix}%
            {\cyrp\cyrr\cyri\cyrl\cyro\cyrzh.}%
            {\cyrp\cyrr\cyri\cyrl\cyro\cyrzh.}%
          \crefname{enumi}%
            {\cyrp.}%
            {\cyrp.\cyrp.}%
          \crefname{enumii}%
            {\cyrp.}%
            {\cyrp.\cyrp.}%
          \crefname{enumiii}%
            {\cyrp.}%
            {\cyrp.\cyrp.}%
          \crefname{enumiv}%
            {\cyrp.}%
            {\cyrp.\cyrp.}%
          \crefname{enumv}%
            {\cyrp.}%
            {\cyrp.\cyrp.}%
          \crefname{footnote}%
            {\cyrs\cyrn\cyro\cyrs\cyrk.}%
            {\cyrs\cyrn\cyro\cyrs\cyrk.}%
          \crefname{figure}%
            {\cyrr\cyri\cyrs.}%
            {\cyrr\cyri\cyrs.}%
          \crefname{subfigure}%
            {\cyrr\cyri\cyrs.}%
            {\cyrr\cyri\cyrs.}%
          \crefname{table}%
            {\cyrt\cyra\cyrb\cyrl.}%
            {\cyrt\cyra\cyrb\cyrl.}%
          \crefname{subtable}%
            {\cyrt\cyra\cyrb\cyrl.}%
            {\cyrt\cyra\cyrb\cyrl.}%
          \crefname{theorem}%
            {\cyrt\cyre\cyro\cyrr\cyre\cyrm.}%
            {\cyrt\cyre\cyro\cyrr\cyre\cyrm.}%
          \crefname{lemma}%
            {\cyrl\cyre\cyrm\cyrm.}%
            {\cyrl\cyre\cyrm\cyrm.}%
          \crefname{corollary}%
            {\cyrv\cyrery\cyrv\cyro\cyrd}%
            {\cyrv\cyrery\cyrv\cyro\cyrd.}%
          \crefname{proposition}%
            {\cyru\cyrt\cyrv\cyre\cyrr\cyrzh\cyrd.}%
            {\cyru\cyrt\cyrv\cyre\cyrr\cyrzh\cyrd.}%
          \crefname{definition}%
            {\cyro\cyrp\cyrr\cyre\cyrd\cyre\cyrl\cyre\cyrn.}%
            {\cyro\cyrp\cyrr\cyre\cyrd\cyre\cyrl\cyre\cyrn.}%
          \crefname{result}%
            {\cyrr\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt.}%
            {\cyrr\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt.}%
          \crefname{example}%
            {\cyrp\cyrr\cyri\cyrm.}%
            {\cyrp\cyrr\cyri\cyrm\cyre\cyrr.}%
          \crefname{remark}%
            {\cyrp\cyrr\cyri\cyrm\cyre\cyrch.}%
            {\cyrp\cyrr\cyri\cyrm\cyre\cyrch.}%
          \crefname{note}%
            {\cyrz\cyra\cyrm\cyre\cyrt\cyrk.}%
            {\cyrz\cyra\cyrm\cyre\cyrt\cyrk.}%
          \crefname{algorithm}%
            {\cyra\cyrl\cyrg.}%
            {\cyra\cyrl\cyrg.}%
          \crefname{listing}%
            {\cyrl\cyri\cyrs\cyrt\cyri\cyrn.}%
            {\cyrl\cyri\cyrs\cyrt\cyri\cyrn\cyrg.}%
          \crefname{line}%
            {\cyrs\cyrt\cyrr\cyrk.}%
            {\cyrs\cyrt\cyrr\cyrk.}%
        \else%  abbrev unset
          \crefname{equation}%
            {\cyrf\cyro\cyrr\cyrm\cyru\cyrl\cyra}%
            {\cyrf\cyro\cyrr\cyrm\cyru\cyrl\cyrery}%
          \crefname{figure}%
            {\cyrr\cyri\cyrs\cyru\cyrn\cyro\cyrk}%
            {\cyrr\cyri\cyrs\cyru\cyrn\cyrk\cyri}%
          \crefname{subfigure}%
            {\cyrr\cyri\cyrs\cyru\cyrn\cyro\cyrk}%
            {\cyrr\cyri\cyrs\cyru\cyrn\cyrk\cyri}%
          \crefname{table}%
            {\cyrt\cyra\cyrb\cyrl\cyri\cyrc\cyra}%
            {\cyrt\cyra\cyrb\cyrl\cyri\cyrc\cyrery}%
          \crefname{subtable}%
            {\cyrt\cyra\cyrb\cyrl\cyri\cyrc\cyra}%
            {\cyrt\cyra\cyrb\cyrl\cyri\cyrc\cyrery}%
          \crefname{enumi}%
            {\cyrp\cyru\cyrn\cyrk\cyrt}%
            {\cyrp\cyru\cyrn\cyrk\cyrt\cyrery}%
          \crefname{enumii}%
            {\cyrp\cyru\cyrn\cyrk\cyrt}%
            {\cyrp\cyru\cyrn\cyrk\cyrt\cyrery}%
          \crefname{enumiii}%
            {\cyrp\cyru\cyrn\cyrk\cyrt}%
            {\cyrp\cyru\cyrn\cyrk\cyrt\cyrery}%
          \crefname{enumiv}%
            {\cyrp\cyru\cyrn\cyrk\cyrt}%
            {\cyrp\cyru\cyrn\cyrk\cyrt\cyrery}%
          \crefname{enumv}%
            {\cyrp\cyru\cyrn\cyrk\cyrt}%
            {\cyrp\cyru\cyrn\cyrk\cyrt\cyrery}%
          \crefname{chapter}%
            {\cyrg\cyrl\cyra\cyrv\cyra}%
            {\cyrg\cyrl\cyra\cyrv\cyrery}%
          \crefname{section}%
            {\cyrr\cyra\cyrz\cyrd\cyre\cyrl}%
            {\cyrr\cyra\cyrz\cyrd\cyre\cyrl\cyrery}%
          \crefname{subsection}%
            {\cyrr\cyra\cyrz\cyrd\cyre\cyrl}%
            {\cyrr\cyra\cyrz\cyrd\cyre\cyrl\cyrery}%
          \crefname{subsubsection}%
            {\cyrr\cyra\cyrz\cyrd\cyre\cyrl}%
            {\cyrr\cyra\cyrz\cyrd\cyre\cyrl\cyrery}%
          \crefname{appendix}%
            {\cyrp\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyre}%
            {\cyrp\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyrya}%
          \crefname{subappendix}%
            {\cyrp\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyre}%
            {\cyrp\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyrya}%
          \crefname{subsubappendix}%
            {\cyrp\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyre}%
            {\cyrp\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyrya}%
          \crefname{subsubsubappendix}%
            {\cyrp\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyre}%
            {\cyrp\cyrr\cyri\cyrl\cyro\cyrzh\cyre\cyrn\cyri\cyrya}%
          \crefname{footnote}%
            {\cyrs\cyrn\cyro\cyrs\cyrk\cyra}%
            {\cyrs\cyrn\cyro\cyrs\cyrk\cyri}%
          \crefname{theorem}%
            {\cyrt\cyre\cyro\cyrr\cyre\cyrm\cyra}%
            {\cyrt\cyre\cyro\cyrr\cyre\cyrm\cyrery}%
          \crefname{lemma}%
            {\cyrl\cyre\cyrm\cyrm\cyra}%
            {\cyrl\cyre\cyrm\cyrm\cyrery}%
          \crefname{corollary}%
            {\cyrv\cyrery\cyrv\cyro\cyrd}%
            {\cyrv\cyrery\cyrv\cyro\cyrd\cyrery}%
          \crefname{proposition}%
            {\cyru\cyrt\cyrv\cyre\cyrr\cyrzh\cyrd\cyre\cyrn\cyri\cyre}%
            {\cyru\cyrt\cyrv\cyre\cyrr\cyrzh\cyrd\cyre\cyrn\cyri\cyrya}%
          \crefname{definition}%
            {\cyro\cyrp\cyrr\cyre\cyrd\cyre\cyrl\cyre\cyrn\cyri\cyre}%
            {\cyro\cyrp\cyrr\cyre\cyrd\cyre\cyrl\cyre\cyrn\cyri\cyrya}%
          \crefname{result}%
            {\cyrr\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt}%
            {\cyrr\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt\cyrery}%
          \crefname{example}%
            {\cyrp\cyrr\cyri\cyrm\cyre\cyrr}%
            {\cyrp\cyrr\cyri\cyrm\cyre\cyrr\cyrery}%
          \crefname{remark}%
            {\cyrp\cyrr\cyri\cyrm\cyre\cyrch\cyra\cyrn\cyri\cyre}%
            {\cyrp\cyrr\cyri\cyrm\cyre\cyrch\cyra\cyrn\cyri\cyrya}%
          \crefname{note}%
            {\cyrz\cyra\cyrm\cyre\cyrt\cyrk\cyra}%
            {\cyrz\cyra\cyrm\cyre\cyrt\cyrk\cyri}%
          \crefname{algorithm}%
            {\cyra\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm}%
            {\cyra\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm\cyrery}%
          \crefname{listing}%
            {\cyrl\cyri\cyrs\cyrt\cyri\cyrn\cyrg}%
            {\cyrl\cyri\cyrs\cyrt\cyri\cyrn\cyrg\cyri}%
          \crefname{line}%
            {\cyrs\cyrt\cyrr\cyro\cyrk\cyra}%
            {\cyrs\cyrt\cyrr\cyro\cyrk\cyri}%
        \fi%
        \crefname{page}%
          {\cyrs\cyrt\cyrr\cyra\cyrn\cyri\cyrc\cyre}%
          {\cyrs\cyrt\cyrr\cyra\cyrn\cyri\cyrc\cyra\cyrh}%
        \crefname{part}%
          {\cyrch\cyra\cyrs\cyrt\cyrsftsn}%
          {\cyrch\cyra\cyrs\cyrt\cyri}%
      \fi%
    }}}
\DeclareOption{ukrainian}{%
  \PackageInfo{cleveref}{loaded `ukrainian' language definitions}
  \AtBeginDocument{%
    \def\crefrangeconjunction@preamble{--}%
    \def\crefrangepreconjunction@preamble{}%
    \def\crefrangepostconjunction@preamble{}%
    \def\crefpairconjunction@preamble{ \cyrii\nobreakspace}%
    \def\crefmiddleconjunction@preamble{, }%
    \def\creflastconjunction@preamble{ \cyrii\nobreakspace}%
    \def\crefpairgroupconjunction@preamble{ \cyrt\cyra\nobreakspace}%
    \def\crefmiddlegroupconjunction@preamble{, }%
    \def\creflastgroupconjunction@preamble%
      {, \cyra\ \cyrt\cyra\cyrk\cyro\cyrzh\nobreakspace}%
 %
    \Crefname@preamble{equation}%
      {\CYRF\cyro\cyrr\cyrm\cyru\cyrl\cyra}%
      {\CYRF\cyro\cyrr\cyrm\cyru\cyrl\cyri}%
    \Crefname@preamble{figure}%
      {\CYRR\cyri\cyrs\cyru\cyrn\cyro\cyrk}%
      {\CYRR\cyri\cyrs\cyru\cyrn\cyrk\cyri}%
    \Crefname@preamble{table}%
      {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyrya}%
      {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyrii}%
    \Crefname@preamble{enumi}%
      {\CYRP\cyru\cyrn\cyrk\cyrt}%
      {\CYRP\cyru\cyrn\cyrk\cyrt\cyri}%
    \Crefname@preamble{chapter}%
      {\CYRG\cyrl\cyra\cyrv\cyra}%
      {\CYRG\cyrl\cyra\cyrv\cyri}%
    \Crefname@preamble{section}%
      {\CYRR\cyro\cyrz\cyrd\cyrii\cyrl}%
      {\CYRR\cyro\cyrz\cyrd\cyrii\cyrl\cyri}%
    \Crefname@preamble{appendix}%
      {\CYRD\cyro\cyrd\cyra\cyrt\cyro\cyrk}%
      {\CYRD\cyro\cyrd\cyra\cyrt\cyrk\cyri}%
    \Crefname@preamble{footnote}%
      {\CYRV\cyri\cyrn\cyro\cyrs\cyrk\cyra}%
      {\CYRV\cyri\cyrn\cyro\cyrs\cyrk\cyri}%
    \Crefname@preamble{theorem}%
      {\CYRT\cyre\cyro\cyrr\cyre\cyrm\cyra}%
      {\CYRT\cyre\cyro\cyrr\cyre\cyrm\cyri}%
    \Crefname@preamble{lemma}%
      {\CYRL\cyre\cyrm\cyrm\cyra}%
      {\CYRL\cyre\cyrm\cyrm\cyri}%
    \Crefname@preamble{corollary}%
      {\CYRV\cyri\cyrs\cyrn\cyro\cyrv\cyro\cyrk}%
      {\CYRV\cyri\cyrs\cyrn\cyro\cyrv\cyrk\cyri}%
    \Crefname@preamble{proposition}%
      {\CYRT\cyrv\cyre\cyrr\cyrd\cyrzh\cyre\cyrn\cyrn\cyrya}%
      {\CYRT\cyrv\cyre\cyrr\cyrd\cyrzh\cyre\cyrn\cyrn\cyrya}%
    \Crefname@preamble{definition}%
      {\CYRV\cyri\cyrz\cyrn\cyra\cyrch\cyre\cyrn\cyrn\cyrya}%
      {\CYRV\cyri\cyrz\cyrn\cyra\cyrch\cyre\cyrn\cyrn\cyrya}%
    \Crefname@preamble{result}%
      {\CYRR\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt}%
      {\CYRR\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt\cyri}%
    \Crefname@preamble{example}%
      {\CYRP\cyrr\cyri\cyrk\cyrl\cyra\cyrd}%
      {\CYRP\cyrr\cyri\cyrk\cyrl\cyra\cyrd\cyri}%
    \Crefname@preamble{remark}%
      {\CYRP\cyrr\cyri\cyrm\cyrii\cyrt\cyrk\cyra}%
      {\CYRP\cyrr\cyri\cyrm\cyrii\cyrt\cyrk\cyri}%
    \Crefname@preamble{note}%
      {\CYRZ\cyra\cyrm\cyrii\cyrt\cyrk\cyra}%
      {\CYRZ\cyra\cyrm\cyrii\cyrt\cyrk\cyri}%
    \Crefname@preamble{algorithm}%
      {\CYRA\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm}%
      {\CYRA\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm\cyri}%
    \Crefname@preamble{listing}%
      {\CYRL\cyrii\cyrs\cyrt\cyri\cyrn\cyrg}%
      {\CYRL\cyrii\cyrs\cyrt\cyri\cyrn\cyrg\cyri}%
    \Crefname@preamble{line}%
      {\CYRS\cyrt\cyrr\cyro\cyrk\cyra}%
      {\CYRS\cyrt\cyrr\cyro\cyrk\cyri}%
    \Crefname@preamble{page}%
      {\CYRS\cyrt\cyro\cyrr\cyri\cyrn\cyrk\cyra}%
      {\CYRS\cyrt\cyro\cyrr\cyrii\cyrn\cyrk\cyri}%
    \Crefname@preamble{part}%
      {\CYRCH\cyra\cyrs\cyrt\cyri\cyrn\cyra}%
      {\CYRCH\cyra\cyrs\cyrt\cyri\cyrn\cyri}%
 %
    \if@cref@capitalise%  capitalise set
      \if@cref@abbrev%  abbrev set
        \crefname@preamble{equation}%
          {\CYRF-\cyrl.}%
          {\CYRF-\cyrl.}%
        \crefname@preamble{figure}%
          {\CYRR\cyri\cyrs.}%
          {\CYRR\cyri\cyrs.}%
        \crefname@preamble{table}%
          {\CYRT\cyra\cyrb\cyrl.}%
          {\CYRT\cyra\cyrb\cyrl.}%
        \crefname@preamble{enumi}%
          {\CYRP.}%
          {\CYRP.\cyrp.}%
      \else%
        \crefname@preamble{equation}%
          {\CYRF\cyro\cyrr\cyrm\cyru\cyrl\cyra}%
          {\CYRF\cyro\cyrr\cyrm\cyru\cyrl\cyri}%
        \crefname@preamble{figure}%
          {\CYRR\cyri\cyrs\cyru\cyrn\cyro\cyrk}%
          {\CYRR\cyri\cyrs\cyru\cyrn\cyrk\cyri}%
        \crefname@preamble{table}%
          {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyrya}%
          {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyrii}%
        \crefname@preamble{enumi}%
          {\CYRP\cyru\cyrn\cyrk\cyrt}%
          {\CYRP\cyru\cyrn\cyrk\cyrt\cyri}%
      \fi%
      \crefname@preamble{chapter}%
        {\CYRG\cyrl\cyra\cyrv\cyra}%
        {\CYRG\cyrl\cyra\cyrv\cyri}%
      \crefname@preamble{section}%
        {\CYRR\cyro\cyrz\cyrd\cyrii\cyrl}%
        {\CYRR\cyro\cyrz\cyrd\cyrii\cyrl\cyri}%
      \crefname@preamble{appendix}%
        {\CYRD\cyro\cyrd\cyra\cyrt\cyro\cyrk}%
        {\CYRD\cyro\cyrd\cyra\cyrt\cyrk\cyri}%
      \crefname@preamble{footnote}%
        {\CYRV\cyri\cyrn\cyro\cyrs\cyrk\cyra}%
        {\CYRV\cyri\cyrn\cyro\cyrs\cyrk\cyri}%
      \crefname@preamble{theorem}%
        {\CYRT\cyre\cyro\cyrr\cyre\cyrm\cyra}%
        {\CYRT\cyre\cyro\cyrr\cyre\cyrm\cyri}%
      \crefname@preamble{lemma}%
        {\CYRL\cyre\cyrm\cyrm\cyra}%
        {\CYRL\cyre\cyrm\cyrm\cyri}%
      \crefname@preamble{corollary}%
        {\CYRV\cyri\cyrs\cyrn\cyro\cyrv\cyro\cyrk}%
        {\CYRV\cyri\cyrs\cyrn\cyro\cyrv\cyrk\cyri}%
      \crefname@preamble{proposition}%
        {\CYRT\cyrv\cyre\cyrr\cyrd\cyrzh\cyre\cyrn\cyrn\cyrya}%
        {\CYRT\cyrv\cyre\cyrr\cyrd\cyrzh\cyre\cyrn\cyrn\cyrya}%
      \crefname@preamble{definition}%
        {\CYRV\cyri\cyrz\cyrn\cyra\cyrch\cyre\cyrn\cyrn\cyrya}%
        {\CYRV\cyri\cyrz\cyrn\cyra\cyrch\cyre\cyrn\cyrn\cyrya}%
      \crefname@preamble{result}%
        {\CYRR\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt}%
        {\CYRR\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt\cyri}%
      \crefname@preamble{example}%
        {\CYRP\cyrr\cyri\cyrk\cyrl\cyra\cyrd}%
        {\CYRP\cyrr\cyri\cyrk\cyrl\cyra\cyrd\cyri}%
      \crefname@preamble{remark}%
        {\CYRP\cyrr\cyri\cyrm\cyrii\cyrt\cyrk\cyra}%
        {\CYRP\cyrr\cyri\cyrm\cyrii\cyrt\cyrk\cyri}%
      \crefname@preamble{note}%
        {\CYRZ\cyra\cyrm\cyrii\cyrt\cyrk\cyra}%
        {\CYRZ\cyra\cyrm\cyrii\cyrt\cyrk\cyri}%
      \crefname@preamble{algorithm}%
        {\CYRA\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm}%
        {\CYRA\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm\cyri}%
      \crefname@preamble{listing}%
        {\CYRL\cyrii\cyrs\cyrt\cyri\cyrn\cyrg}%
        {\CYRL\cyrii\cyrs\cyrt\cyri\cyrn\cyrg\cyri}%
      \crefname@preamble{line}%
        {\CYRS\cyrt\cyrr\cyro\cyrk\cyra}%
        {\CYRS\cyrt\cyrr\cyro\cyrk\cyri}%
      \crefname@preamble{page}%
        {\CYRS\cyrt\cyro\cyrr\cyri\cyrn\cyrk\cyra}%
        {\CYRS\cyrt\cyro\cyrr\cyrii\cyrn\cyrk\cyri}%
      \crefname@preamble{part}%
        {\CYRCH\cyra\cyrs\cyrt\cyri\cyrn\cyra}%
        {\CYRCH\cyra\cyrs\cyrt\cyri\cyrn\cyri}%
 %
    \else%  capitalise unset
      \if@cref@abbrev%  abbrev set
        \crefname@preamble{equation}%
          {\cyrf-\cyrl.}%
          {\cyrf-\cyrl.}%
        \crefname@preamble{figure}%
          {\cyrr\cyri\cyrs.}%
          {\cyrr\cyri\cyrs.}%
        \crefname@preamble{table}%
          {\cyrt\cyra\cyrb\cyrl.}%
          {\cyrt\cyra\cyrb\cyrl.}%
        \crefname@preamble{enumi}%
          {\cyrp.}%
          {\cyrp.\cyrp.}%
        \crefname@preamble{chapter}%
          {\cyrg\cyrl\cyra\cyrv.}%
          {\cyrg\cyrl\cyra\cyrv.}%
        \crefname@preamble{section}%
          {\cyrr\cyro\cyrz\cyrd.}%
          {\cyrr\cyro\cyrz\cyrd\cyrii\cyrl.}%
        \crefname@preamble{appendix}%
          {\cyrd\cyro\cyrd\cyra\cyrt.}%
          {\cyrd\cyro\cyrd\cyra\cyrt\cyrk.}%
        \crefname@preamble{footnote}%
          {\cyrv\cyri\cyrn\cyro\cyrs\cyrk.}%
          {\cyrv\cyri\cyrn\cyro\cyrs\cyrk.}%
        \crefname@preamble{theorem}%
          {\cyrt\cyre\cyro\cyrr\cyre\cyrm.}%
          {\cyrt\cyre\cyro\cyrr\cyre\cyrm.}%
        \crefname@preamble{lemma}%
          {\cyrl\cyre\cyrm\cyrm.}%
          {\cyrl\cyre\cyrm\cyrm.}%
        \crefname@preamble{corollary}%
          {\cyrv\cyri\cyrs\cyrn\cyro\cyrv.}%
          {\cyrv\cyri\cyrs\cyrn\cyro\cyrv\cyrk.}%
        \crefname@preamble{proposition}%
          {\cyrt\cyrv\cyre\cyrr\cyrd\cyrzh\cyre\cyrn\cyrn.}%
          {\cyrt\cyrv\cyre\cyrr\cyrd\cyrzh\cyre\cyrn\cyrn.}%
        \crefname@preamble{definition}%
          {\cyrv\cyri\cyrz\cyrn\cyra\cyrch\cyre\cyrn\cyrn.}%
          {\cyrv\cyri\cyrz\cyrn\cyra\cyrch\cyre\cyrn\cyrn.}%
        \crefname@preamble{result}%
          {\cyrr\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt.}%
          {\cyrr\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt.}%
        \crefname@preamble{example}%
          {\cyrp\cyrr\cyri\cyrk\cyrl.}%
          {\cyrp\cyrr\cyri\cyrk\cyrl\cyra\cyrd.}%
        \crefname@preamble{remark}%
          {\cyrp\cyrr\cyri\cyrm\cyrii\cyrt.}%
          {\cyrp\cyrr\cyri\cyrm\cyrii\cyrt.}%
        \crefname@preamble{note}%
          {\cyrz\cyra\cyrm\cyrii\cyrt.}%
          {\cyrz\cyra\cyrm\cyrii\cyrt.}%
        \crefname@preamble{algorithm}%
          {\cyra\cyrl\cyrg.}%
          {\cyra\cyrl\cyrg.}%
        \crefname@preamble{listing}%
          {\cyrl\cyrii\cyrs\cyrt\cyri\cyrn.}%
          {\cyrl\cyrii\cyrs\cyrt\cyri\cyrn\cyrg.}%
        \crefname@preamble{line}%
          {\cyrs\cyrt\cyrr\cyrk.}%
          {\cyrs\cyrt\cyrr\cyrk.}%
      \else%  abbrev unset
        \crefname@preamble{equation}%
          {\cyrf\cyro\cyrr\cyrm\cyru\cyrl\cyra}%
          {\cyrf\cyro\cyrr\cyrm\cyru\cyrl\cyri}%
        \crefname@preamble{figure}%
          {\cyrr\cyri\cyrs\cyru\cyrn\cyro\cyrk}%
          {\cyrr\cyri\cyrs\cyru\cyrn\cyrk\cyri}%
        \crefname@preamble{table}%
          {\cyrt\cyra\cyrb\cyrl\cyri\cyrc\cyrya}%
          {\cyrt\cyra\cyrb\cyrl\cyri\cyrc\cyrii}%
        \crefname@preamble{enumi}%
          {\cyrp\cyru\cyrn\cyrk\cyrt}%
          {\cyrp\cyru\cyrn\cyrk\cyrt\cyri}%
        \crefname@preamble{chapter}%
          {\cyrg\cyrl\cyra\cyrv\cyra}%
          {\cyrg\cyrl\cyra\cyrv\cyri}%
        \crefname@preamble{section}%
          {\cyrr\cyro\cyrz\cyrd\cyrii\cyrl}%
          {\cyrr\cyro\cyrz\cyrd\cyrii\cyrl\cyri}%
        \crefname@preamble{appendix}%
          {\cyrd\cyro\cyrd\cyra\cyrt\cyro\cyrk}%
          {\cyrd\cyro\cyrd\cyra\cyrt\cyrk\cyri}%
        \crefname@preamble{footnote}%
          {\cyrv\cyri\cyrn\cyro\cyrs\cyrk\cyra}%
          {\cyrv\cyri\cyrn\cyro\cyrs\cyrk\cyri}%
        \crefname@preamble{theorem}%
          {\cyrt\cyre\cyro\cyrr\cyre\cyrm\cyra}%
          {\cyrt\cyre\cyro\cyrr\cyre\cyrm\cyri}%
        \crefname@preamble{lemma}%
          {\cyrl\cyre\cyrm\cyrm\cyra}%
          {\cyrl\cyre\cyrm\cyrm\cyri}%
        \crefname@preamble{corollary}%
          {\cyrv\cyri\cyrs\cyrn\cyro\cyrv\cyro\cyrk}%
          {\cyrv\cyri\cyrs\cyrn\cyro\cyrv\cyrk\cyri}%
        \crefname@preamble{proposition}%
          {\cyrt\cyrv\cyre\cyrr\cyrd\cyrzh\cyre\cyrn\cyrn\cyrya}%
          {\cyrt\cyrv\cyre\cyrr\cyrd\cyrzh\cyre\cyrn\cyrn\cyrya}%
        \crefname@preamble{definition}%
          {\cyrv\cyri\cyrz\cyrn\cyra\cyrch\cyre\cyrn\cyrn\cyrya}%
          {\cyrv\cyri\cyrz\cyrn\cyra\cyrch\cyre\cyrn\cyrn\cyrya}%
        \crefname@preamble{result}%
          {\cyrr\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt}%
          {\cyrr\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt\cyri}%
        \crefname@preamble{example}%
          {\cyrp\cyrr\cyri\cyrk\cyrl\cyra\cyrd}%
          {\cyrp\cyrr\cyri\cyrk\cyrl\cyra\cyrd\cyri}%
        \crefname@preamble{remark}%
          {\cyrp\cyrr\cyri\cyrm\cyrii\cyrt\cyrk\cyra}%
          {\cyrp\cyrr\cyri\cyrm\cyrii\cyrt\cyrk\cyri}%
        \crefname@preamble{note}%
          {\cyrz\cyra\cyrm\cyrii\cyrt\cyrk\cyra}%
          {\cyrz\cyra\cyrm\cyrii\cyrt\cyrk\cyri}%
        \crefname@preamble{algorithm}%
          {\cyra\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm}%
          {\cyra\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm\cyri}%
        \crefname@preamble{listing}%
          {\cyrl\cyrii\cyrs\cyrt\cyri\cyrn\cyrg}%
          {\cyrl\cyrii\cyrs\cyrt\cyri\cyrn\cyrg\cyri}%
        \crefname@preamble{line}%
          {\cyrs\cyrt\cyrr\cyro\cyrk\cyra}%
          {\cyrs\cyrt\cyrr\cyro\cyrk\cyri}%
      \fi%
      \crefname@preamble{page}%
        {\cyrs\cyrt\cyro\cyrr\cyri\cyrn\cyrc\cyrii}%
        {\cyrs\cyrt\cyro\cyrr\cyrii\cyrn\cyrk\cyra\cyrh}%
      \crefname@preamble{part}%
        {\cyrch\cyra\cyrs\cyrt\cyri\cyrn\cyra}%
        {\cyrch\cyra\cyrs\cyrt\cyri\cyrn\cyri}%
    \fi%
    \def\cref@language{ukrainian}%
    \cref@addto\extrasukrainian{%
      \renewcommand{\crefrangeconjunction}{--}%
      \renewcommand\crefrangepreconjunction{}%
      \renewcommand\crefrangepostconjunction{}%
      \renewcommand{\crefpairconjunction}{ \cyrii\nobreakspace}%
      \renewcommand{\crefmiddleconjunction}{, }%
      \renewcommand{\creflastconjunction}{ \cyrii\nobreakspace}%
      \renewcommand{\crefpairgroupconjunction}%
        { \cyrt\cyra\nobreakspace}%
      \renewcommand{\crefmiddlegroupconjunction}{, }%
      \renewcommand{\creflastgroupconjunction}%
        {, \cyra\ \cyrt\cyra\cyrk\cyro\cyrzh\nobreakspace}%
 %
        \Crefname{equation}%
        {\CYRF\cyro\cyrr\cyrm\cyru\cyrl\cyra}%
        {\CYRF\cyro\cyrr\cyrm\cyru\cyrl\cyri}%
      \Crefname{figure}%
        {\CYRR\cyri\cyrs\cyru\cyrn\cyro\cyrk}%
        {\CYRR\cyri\cyrs\cyru\cyrn\cyrk\cyri}%
      \Crefname{subfigure}%
        {\CYRR\cyri\cyrs\cyru\cyrn\cyro\cyrk}%
        {\CYRR\cyri\cyrs\cyru\cyrn\cyrk\cyri}%
      \Crefname{table}%
        {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyrya}%
        {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyrii}%
      \Crefname{subtable}%
        {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyrya}%
        {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyrii}%
      \Crefname{enumi}%
        {\CYRP\cyru\cyrn\cyrk\cyrt}%
        {\CYRP\cyru\cyrn\cyrk\cyrt\cyri}%
      \Crefname{enumii}%
        {\CYRP\cyru\cyrn\cyrk\cyrt}%
        {\CYRP\cyru\cyrn\cyrk\cyrt\cyri}%
      \Crefname{enumiii}%
        {\CYRP\cyru\cyrn\cyrk\cyrt}%
        {\CYRP\cyru\cyrn\cyrk\cyrt\cyri}%
      \Crefname{enumiv}%
        {\CYRP\cyru\cyrn\cyrk\cyrt}%
        {\CYRP\cyru\cyrn\cyrk\cyrt\cyri}%
      \Crefname{enumv}%
        {\CYRP\cyru\cyrn\cyrk\cyrt}%
        {\CYRP\cyru\cyrn\cyrk\cyrt\cyri}%
      \Crefname{chapter}%
        {\CYRG\cyrl\cyra\cyrv\cyra}%
        {\CYRG\cyrl\cyra\cyrv\cyri}%
      \Crefname{section}%
        {\CYRR\cyro\cyrz\cyrd\cyrii\cyrl}%
        {\CYRR\cyro\cyrz\cyrd\cyrii\cyrl\cyri}%
      \Crefname{subsection}%
        {\CYRR\cyro\cyrz\cyrd\cyrii\cyrl}%
        {\CYRR\cyro\cyrz\cyrd\cyrii\cyrl\cyri}%
      \Crefname{subsubsection}%
        {\CYRR\cyro\cyrz\cyrd\cyrii\cyrl}%
        {\CYRR\cyro\cyrz\cyrd\cyrii\cyrl\cyri}%
      \Crefname{appendix}%
        {\CYRD\cyro\cyrd\cyra\cyrt\cyro\cyrk}%
        {\CYRD\cyro\cyrd\cyra\cyrt\cyrk\cyri}%
      \Crefname{subappendix}%
        {\CYRD\cyro\cyrd\cyra\cyrt\cyro\cyrk}%
        {\CYRD\cyro\cyrd\cyra\cyrt\cyrk\cyri}%
      \Crefname{subsubappendix}%
        {\CYRD\cyro\cyrd\cyra\cyrt\cyro\cyrk}%
        {\CYRD\cyro\cyrd\cyra\cyrt\cyrk\cyri}%
      \Crefname{subsubsubappendix}%
        {\CYRD\cyro\cyrd\cyra\cyrt\cyro\cyrk}%
        {\CYRD\cyro\cyrd\cyra\cyrt\cyrk\cyri}%
      \Crefname{footnote}%
        {\CYRV\cyri\cyrn\cyro\cyrs\cyrk\cyra}%
        {\CYRV\cyri\cyrn\cyro\cyrs\cyrk\cyri}%
      \Crefname{theorem}%
        {\CYRT\cyre\cyro\cyrr\cyre\cyrm\cyra}%
        {\CYRT\cyre\cyro\cyrr\cyre\cyrm\cyri}%
      \Crefname{lemma}%
        {\CYRL\cyre\cyrm\cyrm\cyra}%
        {\CYRL\cyre\cyrm\cyrm\cyri}%
      \Crefname{corollary}%
        {\CYRV\cyri\cyrs\cyrn\cyro\cyrv\cyro\cyrk}%
        {\CYRV\cyri\cyrs\cyrn\cyro\cyrv\cyrk\cyri}%
      \Crefname{proposition}%
        {\CYRT\cyrv\cyre\cyrr\cyrd\cyrzh\cyre\cyrn\cyrn\cyrya}%
        {\CYRT\cyrv\cyre\cyrr\cyrd\cyrzh\cyre\cyrn\cyrn\cyrya}%
      \Crefname{definition}%
        {\CYRV\cyri\cyrz\cyrn\cyra\cyrch\cyre\cyrn\cyrn\cyrya}%
        {\CYRV\cyri\cyrz\cyrn\cyra\cyrch\cyre\cyrn\cyrn\cyrya}%
      \Crefname{result}%
        {\CYRR\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt}%
        {\CYRR\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt\cyri}%
      \Crefname{example}%
        {\CYRP\cyrr\cyri\cyrk\cyrl\cyra\cyrd}%
        {\CYRP\cyrr\cyri\cyrk\cyrl\cyra\cyrd\cyri}%
      \Crefname{remark}%
        {\CYRP\cyrr\cyri\cyrm\cyrii\cyrt\cyrk\cyra}%
        {\CYRP\cyrr\cyri\cyrm\cyrii\cyrt\cyrk\cyri}%
      \Crefname{note}%
        {\CYRZ\cyra\cyrm\cyrii\cyrt\cyrk\cyra}%
        {\CYRZ\cyra\cyrm\cyrii\cyrt\cyrk\cyri}%
      \Crefname{algorithm}%
        {\CYRA\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm}%
        {\CYRA\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm\cyri}%
      \Crefname{listing}%
        {\CYRL\cyrii\cyrs\cyrt\cyri\cyrn\cyrg}%
        {\CYRL\cyrii\cyrs\cyrt\cyri\cyrn\cyrg\cyri}%
      \Crefname{line}%
        {\CYRS\cyrt\cyrr\cyro\cyrk\cyra}%
        {\CYRS\cyrt\cyrr\cyro\cyrk\cyri}%
      \Crefname{page}%
        {\CYRS\cyrt\cyro\cyrr\cyri\cyrn\cyrk\cyra}%
        {\CYRS\cyrt\cyro\cyrr\cyrii\cyrn\cyrk\cyri}%
      \Crefname{part}%
        {\CYRCH\cyra\cyrs\cyrt\cyri\cyrn\cyra}%
        {\CYRCH\cyra\cyrs\cyrt\cyri\cyrn\cyri}%
 %
      \if@cref@capitalise%  capitalise set
        \if@cref@abbrev%  abbrev set
          \crefname{equation}%
            {\CYRF-\cyrl.}%
            {\CYRF-\cyrl.}%
          \crefname{figure}%
            {\CYRR\cyri\cyrs.}%
            {\CYRR\cyri\cyrs.}%
          \crefname{subfigure}%
            {\CYRR\cyri\cyrs.}%
            {\CYRR\cyri\cyrs.}%
          \crefname{table}%
            {\CYRT\cyra\cyrb\cyrl.}%
            {\CYRT\cyra\cyrb\cyrl.}%
          \crefname{subtable}%
            {\CYRT\cyra\cyrb\cyrl.}%
            {\CYRT\cyra\cyrb\cyrl.}%
          \crefname{enumi}%
            {\CYRP.}%
            {\CYRP.\cyrp.}%
          \crefname{enumii}%
            {\CYRP.}%
            {\CYRP.\cyrp.}%
          \crefname{enumiii}%
            {\CYRP.}%
            {\CYRP.\cyrp.}%
          \crefname{enumiv}%
            {\CYRP.}%
            {\CYRP.\cyrp.}%
          \crefname{enumv}%
            {\CYRP.}%
            {\CYRP.\cyrp.}%
        \else%  abbrev unset
          \crefname{equation}%
            {\CYRF\cyro\cyrr\cyrm\cyru\cyrl\cyra}%
            {\CYRF\cyro\cyrr\cyrm\cyru\cyrl\cyri}%
          \crefname{figure}%
            {\CYRR\cyri\cyrs\cyru\cyrn\cyro\cyrk}%
            {\CYRR\cyri\cyrs\cyru\cyrn\cyrk\cyri}%
          \crefname{subfigure}%
            {\CYRR\cyri\cyrs\cyru\cyrn\cyro\cyrk}%
            {\CYRR\cyri\cyrs\cyru\cyrn\cyrk\cyri}%
          \crefname{table}%
            {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyrya}%
            {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyrii}%
          \crefname{subtable}%
            {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyrya}%
            {\CYRT\cyra\cyrb\cyrl\cyri\cyrc\cyrii}%
          \crefname{enumi}%
            {\CYRP\cyru\cyrn\cyrk\cyrt}%
            {\CYRP\cyru\cyrn\cyrk\cyrt\cyri}%
          \crefname{enumii}%
            {\CYRP\cyru\cyrn\cyrk\cyrt}%
            {\CYRP\cyru\cyrn\cyrk\cyrt\cyri}%
          \crefname{enumiii}%
            {\CYRP\cyru\cyrn\cyrk\cyrt}%
            {\CYRP\cyru\cyrn\cyrk\cyrt\cyri}%
          \crefname{enumiv}%
            {\CYRP\cyru\cyrn\cyrk\cyrt}%
            {\CYRP\cyru\cyrn\cyrk\cyrt\cyri}%
          \crefname{enumv}%
            {\CYRP\cyru\cyrn\cyrk\cyrt}%
            {\CYRP\cyru\cyrn\cyrk\cyrt\cyri}%
        \fi%
        \crefname{chapter}%
          {\CYRG\cyrl\cyra\cyrv\cyra}%
          {\CYRG\cyrl\cyra\cyrv\cyri}%
        \crefname{section}%
          {\CYRR\cyro\cyrz\cyrd\cyrii\cyrl}%
          {\CYRR\cyro\cyrz\cyrd\cyrii\cyrl\cyri}%
        \crefname{subsection}%
          {\CYRR\cyro\cyrz\cyrd\cyrii\cyrl}%
          {\CYRR\cyro\cyrz\cyrd\cyrii\cyrl\cyri}%
        \crefname{subsubsection}%
          {\CYRR\cyro\cyrz\cyrd\cyrii\cyrl}%
          {\CYRR\cyro\cyrz\cyrd\cyrii\cyrl\cyri}%
        \crefname{appendix}%
          {\CYRD\cyro\cyrd\cyra\cyrt\cyro\cyrk}%
          {\CYRD\cyro\cyrd\cyra\cyrt\cyrk\cyri}%
        \crefname{subappendix}%
          {\CYRD\cyro\cyrd\cyra\cyrt\cyro\cyrk}%
          {\CYRD\cyro\cyrd\cyra\cyrt\cyrk\cyri}%
        \crefname{subsubappendix}%
          {\CYRD\cyro\cyrd\cyra\cyrt\cyro\cyrk}%
          {\CYRD\cyro\cyrd\cyra\cyrt\cyrk\cyri}%
        \crefname{subsubsubappendix}%
          {\CYRD\cyro\cyrd\cyra\cyrt\cyro\cyrk}%
          {\CYRD\cyro\cyrd\cyra\cyrt\cyrk\cyri}%
        \crefname{footnote}%
          {\CYRV\cyri\cyrn\cyro\cyrs\cyrk\cyra}%
          {\CYRV\cyri\cyrn\cyro\cyrs\cyrk\cyri}%
        \crefname{theorem}%
          {\CYRT\cyre\cyro\cyrr\cyre\cyrm\cyra}%
          {\CYRT\cyre\cyro\cyrr\cyre\cyrm\cyri}%
        \crefname{lemma}%
          {\CYRL\cyre\cyrm\cyrm\cyra}%
          {\CYRL\cyre\cyrm\cyrm\cyri}%
        \crefname{corollary}%
          {\CYRV\cyri\cyrs\cyrn\cyro\cyrv\cyro\cyrk}%
          {\CYRV\cyri\cyrs\cyrn\cyro\cyrv\cyrk\cyri}%
        \crefname{proposition}%
          {\CYRT\cyrv\cyre\cyrr\cyrd\cyrzh\cyre\cyrn\cyrn\cyrya}%
          {\CYRT\cyrv\cyre\cyrr\cyrd\cyrzh\cyre\cyrn\cyrn\cyrya}%
        \crefname{definition}%
          {\CYRV\cyri\cyrz\cyrn\cyra\cyrch\cyre\cyrn\cyrn\cyrya}%
          {\CYRV\cyri\cyrz\cyrn\cyra\cyrch\cyre\cyrn\cyrn\cyrya}%
        \crefname{result}%
          {\CYRR\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt}%
          {\CYRR\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt\cyri}%
        \crefname{example}%
          {\CYRP\cyrr\cyri\cyrk\cyrl\cyra\cyrd}%
          {\CYRP\cyrr\cyri\cyrk\cyrl\cyra\cyrd\cyri}%
        \crefname{remark}%
          {\CYRP\cyrr\cyri\cyrm\cyrii\cyrt\cyrk\cyra}%
          {\CYRP\cyrr\cyri\cyrm\cyrii\cyrt\cyrk\cyri}%
        \crefname{note}%
          {\CYRZ\cyra\cyrm\cyrii\cyrt\cyrk\cyra}%
          {\CYRZ\cyra\cyrm\cyrii\cyrt\cyrk\cyri}%
        \crefname{algorithm}%
          {\CYRA\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm}%
          {\CYRA\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm\cyri}%
        \crefname{listing}%
          {\CYRL\cyrii\cyrs\cyrt\cyri\cyrn\cyrg}%
          {\CYRL\cyrii\cyrs\cyrt\cyri\cyrn\cyrg\cyri}%
        \crefname{line}%
          {\CYRS\cyrt\cyrr\cyro\cyrk\cyra}%
          {\CYRS\cyrt\cyrr\cyro\cyrk\cyri}%
        \crefname{page}%
          {\CYRS\cyrt\cyro\cyrr\cyri\cyrn\cyrk\cyra}%
          {\CYRS\cyrt\cyro\cyrr\cyrii\cyrn\cyrk\cyri}%
        \crefname{part}%
          {\CYRCH\cyra\cyrs\cyrt\cyri\cyrn\cyra}%
          {\CYRCH\cyra\cyrs\cyrt\cyri\cyrn\cyri}%
 %
      \else%  capitalise unset
        \if@cref@abbrev%  abbrev set
          \crefname{equation}%
            {\cyrf-\cyrl.}%
            {\cyrf-\cyrl.}%
          \crefname{chapter}%
            {\cyrg\cyrl\cyra\cyrv.}%
            {\cyrg\cyrl\cyra\cyrv.}%
          \crefname{section}%
            {\cyrr\cyro\cyrz\cyrd.}%
            {\cyrr\cyro\cyrz\cyrd\cyrii\cyrl.}%
          \crefname{subsection}%
            {\cyrr\cyro\cyrz\cyrd.}%
            {\cyrr\cyro\cyrz\cyrd\cyrii\cyrl.}%
          \crefname{subsubsection}%
            {\cyrr\cyro\cyrz\cyrd.}%
            {\cyrr\cyro\cyrz\cyrd\cyrii\cyrl.}%
          \crefname{appendix}%
            {\cyrd\cyro\cyrd\cyra\cyrt.}%
            {\cyrd\cyro\cyrd\cyra\cyrt\cyrk.}%
          \crefname{subappendix}%
            {\cyrd\cyro\cyrd\cyra\cyrt.}%
            {\cyrd\cyro\cyrd\cyra\cyrt\cyrk.}%
          \crefname{subsubappendix}%
            {\cyrd\cyro\cyrd\cyra\cyrt.}%
            {\cyrd\cyro\cyrd\cyra\cyrt\cyrk.}%
          \crefname{subsubsubappendix}%
            {\cyrd\cyro\cyrd\cyra\cyrt.}%
            {\cyrd\cyro\cyrd\cyra\cyrt\cyrk.}%
          \crefname{enumi}%
            {\cyrp.}%
            {\cyrp.\cyrp.}%
          \crefname{enumii}%
            {\cyrp.}%
            {\cyrp.\cyrp.}%
          \crefname{enumiii}%
            {\cyrp.}%
            {\cyrp.\cyrp.}%
          \crefname{enumiv}%
            {\cyrp.}%
            {\cyrp.\cyrp.}%
          \crefname{enumv}%
            {\cyrp.}%
            {\cyrp.\cyrp.}%
          \crefname{footnote}%
            {\cyrv\cyri\cyrn\cyro\cyrs\cyrk.}%
            {\cyrv\cyri\cyrn\cyro\cyrs\cyrk.}%
          \crefname{figure}%
            {\cyrr\cyri\cyrs.}%
            {\cyrr\cyri\cyrs.}%
          \crefname{subfigure}%
            {\cyrr\cyri\cyrs.}%
            {\cyrr\cyri\cyrs.}%
          \crefname{table}%
            {\cyrt\cyra\cyrb\cyrl.}%
            {\cyrt\cyra\cyrb\cyrl.}%
          \crefname{subtable}%
            {\cyrt\cyra\cyrb\cyrl.}%
            {\cyrt\cyra\cyrb\cyrl.}%
          \crefname{theorem}%
            {\cyrt\cyre\cyro\cyrr\cyre\cyrm.}%
            {\cyrt\cyre\cyro\cyrr\cyre\cyrm.}%
          \crefname{lemma}%
            {\cyrl\cyre\cyrm\cyrm.}%
            {\cyrl\cyre\cyrm\cyrm.}%
          \crefname{corollary}%
            {\cyrv\cyri\cyrs\cyrn\cyro\cyrv.}%
            {\cyrv\cyri\cyrs\cyrn\cyro\cyrv\cyrk.}%
          \crefname{proposition}%
            {\cyrt\cyrv\cyre\cyrr\cyrd\cyrzh\cyre\cyrn\cyrn.}%
            {\cyrt\cyrv\cyre\cyrr\cyrd\cyrzh\cyre\cyrn\cyrn.}%
          \crefname{definition}%
            {\cyrv\cyri\cyrz\cyrn\cyra\cyrch\cyre\cyrn\cyrn.}%
            {\cyrv\cyri\cyrz\cyrn\cyra\cyrch\cyre\cyrn\cyrn.}%
          \crefname{result}%
            {\cyrr\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt.}%
            {\cyrr\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt.}%
          \crefname{example}%
            {\cyrp\cyrr\cyri\cyrk\cyrl.}%
            {\cyrp\cyrr\cyri\cyrk\cyrl\cyra\cyrd.}%
          \crefname{remark}%
            {\cyrp\cyrr\cyri\cyrm\cyrii\cyrt.}%
            {\cyrp\cyrr\cyri\cyrm\cyrii\cyrt.}%
          \crefname{note}%
            {\cyrz\cyra\cyrm\cyrii\cyrt.}%
            {\cyrz\cyra\cyrm\cyrii\cyrt.}%
          \crefname{algorithm}%
            {\cyra\cyrl\cyrg.}%
            {\cyra\cyrl\cyrg.}%
          \crefname{listing}%
            {\cyrl\cyrii\cyrs\cyrt\cyri\cyrn.}%
            {\cyrl\cyrii\cyrs\cyrt\cyri\cyrn\cyrg.}%
          \crefname{line}%
            {\cyrs\cyrt\cyrr\cyrk.}%
            {\cyrs\cyrt\cyrr\cyrk.}%
        \else%  abbrev unset
          \crefname{equation}%
            {\cyrf\cyro\cyrr\cyrm\cyru\cyrl\cyra}%
            {\cyrf\cyro\cyrr\cyrm\cyru\cyrl\cyri}%
          \crefname{figure}%
            {\cyrr\cyri\cyrs\cyru\cyrn\cyro\cyrk}%
            {\cyrr\cyri\cyrs\cyru\cyrn\cyrk\cyri}%
          \crefname{subfigure}%
            {\cyrr\cyri\cyrs\cyru\cyrn\cyro\cyrk}%
            {\cyrr\cyri\cyrs\cyru\cyrn\cyrk\cyri}%
          \crefname{table}%
            {\cyrt\cyra\cyrb\cyrl\cyri\cyrc\cyrya}%
            {\cyrt\cyra\cyrb\cyrl\cyri\cyrc\cyrii}%
          \crefname{subtable}%
            {\cyrt\cyra\cyrb\cyrl\cyri\cyrc\cyrya}%
            {\cyrt\cyra\cyrb\cyrl\cyri\cyrc\cyrii}%
          \crefname{enumi}%
            {\cyrp\cyru\cyrn\cyrk\cyrt}%
            {\cyrp\cyru\cyrn\cyrk\cyrt\cyri}%
          \crefname{enumii}%
            {\cyrp\cyru\cyrn\cyrk\cyrt}%
            {\cyrp\cyru\cyrn\cyrk\cyrt\cyri}%
          \crefname{enumiii}%
            {\cyrp\cyru\cyrn\cyrk\cyrt}%
            {\cyrp\cyru\cyrn\cyrk\cyrt\cyri}%
          \crefname{enumiv}%
            {\cyrp\cyru\cyrn\cyrk\cyrt}%
            {\cyrp\cyru\cyrn\cyrk\cyrt\cyri}%
          \crefname{enumv}%
            {\cyrp\cyru\cyrn\cyrk\cyrt}%
            {\cyrp\cyru\cyrn\cyrk\cyrt\cyri}%
          \crefname{chapter}%
            {\cyrg\cyrl\cyra\cyrv\cyra}%
            {\cyrg\cyrl\cyra\cyrv\cyri}%
          \crefname{section}%
            {\cyrr\cyro\cyrz\cyrd\cyrii\cyrl}%
            {\cyrr\cyro\cyrz\cyrd\cyrii\cyrl\cyri}%
          \crefname{subsection}%
            {\cyrr\cyro\cyrz\cyrd\cyrii\cyrl}%
            {\cyrr\cyro\cyrz\cyrd\cyrii\cyrl\cyri}%
          \crefname{subsubsection}%
            {\cyrr\cyro\cyrz\cyrd\cyrii\cyrl}%
            {\cyrr\cyro\cyrz\cyrd\cyrii\cyrl\cyri}%
          \crefname{appendix}%
            {\cyrd\cyro\cyrd\cyra\cyrt\cyro\cyrk}%
            {\cyrd\cyro\cyrd\cyra\cyrt\cyrk\cyri}%
          \crefname{subappendix}%
            {\cyrd\cyro\cyrd\cyra\cyrt\cyro\cyrk}%
            {\cyrd\cyro\cyrd\cyra\cyrt\cyrk\cyri}%
          \crefname{subsubappendix}%
            {\cyrd\cyro\cyrd\cyra\cyrt\cyro\cyrk}%
            {\cyrd\cyro\cyrd\cyra\cyrt\cyrk\cyri}%
          \crefname{subsubsubappendix}%
            {\cyrd\cyro\cyrd\cyra\cyrt\cyro\cyrk}%
            {\cyrd\cyro\cyrd\cyra\cyrt\cyrk\cyri}%
          \crefname{footnote}%
            {\cyrv\cyri\cyrn\cyro\cyrs\cyrk\cyra}%
            {\cyrv\cyri\cyrn\cyro\cyrs\cyrk\cyri}%
          \crefname{theorem}%
            {\cyrt\cyre\cyro\cyrr\cyre\cyrm\cyra}%
            {\cyrt\cyre\cyro\cyrr\cyre\cyrm\cyri}%
          \crefname{lemma}%
            {\cyrl\cyre\cyrm\cyrm\cyra}%
            {\cyrl\cyre\cyrm\cyrm\cyri}%
          \crefname{corollary}%
            {\cyrv\cyri\cyrs\cyrn\cyro\cyrv\cyro\cyrk}%
            {\cyrv\cyri\cyrs\cyrn\cyro\cyrv\cyrk\cyri}%
          \crefname{proposition}%
            {\cyrt\cyrv\cyre\cyrr\cyrd\cyrzh\cyre\cyrn\cyrn\cyrya}%
            {\cyrt\cyrv\cyre\cyrr\cyrd\cyrzh\cyre\cyrn\cyrn\cyrya}%
          \crefname{definition}%
            {\cyrv\cyri\cyrz\cyrn\cyra\cyrch\cyre\cyrn\cyrn\cyrya}%
            {\cyrv\cyri\cyrz\cyrn\cyra\cyrch\cyre\cyrn\cyrn\cyrya}%
          \crefname{result}%
            {\cyrr\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt}%
            {\cyrr\cyre\cyrz\cyru\cyrl\cyrsftsn\cyrt\cyra\cyrt\cyri}%
          \crefname{example}%
            {\cyrp\cyrr\cyri\cyrk\cyrl\cyra\cyrd}%
            {\cyrp\cyrr\cyri\cyrk\cyrl\cyra\cyrd\cyri}%
          \crefname{remark}%
            {\cyrp\cyrr\cyri\cyrm\cyrii\cyrt\cyrk\cyra}%
            {\cyrp\cyrr\cyri\cyrm\cyrii\cyrt\cyrk\cyri}%
          \crefname{note}%
            {\cyrz\cyra\cyrm\cyrii\cyrt\cyrk\cyra}%
            {\cyrz\cyra\cyrm\cyrii\cyrt\cyrk\cyri}%
          \crefname{algorithm}%
            {\cyra\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm}%
            {\cyra\cyrl\cyrg\cyro\cyrr\cyri\cyrt\cyrm\cyri}%
          \crefname{listing}%
            {\cyrl\cyrii\cyrs\cyrt\cyri\cyrn\cyrg}%
            {\cyrl\cyrii\cyrs\cyrt\cyri\cyrn\cyrg\cyri}%
          \crefname{line}%
            {\cyrs\cyrt\cyrr\cyro\cyrk\cyra}%
            {\cyrs\cyrt\cyrr\cyro\cyrk\cyri}%
        \fi%
        \crefname{page}%
          {\cyrs\cyrt\cyro\cyrr\cyri\cyrn\cyrc\cyrii}%
          {\cyrs\cyrt\cyro\cyrr\cyrii\cyrn\cyrk\cyra\cyrh}%
        \crefname{part}%
          {\cyrch\cyra\cyrs\cyrt\cyri\cyrn\cyra}%
          {\cyrch\cyra\cyrs\cyrt\cyri\cyrn\cyri}%
      \fi%
    }}}
\DeclareOption{norsk}{%
  \PackageInfo{cleveref}{loaded norsk language definitions}
  \AtBeginDocument{%
    \def\crefrangeconjunction@preamble{ til\nobreakspace}%
    \def\crefrangepreconjunction@preamble{}%
    \def\crefrangepostconjunction@preamble{}%
    \def\crefpairconjunction@preamble{ og\nobreakspace}%
    \def\crefmiddleconjunction@preamble{, }%
    \def\creflastconjunction@preamble{ og\nobreakspace}%
    \def\crefpairgroupconjunction@preamble{ og\nobreakspace}%
    \def\crefmiddlegroupconjunction@preamble{, }%
    \def\creflastgroupconjunction@preamble{ og\nobreakspace}%
 %
    \Crefname@preamble{equation}{Likning}{Likningene}%
    \Crefname@preamble{figure}{Figur}{Figurene}%
    \Crefname@preamble{table}{Tabell}{Tabellene}%
    \Crefname@preamble{page}{Side}{Siden}%
    \Crefname@preamble{part}{Del}{Delene}%
    \Crefname@preamble{chapter}{Kapittel}{Kapitlene}%
    \Crefname@preamble{section}{Avsnitt}{Avsnittene}%
    \Crefname@preamble{appendix}{Tillegg}{Tilleggene}%
    \Crefname@preamble{enumi}{Punkt}{Punktene}%
    \Crefname@preamble{footnote}{Fotnote}{Fotnotene}%
    \Crefname@preamble{theorem}{Teorem}{Teoremene}%
    \Crefname@preamble{lemma}{Lemma}{Lemma}%
    \Crefname@preamble{corollary}{Korollar}{Korollarene}%
    \Crefname@preamble{proposition}{P\aa stand}{P\aa standene}%
    \Crefname@preamble{definition}{Definisjon}{Definisjonene}%
    \Crefname@preamble{result}{Resultat}{Resultatene}%
    \Crefname@preamble{example}{Eksempel}{Eksemplene}%
    \Crefname@preamble{remark}{Bemerkning}{Bemerkningene}%
    \Crefname@preamble{note}{Note}{Notene}%
    \Crefname@preamble{algorithm}{Algoritme}{Algoritmene}%
    \Crefname@preamble{listing}{Opplisting}{Opplistingene}%
    \Crefname@preamble{line}{Linje}{Linjene}%
 %
    \if@cref@capitalise%
      \crefname@preamble{page}{Side}{Siden}%
      \crefname@preamble{equation}{Likning}{Likningene}%
      \crefname@preamble{figure}{Figur}{Figurene}%
      \crefname@preamble{table}{Tabell}{Tabellene}%
      \crefname@preamble{part}{Del}{Delene}%
      \crefname@preamble{chapter}{Kapittel}{Kapitlene}%
      \crefname@preamble{section}{Avsnitt}{Avsnittene}%
      \crefname@preamble{appendix}{Tillegg}{Tilleggene}%
      \crefname@preamble{enumi}{Punkt}{Punktene}%
      \crefname@preamble{footnote}{Fotnote}{Fotnotene}%
      \crefname@preamble{theorem}{Teorem}{Teoremene}%
      \crefname@preamble{lemma}{Lemma}{Lemma}%
      \crefname@preamble{corollary}{Korollar}{Korollarene}%
      \crefname@preamble{proposition}{P\aa stand}{P\aa standene}%
      \crefname@preamble{definition}{Definisjon}{Definisjonene}%
      \crefname@preamble{result}{Resultat}{Resultatene}%
      \crefname@preamble{example}{Eksempel}{Eksemplene}%
      \crefname@preamble{remark}{Bemerkning}{Bemerkningene}%
      \crefname@preamble{note}{Note}{Notene}%
      \crefname@preamble{algorithm}{Algoritme}{Algoritmene}%
      \crefname@preamble{listing}{Opplisting}{Opplistingene}%
      \crefname@preamble{line}{Linje}{Linjene}%
 %
    \else%
      \crefname@preamble{equation}{likning}{likningene}%
      \crefname@preamble{figure}{figur}{figurene}%
      \crefname@preamble{table}{tabell}{tabeller}%
      \crefname@preamble{page}{side}{siden}%
      \crefname@preamble{part}{del}{delene}%
      \crefname@preamble{chapter}{kapittel}{kapitlene}%
      \crefname@preamble{section}{avsnitt}{avsnittene}%
      \crefname@preamble{appendix}{tillegg}{tilleggene}%
      \crefname@preamble{enumi}{punkt}{punktene}%
      \crefname@preamble{footnote}{fotnote}{fotnotene}%
      \crefname@preamble{theorem}{teorem}{teoremene}%
      \crefname@preamble{lemma}{lemma}{lemma}%
      \crefname@preamble{corollary}{korollar}{korollarene}%
      \crefname@preamble{proposition}{p\aa stand}{p\aa standene}%
      \crefname@preamble{definition}{definisjon}{definisjonene}%
      \crefname@preamble{result}{resultat}{resultatene}%
      \crefname@preamble{example}{eksempel}{eksemplene}%
      \crefname@preamble{remark}{bemerkning}{bemerkningene}%
      \crefname@preamble{note}{note}{notene}%
      \crefname@preamble{algorithm}{algoritme}{algoritmene}%
      \crefname@preamble{listing}{opplisting}{opplistingene}%
      \crefname@preamble{line}{linje}{linjene}%
    \fi%
    \def\cref@language{norsk}%
    \cref@addto\extrasnorsk{%
      \renewcommand{\crefrangeconjunction}{ til\nobreakspace}%
      \renewcommand\crefrangepreconjunction{}%
      \renewcommand\crefrangepostconjunction{}%
      \renewcommand{\crefpairconjunction}{ og\nobreakspace}%
      \renewcommand{\crefmiddleconjunction}{, }%
      \renewcommand{\creflastconjunction}{ og\nobreakspace}%
      \renewcommand{\crefpairgroupconjunction}{ og\nobreakspace}%
      \renewcommand{\crefmiddlegroupconjunction}{, }%
      \renewcommand{\creflastgroupconjunction}{ og\nobreakspace}%
 %
      \Crefname{equation}{Likning}{Likningene}%
      \Crefname{figure}{Figur}{Figurene}%
      \Crefname{subfigure}{Figur}{Figurene}%
      \Crefname{table}{Tabell}{Tabellene}%
      \Crefname{subtable}{Tabell}{Tabellene}%
      \Crefname{page}{Side}{Siden}%
      \Crefname{part}{Del}{Delene}%
      \Crefname{chapter}{Kapittel}{Kapitlene}%
      \Crefname{section}{Avsnitt}{Avsnittene}%
      \Crefname{subsection}{Avsnitt}{Avsnittene}%
      \Crefname{subsubsection}{Avsnitt}{Avsnittene}%
      \Crefname{appendix}{Tillegg}{Tilleggene}%
      \Crefname{subappendix}{Tillegg}{Tilleggene}%
      \Crefname{subsubappendix}{Tillegg}{Tilleggene}%
      \Crefname{subsubsubappendix}{Tillegg}{Tilleggene}%
      \Crefname{enumi}{Punkt}{Punktene}%
      \Crefname{enumii}{Punkt}{Punktene}%
      \Crefname{enumiii}{Punkt}{Punktene}%
      \Crefname{enumiv}{Punkt}{Punktene}%
      \Crefname{enumv}{Punkt}{Punktene}%
      \Crefname{footnote}{Fotnote}{Fotnotene}%
      \Crefname{theorem}{Teorem}{Teoremene}%
      \Crefname{lemma}{Lemma}{Lemma}%
      \Crefname{corollary}{Korollar}{Korollarene}%
      \Crefname{proposition}{P\aa stand}{P\aa standene}%
      \Crefname{definition}{Definisjon}{Definisjonene}%
      \Crefname{result}{Resultat}{Resultatene}%
      \Crefname{example}{Eksempel}{Eksemplene}%
      \Crefname{remark}{Bemerkning}{Bemerkningene}%
      \Crefname{note}{Note}{Notene}%
      \Crefname{algorithm}{Algoritme}{Algoritmene}%
      \Crefname{listing}{Opplisting}{Opplistingene}%
      \Crefname{line}{Linje}{Linjene}%
 %
      \if@cref@capitalise%
        \crefname{equation}{Likning}{Likningene}%
        \crefname{figure}{Figur}{Figurene}%
        \crefname{subfigure}{Figur}{Figurene}%
        \crefname{table}{Tabell}{Tabellene}%
        \crefname{subtable}{Tabell}{Tabellene}%
        \crefname{page}{Side}{Siden}%
        \crefname{part}{Del}{Delene}%
        \crefname{chapter}{Kapittel}{Kapitlene}%
        \crefname{section}{Avsnitt}{Avsnittene}%
        \crefname{subsection}{Avsnitt}{Avsnittene}%
        \crefname{subsubsection}{Avsnitt}{Avsnittene}%
        \crefname{appendix}{Tillegg}{Tilleggene}%
        \crefname{subappendix}{Tillegg}{Tilleggene}%
        \crefname{subsubappendix}{Tillegg}{Tilleggene}%
        \crefname{subsubsubappendix}{Tillegg}{Tilleggene}%
        \crefname{enumi}{Punkt}{Punktene}%
        \crefname{enumii}{Punkt}{Punktene}%
        \crefname{enumiii}{Punkt}{Punktene}%
        \crefname{enumiv}{Punkt}{Punktene}%
        \crefname{enumv}{Punkt}{Punktene}%
        \crefname{footnote}{Fotnote}{Fotnotene}%
        \crefname{theorem}{Teorem}{Teoremene}%
        \crefname{lemma}{Lemma}{Lemma}%
        \crefname{corollary}{Korollar}{Korollarene}%
        \crefname{proposition}{P\aa stand}{P\aa standene}%
        \crefname{definition}{Definisjon}{Definisjonene}%
        \crefname{result}{Resultat}{Resultatene}%
        \crefname{example}{Eksempel}{Eksemplene}%
        \crefname{remark}{Bemerkning}{Bemerkningene}%
        \crefname{note}{Note}{Notene}%
        \crefname{algorithm}{Algoritme}{Algoritmene}%
        \crefname{listing}{Opplisting}{Opplistingene}%
        \crefname{line}{Linje}{Linjene}%
 %
      \else%
        \crefname{equation}{likning}{likningene}%
        \crefname{figure}{figur}{figurene}%
        \crefname{subfigure}{figur}{figurene}%
        \crefname{table}{tabell}{tabellene}%
        \crefname{subtable}{tabell}{tabellene}%
        \crefname{page}{side}{siden}%
        \crefname{part}{del}{delene}%
        \crefname{chapter}{kapittel}{kapitlene}%
        \crefname{section}{avsnitt}{avsnittene}%
        \crefname{subsection}{avsnitt}{avsnittene}%
        \crefname{subsubsection}{avsnitt}{avsnittene}%
        \crefname{appendix}{tillegg}{tilleggene}%
        \crefname{subappendix}{tillegg}{tilleggene}%
        \crefname{subsubappendix}{tillegg}{tilleggene}%
        \crefname{subsubsubappendix}{tillegg}{tilleggene}%
        \crefname{enumi}{punkt}{punktene}%
        \crefname{enumii}{punkt}{punktene}%
        \crefname{enumiii}{punkt}{punktene}%
        \crefname{enumiv}{punkt}{punktene}%
        \crefname{enumv}{punkt}{punktene}%
        \crefname{footnote}{fotnote}{fotnotene}%
        \crefname{theorem}{teorem}{teoremene}%
        \crefname{lemma}{lemma}{lemma}%
        \crefname{corollary}{korollar}{korollarene}%
        \crefname{proposition}{p\aa stand}{p\aa standene}%
        \crefname{definition}{definisjon}{definisjonene}%
        \crefname{result}{resultat}{resultatene}%
        \crefname{example}{eksempel}{eksemplene}%
        \crefname{remark}{bemerkning}{bemerkningene}%
        \crefname{note}{note}{notene}%
        \crefname{algorithm}{algoritme}{algoritmene}%
        \crefname{listing}{opplisting}{opplistingene}%
        \crefname{line}{linje}{linjene}%
      \fi%
    }}}
\DeclareOption{danish}{%
  \PackageInfo{cleveref}{loaded danish language definitions}
  \AtBeginDocument{%
    \def\crefrangeconjunction@preamble{ til\nobreakspace}%
    \def\crefrangepreconjunction@preamble{}%
    \def\crefrangepostconjunction@preamble{}%
    \def\crefpairconjunction@preamble{ og\nobreakspace}%
    \def\crefmiddleconjunction@preamble{, }%
    \def\creflastconjunction@preamble{ og\nobreakspace}%
    \def\crefpairgroupconjunction@preamble{ og\nobreakspace}%
    \def\crefmiddlegroupconjunction@preamble{, }%
    \def\creflastgroupconjunction@preamble{ og\nobreakspace}%
 %
    \Crefname@preamble{equation}{Ligning}{Ligninger}%
    \Crefname@preamble{figure}{Figur}{Figurer}%
    \Crefname@preamble{table}{Tabel}{Tabeller}%
    \Crefname@preamble{page}{Side}{Sider}%
    \Crefname@preamble{part}{Del}{Dele}%
    \Crefname@preamble{chapter}{Kapitel}{Kapitler}%
    \Crefname@preamble{section}{Afsnit}{Afsnit}%
    \Crefname@preamble{appendix}{Appendiks}{Appendiks}%
    \Crefname@preamble{enumi}{Punkt}{Punkter}%
    \Crefname@preamble{footnote}{Fodnote}{Fodnoter}%
    \Crefname@preamble{theorem}{Teorem}{Teoremer}%
    \Crefname@preamble{lemma}{Lemma}{Lemma}%
    \Crefname@preamble{corollary}{F\o lgeslutning}{F\o lgeslutninger}%
    \Crefname@preamble{proposition}{Udsagn}{Udsagn}%
    \Crefname@preamble{definition}{Definition}{Definitioner}%
    \Crefname@preamble{result}{Resultat}{Resultater}%
    \Crefname@preamble{example}{Eksempel}{Eksempler}%
    \Crefname@preamble{remark}{Bem\ae rkning}{Bem\ae rkninger}%
    \Crefname@preamble{note}{Note}{Noter}%
    \Crefname@preamble{algorithm}{Algoritme}{Algoritmer}%
    \Crefname@preamble{line}{Linje}{Linjer}%
 %
    \if@cref@capitalise%
      \crefname@preamble{equation}{Ligning}{Ligninger}%
      \crefname@preamble{figure}{Figur}{Figurer}%
      \crefname@preamble{table}{Tabel}{Tabeller}%
      \crefname@preamble{page}{Side}{Sider}%
      \crefname@preamble{part}{Del}{Dele}%
      \crefname@preamble{chapter}{Kapitel}{Kapitler}%
      \crefname@preamble{section}{Afsnit}{Afsnit}%
      \crefname@preamble{appendix}{Appendiks}{Appendiks}%
      \crefname@preamble{enumi}{Punkt}{Punkter}%
      \crefname@preamble{footnote}{Fodnote}{Fodnoter}%
      \crefname@preamble{theorem}{Teorem}{Teoremer}%
      \crefname@preamble{lemma}{Lemma}{Lemma}%
      \crefname@preamble{corollary}{F\o lgeslutning}{F\o lgeslutninger}%
      \crefname@preamble{proposition}{Udsagn}{Udsagn}%
      \crefname@preamble{definition}{Definition}{Definitioner}%
      \crefname@preamble{result}{Resultat}{Resultater}%
      \crefname@preamble{example}{Eksempel}{Eksempler}%
      \crefname@preamble{remark}{Bem\ae rkning}{Bem\ae rkninger}%
      \crefname@preamble{note}{Note}{Noter}%
      \crefname@preamble{algorithm}{Algoritme}{Algoritmer}%
      \crefname@preamble{line}{Linje}{Linjer}%
 %
    \else%
      \crefname@preamble{equation}{ligning}{ligninger}%
      \crefname@preamble{figure}{figur}{figurer}%
      \crefname@preamble{table}{tabel}{tabeller}%
      \crefname@preamble{page}{side}{sider}%
      \crefname@preamble{part}{del}{dele}%
      \crefname@preamble{chapter}{kapitel}{kapitler}%
      \crefname@preamble{section}{afsnit}{afsnit}%
      \crefname@preamble{appendix}{appendiks}{appendiks}%
      \crefname@preamble{enumi}{punkt}{punkter}%
      \crefname@preamble{footnote}{fodnote}{fodnoter}%
      \crefname@preamble{theorem}{teorem}{teoremer}%
      \crefname@preamble{lemma}{lemma}{lemma}%
      \crefname@preamble{corollary}{f\o lgeslutning}{f\o lgeslutninger}%
      \crefname@preamble{proposition}{udsagn}{udsagn}%
      \crefname@preamble{definition}{definition}{definitioner}%
      \crefname@preamble{result}{resultat}{resultater}%
      \crefname@preamble{example}{eksempel}{eksempler}%
      \crefname@preamble{remark}{bem\ae rkning}{bem\ae rkninger}%
      \crefname@preamble{note}{note}{noter}%
      \crefname@preamble{algorithm}{algoritme}{algoritmer}%
      \crefname@preamble{line}{linje}{linjer}%
    \fi%
    \def\cref@language{danish}%
    \cref@addto\extrasdanish{%
    \renewcommand{\crefrangeconjunction@preamble}{ til\nobreakspace}%
    \renewcommand\crefrangepreconjunction@preamble{}%
    \renewcommand\crefrangepostconjunction@preamble{}%
    \renewcommand{\crefpairconjunction@preamble}{ og\nobreakspace}%
    \renewcommand{\crefmiddleconjunction@preamble}{, }%
    \renewcommand{\creflastconjunction@preamble}{ og\nobreakspace}%
    \renewcommand{\crefpairgroupconjunction@preamble}{ og\nobreakspace}%
    \renewcommand{\crefmiddlegroupconjunction@preamble}{, }%
    \renewcommand{\creflastgroupconjunction@preamble}{ og\nobreakspace}%
 %
    \Crefname{equation}{Ligning}{Ligninger}%
    \Crefname{figure}{Figur}{Figurer}%
    \Crefname{subfigure}{Figur}{Figurer}%
    \Crefname{table}{Tabel}{Tabeller}%
    \Crefname{subtable}{Tabel}{Tabeller}%
    \Crefname{page}{Side}{Sider}%
    \Crefname{part}{Del}{Dele}%
    \Crefname{chapter}{Kapitel}{Kapitler}%
    \Crefname{section}{Afsnit}{Afsnit}%
    \Crefname{subsection}{Afsnit}{Afsnit}%
    \Crefname{subsubsection}{Afsnit}{Afsnit}%
    \Crefname{appendix}{Appendiks}{Appendiks}%
    \Crefname{subappendix}{Appendiks}{Appendiks}%
    \Crefname{subsubappendix}{Appendiks}{Appendiks}%
    \Crefname{subsubsubappendix}{Appendiks}{Appendiks}%
    \Crefname{enumi}{Punkt}{Punkter}%
    \Crefname{enumii}{Punkt}{Punkter}%
    \Crefname{enumiii}{Punkt}{Punkter}%
    \Crefname{enumiv}{Punkt}{Punkter}%
    \Crefname{enumv}{Punkt}{Punkter}%
    \Crefname{footnote}{Fodnote}{Fodnoter}%
    \Crefname{theorem}{Teorem}{Teoremer}%
    \Crefname{lemma}{Lemma}{Lemma}%
    \Crefname{corollary}{F\o lgeslutning}{F\o lgeslutninger}%
    \Crefname{proposition}{Udsagn}{Udsagn}%
    \Crefname{definition}{Definition}{Definitioner}%
    \Crefname{result}{Resultat}{Resultater}%
    \Crefname{example}{Eksempel}{Eksempler}%
    \Crefname{remark}{Bem\ae rkning}{Bem\ae rkninger}%
    \Crefname{note}{Note}{Noter}%
    \Crefname{algorithm}{Algoritme}{Algoritmer}%
    \Crefname{line}{Linje}{Linjer}%
 %
    \if@cref@capitalise%
      \crefname{equation}{Ligning}{Ligninger}%
      \crefname{figure}{Figur}{Figurer}%
      \crefname{subfigure}{Figur}{Figurer}%
      \crefname{table}{Tabel}{Tabeller}%
      \crefname{subtable}{Tabel}{Tabeller}%
      \crefname{page}{Side}{Sider}%
      \crefname{part}{Del}{Dele}%
      \crefname{chapter}{Kapitel}{Kapitler}%
      \crefname{section}{Afsnit}{Afsnit}%
      \crefname{subsection}{Afsnit}{Afsnit}%
      \crefname{subsubsection}{Afsnit}{Afsnit}%
      \crefname{appendix}{Appendiks}{Appendiks}%
      \crefname{subappendix}{Appendiks}{Appendiks}%
      \crefname{subsubappendix}{Appendiks}{Appendiks}%
      \crefname{subsubsubappendix}{Appendiks}{Appendiks}%
      \crefname{enumi}{Punkt}{Punkter}%
      \crefname{enumii}{Punkt}{Punkter}%
      \crefname{enumiii}{Punkt}{Punkter}%
      \crefname{enumiv}{Punkt}{Punkter}%
      \crefname{enumv}{Punkt}{Punkter}%
      \crefname{footnote}{Fodnote}{Fodnoter}%
      \crefname{theorem}{Teorem}{Teoremer}%
      \crefname{lemma}{Lemma}{Lemma}%
      \crefname{corollary}{F\o lgeslutning}{F\o lgeslutninger}%
      \crefname{proposition}{Udsagn}{Udsagn}%
      \crefname{definition}{Definition}{Definitioner}%
      \crefname{result}{Resultat}{Resultater}%
      \crefname{example}{Eksempel}{Eksempler}%
      \crefname{remark}{Bem\ae rkning}{Bem\ae rkninger}%
      \crefname{note}{Note}{Noter}%
      \crefname{algorithm}{Algoritme}{Algoritmer}%
      \crefname{line}{Linje}{Linjer}%
 %
    \else%
      \crefname{equation}{ligning}{ligninger}%
      \crefname{figure}{figur}{figurer}%
      \crefname{subfigure}{figur}{figurer}%
      \crefname{table}{tabel}{tabeller}%
      \crefname{subtable}{tabel}{tabeller}%
      \crefname{page}{side}{sider}%
      \crefname{part}{del}{dele}%
      \crefname{chapter}{kapitel}{kapitler}%
      \crefname{section}{afsnit}{afsnit}%
      \crefname{subsection}{afsnit}{afsnit}%
      \crefname{subsubsection}{afsnit}{afsnit}%
      \crefname{appendix}{appendiks}{appendiks}%
      \crefname{subappendix}{appendiks}{appendiks}%
      \crefname{subsubappendix}{appendiks}{appendiks}%
      \crefname{subsubsubappendix}{appendiks}{appendiks}%
      \crefname{enumi}{punkt}{punkter}%
      \crefname{enumii}{punkt}{punkter}%
      \crefname{enumiii}{punkt}{punkter}%
      \crefname{enumiv}{punkt}{punkter}%
      \crefname{enumv}{punkt}{punkter}%
      \crefname{footnote}{fodnote}{fodnoter}%
      \crefname{theorem}{teorem}{teoremer}%
      \crefname{lemma}{lemma}{lemma}%
      \crefname{corollary}{f\o lgeslutning}{f\o lgeslutninger}%
      \crefname{proposition}{udsagn}{udsagn}%
      \crefname{definition}{definition}{definitioner}%
      \crefname{result}{resultat}{resultater}%
      \crefname{example}{eksempel}{eksempler}%
      \crefname{remark}{bem\ae rkning}{bem\ae rkninger}%
      \crefname{note}{note}{noter}%
      \crefname{algorithm}{algoritme}{algoritmer}%
      \crefname{line}{linje}{linjer}%
      \fi%
    }}}
\edef\@curroptions{\@ptionlist{\@currname.\@currext}}%
\@expandtwoargs\in@{,capitalise,}{%
  ,\@classoptionslist,\@curroptions,}%
\ifin@%
  \ExecuteOptions{capitalise}%
\else%
  \@expandtwoargs\in@{,capitalize,}{%
    ,\@classoptionslist,\@curroptions,}%
  \ifin@%
    \ExecuteOptions{capitalise}%
  \fi%
\fi%
\@expandtwoargs\in@{,nameinlink,}{%
  ,\@classoptionslist,\@curroptions,}%
\ifin@%
  \ExecuteOptions{nameinlink}%
\fi%
\crefdefaultlabelformat{#2#1#3}
\if@cref@nameinlink%
  \creflabelformat{equation}{#2\textup{(#1)}#3}%
\else%
  \creflabelformat{equation}{\textup{(#2#1#3)}}%
\fi
\@labelcrefdefinedefaultformats
\ExecuteOptions{english}
\ProcessOptions*\relax
\AtBeginDocument{%
  \edef\@tempa{%
    \expandafter\noexpand\csname extras\cref@language\endcsname}%
  \@ifundefined{crefrangeconjunction}{%
    \let\crefrangeconjunction\crefrangeconjunction@preamble%
  }{%
    \expandafter\def\expandafter\@tempb\expandafter{%
      \expandafter\renewcommand\expandafter%
      {\expandafter\crefrangeconjunction\expandafter}%
      \expandafter{\crefrangeconjunction}}%
    \expandafter\expandafter\expandafter\cref@addto%
      \expandafter\@tempa\expandafter{\@tempb}%
  }%
  \@ifundefined{crefrangepreconjunction}{%
    \let\crefrangepreconjunction\crefrangepreconjunction@preamble%
  }{%
    \expandafter\def\expandafter\@tempb\expandafter{%
      \expandafter\renewcommand\expandafter%
      {\expandafter\crefrangepreconjunction\expandafter}%
      \expandafter{\crefrangepreconjunction}}%
    \expandafter\expandafter\expandafter\cref@addto%
      \expandafter\@tempa\expandafter{\@tempb}%
  }%
  \@ifundefined{crefrangepostconjunction}{%
    \let\crefrangepostconjunction\crefrangepostconjunction@preamble%
  }{%
    \expandafter\def\expandafter\@tempb\expandafter{%
      \expandafter\renewcommand\expandafter%
      {\expandafter\crefrangepostconjunction\expandafter}%
      \expandafter{\crefrangepostconjunction}}%
    \expandafter\expandafter\expandafter\cref@addto%
      \expandafter\@tempa\expandafter{\@tempb}%
  }%
  \@ifundefined{crefpairconjunction}{%
    \let\crefpairconjunction\crefpairconjunction@preamble%
  }{%
    \expandafter\def\expandafter\@tempb\expandafter{%
      \expandafter\renewcommand\expandafter%
      {\expandafter\crefpairconjunction\expandafter}%
      \expandafter{\crefpairconjunction}}%
    \expandafter\expandafter\expandafter\cref@addto%
      \expandafter\@tempa\expandafter{\@tempb}%
    \@ifundefined{crefpairgroupconjunction}{%
      \let\crefpairgroupconjunction\crefpairconjunction}{}%
  }%
  \@ifundefined{crefmiddleconjunction}{%
    \let\crefmiddleconjunction\crefmiddleconjunction@preamble%
  }{%
    \expandafter\def\expandafter\@tempb\expandafter{%
      \expandafter\renewcommand\expandafter%
      {\expandafter\crefmiddleconjunction\expandafter}%
      \expandafter{\crefmiddleconjunction}}%
    \expandafter\expandafter\expandafter\cref@addto%
      \expandafter\@tempa\expandafter{\@tempb}%
    \@ifundefined{crefmiddlegroupconjunction}{%
      \let\crefmiddlegroupconjunction\crefmiddleconjunction}{}%
  }%
  \@ifundefined{creflastconjunction}{%
    \let\creflastconjunction\creflastconjunction@preamble%
  }{%
    \expandafter\def\expandafter\@tempb\expandafter{%
      \expandafter\renewcommand\expandafter%
      {\expandafter\creflastconjunction\expandafter}%
      \expandafter{\creflastconjunction}}%
    \expandafter\expandafter\expandafter\cref@addto%
      \expandafter\@tempa\expandafter{\@tempb}%
    \@ifundefined{creflastgroupconjunction}{%
      \edef\creflastgroupconjunction{, \creflastconjunction}}{}%
  }%
  \@ifundefined{crefpairgroupconjunction}{%
    \let\crefpairgroupconjunction%
    \crefpairgroupconjunction@preamble%
  }{%
    \expandafter\def\expandafter\@tempb\expandafter{%
      \expandafter\renewcommand\expandafter%
      {\expandafter\crefpairgroupconjunction\expandafter}%
      \expandafter{\crefpairgroupconjunction}}%
    \expandafter\expandafter\expandafter\cref@addto%
      \expandafter\@tempa\expandafter{\@tempb}%
  }%
  \@ifundefined{crefmiddlegroupconjunction}{%
    \let\crefmiddlegroupconjunction%
      \crefmiddlegroupconjunction@preamble%
  }{%
    \expandafter\def\expandafter\@tempb\expandafter{%
      \expandafter\renewcommand\expandafter%
      {\expandafter\crefmiddlegroupconjunction\expandafter}%
      \expandafter{\crefmiddlegroupconjunction}}%
    \expandafter\expandafter\expandafter\cref@addto%
      \expandafter\@tempa\expandafter{\@tempb}%
  }%
  \@ifundefined{creflastgroupconjunction}{%
    \let\creflastgroupconjunction%
      \creflastgroupconjunction@preamble%
  }{%
    \expandafter\def\expandafter\@tempb\expandafter{%
      \expandafter\renewcommand\expandafter%
      {\expandafter\creflastgroupconjunction\expandafter}%
      \expandafter{\creflastgroupconjunction}}%
    \expandafter\expandafter\expandafter\cref@addto%
      \expandafter\@tempa\expandafter{\@tempb}%
  }%
  \let\@tempstack\cref@label@types%
  \cref@isstackfull{\@tempstack}%
  \@whilesw\if@cref@stackfull\fi{%
    \edef\@tempa{\cref@stack@top{\@tempstack}}%
    \@ifundefined{cref@\@tempa @name}{%
      \expandafter\def\expandafter\@tempb\expandafter{%
        \csname cref@\@tempa @name\endcsname}%
      \expandafter\def\expandafter\@tempc\expandafter{%
        \csname cref@\@tempa @name@preamble\endcsname}%
      \expandafter\expandafter\expandafter%
        \let\expandafter\@tempb\@tempc%
      \expandafter\def\expandafter\@tempb\expandafter{%
        \csname cref@\@tempa @name@plural\endcsname}%
      \expandafter\def\expandafter\@tempc\expandafter{%
        \csname cref@\@tempa @name@plural@preamble\endcsname}%
      \expandafter\expandafter\expandafter%
        \let\expandafter\@tempb\@tempc%
    }{%
      \edef\@tempb{%
        \expandafter\noexpand\csname extras\cref@language\endcsname}%
      \expandafter\def\expandafter\@tempc\expandafter{%
        \expandafter\crefname\expandafter{\@tempa}}%
      \expandafter\expandafter\expandafter\cref@addto%
      \expandafter\expandafter\expandafter\@tempc%
      \expandafter\expandafter\expandafter{%
        \expandafter\expandafter\expandafter{%
          \csname cref@\@tempa @name\endcsname}}%
      \expandafter\expandafter\expandafter\cref@addto%
      \expandafter\expandafter\expandafter\@tempc%
      \expandafter\expandafter\expandafter{%
        \expandafter\expandafter\expandafter{%
          \csname cref@\@tempa @name@plural\endcsname}}%
      \expandafter\expandafter\expandafter\cref@addto%
        \expandafter\@tempb\expandafter{\@tempc}%
    }%
    \@ifundefined{Cref@\@tempa @name}{%
      \expandafter\def\expandafter\@tempb\expandafter{%
        \csname Cref@\@tempa @name\endcsname}%
      \expandafter\def\expandafter\@tempc\expandafter{%
        \csname Cref@\@tempa @name@preamble\endcsname}%
      \expandafter\expandafter\expandafter%
        \let\expandafter\@tempb\@tempc%
      \expandafter\def\expandafter\@tempb\expandafter{%
        \csname Cref@\@tempa @name@plural\endcsname}%
      \expandafter\def\expandafter\@tempc\expandafter{%
        \csname Cref@\@tempa @name@plural@preamble\endcsname}%
      \expandafter\expandafter\expandafter%
        \let\expandafter\@tempb\@tempc%
    }{%
      \edef\@tempb{%
        \expandafter\noexpand\csname extras\cref@language\endcsname}%
      \expandafter\def\expandafter\@tempc\expandafter{%
        \expandafter\Crefname\expandafter{\@tempa}}%
      \expandafter\expandafter\expandafter\cref@addto%
      \expandafter\expandafter\expandafter\@tempc%
      \expandafter\expandafter\expandafter{%
        \expandafter\expandafter\expandafter{%
          \csname Cref@\@tempa @name\endcsname}}%
      \expandafter\expandafter\expandafter\cref@addto%
      \expandafter\expandafter\expandafter\@tempc%
      \expandafter\expandafter\expandafter{%
        \expandafter\expandafter\expandafter{%
          \csname Cref@\@tempa @name@plural\endcsname}}%
      \expandafter\expandafter\expandafter\cref@addto%
        \expandafter\@tempb\expandafter{\@tempc}%
    }%
    \@ifundefined{cref@\@tempa @format}{%
      \@ifundefined{cref@\@tempa @name}{}{%
        \expandafter\@crefdefineformat\expandafter{\@tempa}}}{}%
    \@ifundefined{crefrange@\@tempa @format}{%
      \@ifundefined{cref@\@tempa @name@plural}{}{%
        \expandafter\@crefrangedefineformat\expandafter{\@tempa}}}{}%
    \@ifundefined{cref@\@tempa @format@first}{%
      \@ifundefined{cref@\@tempa @name@plural}{}{%
        \expandafter\@crefdefinemultiformat\expandafter{\@tempa}}}{}%
    \@ifundefined{crefrange@\@tempa @format@first}{%
      \@ifundefined{cref@\@tempa @name@plural}{}{%
        \expandafter\@crefrangedefinemultiformat%
        \expandafter{\@tempa}}}{}%
    \cref@stack@pop{\@tempstack}%
    \cref@isstackfull{\@tempstack}}%
    \@ifundefined{cref@subsection@name}{%
      \let\cref@subsection@name\cref@section@name%
      \let\cref@subsection@name@plural\cref@section@name@plural}{}%
    \@ifundefined{Cref@subsection@name}{%
      \let\Cref@subsection@name\Cref@section@name%
      \let\Cref@subsection@name@plural\Cref@section@name@plural}{}%
    \@ifundefined{cref@subsection@format}{%
      \let\cref@subsection@format\cref@section@format}{}%
    \@ifundefined{Cref@subsection@format}{%
      \let\Cref@subsection@format\Cref@section@format}{}%
    \@ifundefined{crefrange@subsection@format}{%
      \let\crefrange@subsection@format%
      \crefrange@section@format}{}%
    \@ifundefined{Crefrange@subsection@format}{%
      \let\Crefrange@subsection@format%
      \Crefrange@section@format}{}%
    \@ifundefined{cref@subsection@format@first}{%
      \let\cref@subsection@format@first%
      \cref@section@format@first}{}%
    \@ifundefined{Cref@subsection@format@first}{%
      \let\Cref@subsection@format@first%
      \Cref@section@format@first}{}%
    \@ifundefined{cref@subsection@format@second}{%
      \let\cref@subsection@format@second%
      \cref@section@format@second}{}%
    \@ifundefined{Cref@subsection@format@second}{%
      \let\Cref@subsection@format@second%
      \Cref@section@format@second}{}%
    \@ifundefined{cref@subsection@format@middle}{%
      \let\cref@subsection@format@middle%
      \cref@section@format@middle}{}%
    \@ifundefined{Cref@subsection@format@middle}{%
      \let\Cref@subsection@format@middle%
      \Cref@section@format@middle}{}%
    \@ifundefined{cref@subsection@format@last}{%
      \let\cref@subsection@format@last%
      \cref@section@format@last}{}%
    \@ifundefined{Cref@subsection@format@last}{%
      \let\Cref@subsection@format@last%
      \Cref@section@format@last}{}%
    \@ifundefined{crefrange@subsection@format@first}{%
      \let\crefrange@subsection@format@first%
      \crefrange@section@format@first}{}%
    \@ifundefined{Crefrange@subsection@format@first}{%
      \let\Crefrange@subsection@format@first%
      \Crefrange@section@format@first}{}%
    \@ifundefined{crefrange@subsection@format@second}{%
      \let\crefrange@subsection@format@second%
      \crefrange@section@format@second}{}%
    \@ifundefined{Crefrange@subsection@format@second}{%
      \let\Crefrange@subsection@format@second%
      \Crefrange@section@format@second}{}%
    \@ifundefined{crefrange@subsection@format@middle}{%
      \let\crefrange@subsection@format@middle%
      \crefrange@section@format@middle}{}%
    \@ifundefined{Crefrange@subsection@format@middle}{%
      \let\Crefrange@subsection@format@middle%
      \Crefrange@section@format@middle}{}%
    \@ifundefined{crefrange@subsection@format@last}{%
      \let\crefrange@subsection@format@last%
      \crefrange@section@format@last}{}%
    \@ifundefined{Crefrange@subsection@format@last}{%
      \let\Crefrange@subsection@format@last%
      \Crefrange@section@format@last}{}%
    \@ifundefined{cref@subsubsection@name}{%
      \let\cref@subsubsection@name\cref@section@name%
      \let\cref@subsubsection@name@plural\cref@section@name@plural}{}%
    \@ifundefined{Cref@subsection@name}{%
      \let\Cref@subsection@name\Cref@section@name%
      \let\Cref@subsection@name@plural\Cref@section@name@plural}{}%
    \@ifundefined{cref@subsubsection@format}{%
      \let\cref@subsubsection@format%
      \cref@subsection@format}{}%
    \@ifundefined{Cref@subsubsection@format}{%
      \let\Cref@subsubsection@format%
      \Cref@subsection@format}{}%
    \@ifundefined{crefrange@subsubsection@format}{%
      \let\crefrange@subsubsection@format%
      \crefrange@subsection@format}{}%
    \@ifundefined{Crefrange@subsubsection@format}{%
      \let\Crefrange@subsubsection@format%
      \Crefrange@subsection@format}{}%
    \@ifundefined{cref@subsubsection@format@first}{%
      \let\cref@subsubsection@format@first%
      \cref@subsection@format@first}{}%
    \@ifundefined{Cref@subsubsection@format@first}{%
      \let\Cref@subsubsection@format@first%
      \Cref@subsection@format@first}{}%
    \@ifundefined{cref@subsubsection@format@second}{%
      \let\cref@subsubsection@format@second%
      \cref@subsection@format@second}{}%
    \@ifundefined{Cref@subsubsection@format@second}{%
      \let\Cref@subsubsection@format@second%
      \Cref@subsection@format@second}{}%
    \@ifundefined{cref@subsubsection@format@middle}{%
      \let\cref@subsubsection@format@middle%
      \cref@subsection@format@middle}{}%
    \@ifundefined{Cref@subsubsection@format@middle}{%
      \let\Cref@subsubsection@format@middle%
      \Cref@subsection@format@middle}{}%
    \@ifundefined{cref@subsubsection@format@last}{%
      \let\cref@subsubsection@format@last%
      \cref@subsection@format@last}{}%
    \@ifundefined{Cref@subsubsection@format@last}{%
      \let\Cref@subsubsection@format@last%
      \Cref@subsection@format@last}{}%
    \@ifundefined{crefrange@subsubsection@format@first}{%
      \let\crefrange@subsubsection@format@first%
      \crefrange@subsection@format@first}{}%
    \@ifundefined{Crefrange@subsubsection@format@first}{%
      \let\Crefrange@subsubsection@format@first%
      \Crefrange@subsection@format@first}{}%
    \@ifundefined{crefrange@subsubsection@format@second}{%
      \let\crefrange@subsubsection@format@second%
      \crefrange@subsection@format@second}{}%
    \@ifundefined{Crefrange@subsubsection@format@second}{%
      \let\Crefrange@subsubsection@format@second%
      \Crefrange@subsection@format@second}{}%
    \@ifundefined{crefrange@subsubsection@format@middle}{%
      \let\crefrange@subsubsection@format@middle%
      \crefrange@subsection@format@middle}{}%
    \@ifundefined{Crefrange@subsubsection@format@middle}{%
      \let\Crefrange@subsubsection@format@middle%
      \Crefrange@subsection@format@middle}{}%
    \@ifundefined{crefrange@subsubsection@format@last}{%
      \let\crefrange@subsubsection@format@last%
      \crefrange@subsection@format@last}{}%
    \@ifundefined{Crefrange@subsubsection@format@last}{%
      \let\Crefrange@subsubsection@format@last%
      \Crefrange@subsection@format@last}{}%
    \@ifundefined{cref@subappendix@name}{%
      \let\cref@subappendix@name\cref@appendix@name%
      \let\cref@subappendix@name@plural%
        \cref@appendix@name@plural}{}%
    \@ifundefined{Cref@subappendix@name}{%
      \let\Cref@subappendix@name\Cref@section@name%
      \let\Cref@subappendixsection@name@plural%
        \Cref@appendix@name@plural}{}%
    \@ifundefined{cref@subappendix@format}{%
      \let\cref@subappendix@format\cref@appendix@format}{}%
    \@ifundefined{Cref@subappendix@format}{%
      \let\Cref@subappendix@format\Cref@appendix@format}{}%
    \@ifundefined{crefrange@subappendix@format}{%
      \let\crefrange@subappendix@format%
      \crefrange@appendix@format}{}%
    \@ifundefined{Crefrange@subappendix@format}{%
      \let\Crefrange@subappendix@format%
      \Crefrange@appendix@format}{}%
    \@ifundefined{cref@subappendix@format@first}{%
      \let\cref@subappendix@format@first%
      \cref@appendix@format@first}{}%
    \@ifundefined{Cref@subappendix@format@first}{%
      \let\Cref@subappendix@format@first%
      \Cref@appendix@format@first}{}%
    \@ifundefined{cref@subappendix@format@second}{%
      \let\cref@subappendix@format@second%
      \cref@appendix@format@second}{}%
    \@ifundefined{Cref@subappendix@format@second}{%
      \let\Cref@subappendix@format@second%
      \Cref@appendix@format@second}{}%
    \@ifundefined{cref@subappendix@format@middle}{%
      \let\cref@subappendix@format@middle%
      \cref@appendix@format@middle}{}%
    \@ifundefined{Cref@subappendix@format@middle}{%
      \let\Cref@subappendix@format@middle%
      \Cref@appendix@format@middle}{}%
    \@ifundefined{cref@subappendix@format@last}{%
      \let\cref@subappendix@format@last%
      \cref@appendix@format@last}{}%
    \@ifundefined{Cref@subappendix@format@last}{%
      \let\Cref@subappendix@format@last%
      \Cref@appendix@format@last}{}%
    \@ifundefined{crefrange@subappendix@format@first}{%
      \let\crefrange@subappendix@format@first%
      \crefrange@appendix@format@first}{}%
    \@ifundefined{Crefrange@subappendix@format@first}{%
      \let\Crefrange@subappendix@format@first%
      \Crefrange@appendix@format@first}{}%
    \@ifundefined{crefrange@subappendix@format@second}{%
      \let\crefrange@subappendix@format@second%
      \crefrange@appendix@format@second}{}%
    \@ifundefined{Crefrange@subappendix@format@second}{%
      \let\Crefrange@subappendix@format@second%
      \Crefrange@appendix@format@second}{}%
    \@ifundefined{crefrange@subappendix@format@middle}{%
      \let\crefrange@subappendix@format@middle%
      \crefrange@appendix@format@middle}{}%
    \@ifundefined{Crefrange@subappendix@format@middle}{%
      \let\Crefrange@subappendix@format@middle%
      \Crefrange@appendix@format@middle}{}%
    \@ifundefined{crefrange@subappendix@format@last}{%
      \let\crefrange@subappendix@format@last%
      \crefrange@appendix@format@last}{}%
    \@ifundefined{Crefrange@subappendix@format@last}{%
      \let\Crefrange@subappendix@format@last%
      \Crefrange@appendix@format@last}{}%
    \@ifundefined{cref@subsubappendix@name}{%
      \let\cref@subsubappendix@name\cref@appendix@name%
      \let\cref@subsubappendix@name@plural%
        \cref@appendix@name@plural}{}%
    \@ifundefined{Cref@subsubappendix@name}{%
      \let\Cref@subsubappendix@name\Cref@section@name%
      \let\Cref@subsubappendixsection@name@plural%
        \Cref@appendix@name@plural}{}%
    \@ifundefined{cref@subsubappendix@format}{%
      \let\cref@subsubappendix@format%
      \cref@subappendix@format}{}%
    \@ifundefined{Cref@subsubappendix@format}{%
      \let\Cref@subsubappendix@format%
      \Cref@subappendix@format}{}%
    \@ifundefined{crefrange@subsubappendix@format}{%
      \let\crefrange@subsubappendix@format%
      \crefrange@subappendix@format}{}%
    \@ifundefined{Crefrange@subsubappendix@format}{%
      \let\Crefrange@subsubappendix@format%
      \Crefrange@subappendix@format}{}%
    \@ifundefined{cref@subsubappendix@format@first}{%
      \let\cref@subsubappendix@format@first%
      \cref@subappendix@format@first}{}%
    \@ifundefined{Cref@subsubappendix@format@first}{%
      \let\Cref@subsubappendix@format@first%
      \Cref@subappendix@format@first}{}%
    \@ifundefined{cref@subsubappendix@format@second}{%
      \let\cref@subsubappendix@format@second%
      \cref@subappendix@format@second}{}%
    \@ifundefined{Cref@subsubappendix@format@second}{%
      \let\Cref@subsubappendix@format@second%
      \Cref@subappendix@format@second}{}%
    \@ifundefined{cref@subsubappendix@format@middle}{%
      \let\cref@subsubappendix@format@middle%
      \cref@subappendix@format@middle}{}%
    \@ifundefined{Cref@subsubappendix@format@middle}{%
      \let\Cref@subsubappendix@format@middle%
      \Cref@subappendix@format@middle}{}%
    \@ifundefined{cref@subsubappendix@format@last}{%
      \let\cref@subsubappendix@format@last%
      \cref@subappendix@format@last}{}%
    \@ifundefined{Cref@subsubappendix@format@last}{%
      \let\Cref@subsubappendix@format@last%
      \Cref@subappendix@format@last}{}%
    \@ifundefined{crefrange@subsubappendix@format@first}{%
      \let\crefrange@subsubappendix@format@first%
      \crefrange@subappendix@format@first}{}%
    \@ifundefined{Crefrange@subsubappendix@format@first}{%
      \let\Crefrange@subsubappendix@format@first%
      \Crefrange@subappendix@format@first}{}%
    \@ifundefined{crefrange@subsubappendix@format@second}{%
      \let\crefrange@subsubappendix@format@second%
      \crefrange@subappendix@format@second}{}%
    \@ifundefined{Crefrange@subsubappendix@format@second}{%
      \let\Crefrange@subsubappendix@format@second%
      \Crefrange@subappendix@format@second}{}%
    \@ifundefined{crefrange@subsubappendix@format@middle}{%
      \let\crefrange@subsubappendix@format@middle%
      \crefrange@subappendix@format@middle}{}%
    \@ifundefined{Crefrange@subsubappendix@format@middle}{%
      \let\Crefrange@subsubappendix@format@middle%
      \Crefrange@subappendix@format@middle}{}%
    \@ifundefined{crefrange@subsubappendix@format@last}{%
      \let\crefrange@subsubappendix@format@last%
      \crefrange@subappendix@format@last}{}%
    \@ifundefined{Crefrange@subsubappendix@format@last}{%
      \let\Crefrange@subsubappendix@format@last%
      \Crefrange@subappendix@format@last}{}%
    \@ifundefined{cref@subsubsubappendix@format}{%
      \let\cref@subsubsubappendix@format%
      \cref@subsubappendix@format}{}%
    \@ifundefined{Cref@subsubsubappendix@format}{%
      \let\Cref@subsubsubappendix@format%
      \Cref@subsubappendix@format}{}%
    \@ifundefined{crefrange@subsubsubappendix@format}{%
      \let\crefrange@subsubsubappendix@format%
      \crefrange@subsubappendix@format}{}%
    \@ifundefined{Crefrange@subsubsubappendix@format}{%
      \let\Crefrange@subsubsubappendix@format%
      \Crefrange@subsubappendix@format}{}%
    \@ifundefined{cref@subsubsubappendix@format@first}{%
      \let\cref@subsubsubappendix@format@first%
      \cref@subsubappendix@format@first}{}%
    \@ifundefined{Cref@subsubsubappendix@format@first}{%
      \let\Cref@subsubsubappendix@format@first%
      \Cref@subsubappendix@format@first}{}%
    \@ifundefined{cref@subsubsubappendix@format@second}{%
      \let\cref@subsubsubappendix@format@second%
      \cref@subsubappendix@format@second}{}%
    \@ifundefined{Cref@subsubsubappendix@format@second}{%
      \let\Cref@subsubsubappendix@format@second%
      \Cref@subsubappendix@format@second}{}%
    \@ifundefined{cref@subsubsubappendix@format@middle}{%
      \let\cref@subsubsubappendix@format@middle%
      \cref@subsubappendix@format@middle}{}%
    \@ifundefined{Cref@subsubsubappendix@format@middle}{%
      \let\Cref@subsubsubappendix@format@middle%
      \Cref@subsubappendix@format@middle}{}%
    \@ifundefined{cref@subsubsubappendix@format@last}{%
      \let\cref@subsubsubappendix@format@last%
      \cref@subsubappendix@format@last}{}%
    \@ifundefined{Cref@subsubsubappendix@format@last}{%
      \let\Cref@subsubsubappendix@format@last%
      \Cref@subsubappendix@format@last}{}%
    \@ifundefined{crefrange@subsubsubappendix@format@first}{%
      \let\crefrange@subsubsubappendix@format@first%
      \crefrange@subsubappendix@format@first}{}%
    \@ifundefined{Crefrange@subsubsubappendix@format@first}{%
      \let\Crefrange@subsubsubappendix@format@first%
      \Crefrange@subsubappendix@format@first}{}%
    \@ifundefined{crefrange@subsubsubappendix@format@second}{%
      \let\crefrange@subsubsubappendix@format@second%
      \crefrange@subsubappendix@format@second}{}%
    \@ifundefined{Crefrange@subsubsubappendix@format@second}{%
      \let\Crefrange@subsubsubappendix@format@second%
      \Crefrange@subsubappendix@format@second}{}%
    \@ifundefined{crefrange@subsubsubappendix@format@middle}{%
      \let\crefrange@subsubsubappendix@format@middle%
      \crefrange@subsubappendix@format@middle}{}%
    \@ifundefined{Crefrange@subsubsubappendix@format@middle}{%
      \let\Crefrange@subsubsubappendix@format@middle%
      \Crefrange@subsubappendix@format@middle}{}%
    \@ifundefined{crefrange@subsubsubappendix@format@last}{%
      \let\crefrange@subsubsubappendix@format@last%
      \crefrange@subsubappendix@format@last}{}%
    \@ifundefined{Crefrange@subsubsubappendix@format@last}{%
      \let\Crefrange@subsubsubappendix@format@last%
      \Crefrange@subsubappendix@format@last}{}%
    \@ifundefined{cref@subfigure@format}{%
      \let\cref@subfigure@format%
      \cref@figure@format}{}%
    \@ifundefined{Cref@subfigure@format}{%
      \let\Cref@subfigure@format%
      \Cref@figure@format}{}%
    \@ifundefined{crefrange@subfigure@format}{%
      \let\crefrange@subfigure@format%
      \crefrange@figure@format}{}%
    \@ifundefined{Crefrange@subfigure@format}{%
      \let\Crefrange@subfigure@format%
      \Crefrange@figure@format}{}%
    \@ifundefined{cref@subfigure@format@first}{%
      \let\cref@subfigure@format@first%
      \cref@figure@format@first}{}%
    \@ifundefined{Cref@subfigure@format@first}{%
      \let\Cref@subfigure@format@first%
      \Cref@figure@format@first}{}%
    \@ifundefined{cref@subfigure@format@second}{%
      \let\cref@subfigure@format@second%
      \cref@figure@format@second}{}%
    \@ifundefined{Cref@subfigure@format@second}{%
      \let\Cref@subfigure@format@second%
      \Cref@figure@format@second}{}%
    \@ifundefined{cref@subfigure@format@middle}{%
      \let\cref@subfigure@format@middle%
      \cref@figure@format@middle}{}%
    \@ifundefined{Cref@subfigure@format@middle}{%
      \let\Cref@subfigure@format@middle%
      \Cref@figure@format@middle}{}%
    \@ifundefined{cref@subfigure@format@last}{%
      \let\cref@subfigure@format@last%
      \cref@figure@format@last}{}%
    \@ifundefined{Cref@subfigure@format@last}{%
      \let\Cref@subfigure@format@last%
      \Cref@figure@format@last}{}%
    \@ifundefined{crefrange@subfigure@format@first}{%
      \let\crefrange@subfigure@format@first%
      \crefrange@figure@format@first}{}%
    \@ifundefined{Crefrange@subfigure@format@first}{%
      \let\Crefrange@subfigure@format@first%
      \Crefrange@figure@format@first}{}%
    \@ifundefined{crefrange@subfigure@format@second}{%
      \let\crefrange@subfigure@format@second%
      \crefrange@figure@format@second}{}%
    \@ifundefined{Crefrange@subfigure@format@second}{%
      \let\Crefrange@subfigure@format@second%
      \Crefrange@figure@format@second}{}%
    \@ifundefined{crefrange@subfigure@format@middle}{%
      \let\crefrange@subfigure@format@middle%
      \crefrange@figure@format@middle}{}%
    \@ifundefined{Crefrange@subfigure@format@middle}{%
      \let\Crefrange@subfigure@format@middle%
      \Crefrange@figure@format@middle}{}%
    \@ifundefined{crefrange@subfigure@format@last}{%
      \let\crefrange@subfigure@format@last%
      \crefrange@figure@format@last}{}%
    \@ifundefined{Crefrange@subfigure@format@last}{%
      \let\Crefrange@subfigure@format@last%
      \Crefrange@figure@format@last}{}%
    \@ifundefined{cref@subtable@format}{%
      \let\cref@subtable@format%
      \cref@table@format}{}%
    \@ifundefined{Cref@subtable@format}{%
      \let\Cref@subtable@format%
      \Cref@table@format}{}%
    \@ifundefined{crefrange@subtable@format}{%
      \let\crefrange@subtable@format%
      \crefrange@table@format}{}%
    \@ifundefined{Crefrange@subtable@format}{%
      \let\Crefrange@subtable@format%
      \Crefrange@table@format}{}%
    \@ifundefined{cref@subtable@format@first}{%
      \let\cref@subtable@format@first%
      \cref@table@format@first}{}%
    \@ifundefined{Cref@subtable@format@first}{%
      \let\Cref@subtable@format@first%
      \Cref@table@format@first}{}%
    \@ifundefined{cref@subtable@format@second}{%
      \let\cref@subtable@format@second%
      \cref@table@format@second}{}%
    \@ifundefined{Cref@subtable@format@second}{%
      \let\Cref@subtable@format@second%
      \Cref@table@format@second}{}%
    \@ifundefined{cref@subtable@format@middle}{%
      \let\cref@subtable@format@middle%
      \cref@table@format@middle}{}%
    \@ifundefined{Cref@subtable@format@middle}{%
      \let\Cref@subtable@format@middle%
      \Cref@table@format@middle}{}%
    \@ifundefined{cref@subtable@format@last}{%
      \let\cref@subtable@format@last%
      \cref@table@format@last}{}%
    \@ifundefined{Cref@subtable@format@last}{%
      \let\Cref@subtable@format@last%
      \Cref@table@format@last}{}%
    \@ifundefined{crefrange@subtable@format@first}{%
      \let\crefrange@subtable@format@first%
      \crefrange@table@format@first}{}%
    \@ifundefined{Crefrange@subtable@format@first}{%
      \let\Crefrange@subtable@format@first%
      \Crefrange@table@format@first}{}%
    \@ifundefined{crefrange@subtable@format@second}{%
      \let\crefrange@subtable@format@second%
      \crefrange@table@format@second}{}%
    \@ifundefined{Crefrange@subtable@format@second}{%
      \let\Crefrange@subtable@format@second%
      \Crefrange@table@format@second}{}%
    \@ifundefined{crefrange@subtable@format@middle}{%
      \let\crefrange@subtable@format@middle%
      \crefrange@table@format@middle}{}%
    \@ifundefined{Crefrange@subtable@format@middle}{%
      \let\Crefrange@subtable@format@middle%
      \Crefrange@table@format@middle}{}%
    \@ifundefined{crefrange@subtable@format@last}{%
      \let\crefrange@subtable@format@last%
      \crefrange@table@format@last}{}%
    \@ifundefined{Crefrange@subtable@format@last}{%
      \let\Crefrange@subtable@format@last%
      \Crefrange@table@format@last}{}%
    \@ifundefined{cref@enumii@format}{%
      \let\cref@enumii@format%
      \cref@enumi@format}{}%
    \@ifundefined{Cref@enumii@format}{%
      \let\Cref@enumii@format%
      \Cref@enumi@format}{}%
    \@ifundefined{crefrange@enumii@format}{%
      \let\crefrange@enumii@format%
      \crefrange@enumi@format}{}%
    \@ifundefined{Crefrange@enumii@format}{%
      \let\Crefrange@enumii@format%
      \Crefrange@enumi@format}{}%
    \@ifundefined{cref@enumii@format@first}{%
      \let\cref@enumii@format@first%
      \cref@enumi@format@first}{}%
    \@ifundefined{Cref@enumii@format@first}{%
      \let\Cref@enumii@format@first%
      \Cref@enumi@format@first}{}%
    \@ifundefined{cref@enumii@format@second}{%
      \let\cref@enumii@format@second%
      \cref@enumi@format@second}{}%
    \@ifundefined{Cref@enumii@format@second}{%
      \let\Cref@enumii@format@second%
      \Cref@enumi@format@second}{}%
    \@ifundefined{cref@enumii@format@middle}{%
      \let\cref@enumii@format@middle%
      \cref@enumi@format@middle}{}%
    \@ifundefined{Cref@enumii@format@middle}{%
      \let\Cref@enumii@format@middle%
      \Cref@enumi@format@middle}{}%
    \@ifundefined{cref@enumii@format@last}{%
      \let\cref@enumii@format@last%
      \cref@enumi@format@last}{}%
    \@ifundefined{Cref@enumii@format@last}{%
      \let\Cref@enumii@format@last%
      \Cref@enumi@format@last}{}%
    \@ifundefined{crefrange@enumii@format@first}{%
      \let\crefrange@enumii@format@first%
      \crefrange@enumi@format@first}{}%
    \@ifundefined{Crefrange@enumii@format@first}{%
      \let\Crefrange@enumii@format@first%
      \Crefrange@enumi@format@first}{}%
    \@ifundefined{crefrange@enumii@format@second}{%
      \let\crefrange@enumii@format@second%
      \crefrange@enumi@format@second}{}%
    \@ifundefined{Crefrange@enumii@format@second}{%
      \let\Crefrange@enumii@format@second%
      \Crefrange@enumi@format@second}{}%
    \@ifundefined{crefrange@enumii@format@middle}{%
      \let\crefrange@enumii@format@middle%
      \crefrange@enumi@format@middle}{}%
    \@ifundefined{Crefrange@enumii@format@middle}{%
      \let\Crefrange@enumii@format@middle%
      \Crefrange@enumi@format@middle}{}%
    \@ifundefined{crefrange@enumii@format@last}{%
      \let\crefrange@enumii@format@last%
      \crefrange@enumi@format@last}{}%
    \@ifundefined{Crefrange@enumii@format@last}{%
      \let\Crefrange@enumii@format@last%
      \Crefrange@enumi@format@last}{}%
    \@ifundefined{cref@enumiii@format}{%
      \let\cref@enumiii@format%
      \cref@enumii@format}{}%
    \@ifundefined{Cref@enumiii@format}{%
      \let\Cref@enumiii@format%
      \Cref@enumii@format}{}%
    \@ifundefined{crefrange@enumiii@format}{%
      \let\crefrange@enumiii@format%
      \crefrange@enumii@format}{}%
    \@ifundefined{Crefrange@enumiii@format}{%
      \let\Crefrange@enumiii@format%
      \Crefrange@enumii@format}{}%
    \@ifundefined{cref@enumiii@format@first}{%
      \let\cref@enumiii@format@first%
      \cref@enumii@format@first}{}%
    \@ifundefined{Cref@enumiii@format@first}{%
      \let\Cref@enumiii@format@first%
      \Cref@enumii@format@first}{}%
    \@ifundefined{cref@enumiii@format@second}{%
      \let\cref@enumiii@format@second%
      \cref@enumii@format@second}{}%
    \@ifundefined{Cref@enumiii@format@second}{%
      \let\Cref@enumiii@format@second%
      \Cref@enumii@format@second}{}%
    \@ifundefined{cref@enumiii@format@middle}{%
      \let\cref@enumiii@format@middle%
      \cref@enumii@format@middle}{}%
    \@ifundefined{Cref@enumiii@format@middle}{%
      \let\Cref@enumiii@format@middle%
      \Cref@enumii@format@middle}{}%
    \@ifundefined{cref@enumiii@format@last}{%
      \let\cref@enumiii@format@last%
      \cref@enumii@format@last}{}%
    \@ifundefined{Cref@enumiii@format@last}{%
      \let\Cref@enumiii@format@last%
      \Cref@enumii@format@last}{}%
    \@ifundefined{crefrange@enumiii@format@first}{%
      \let\crefrange@enumiii@format@first%
      \crefrange@enumii@format@first}{}%
    \@ifundefined{Crefrange@enumiii@format@first}{%
      \let\Crefrange@enumiii@format@first%
      \Crefrange@enumii@format@first}{}%
    \@ifundefined{crefrange@enumiii@format@second}{%
      \let\crefrange@enumiii@format@second%
      \crefrange@enumii@format@second}{}%
    \@ifundefined{Crefrange@enumiii@format@second}{%
      \let\Crefrange@enumiii@format@second%
      \Crefrange@enumii@format@second}{}%
    \@ifundefined{crefrange@enumiii@format@middle}{%
      \let\crefrange@enumiii@format@middle%
      \crefrange@enumii@format@middle}{}%
    \@ifundefined{Crefrange@enumiii@format@middle}{%
      \let\Crefrange@enumiii@format@middle%
      \Crefrange@enumii@format@middle}{}%
    \@ifundefined{crefrange@enumiii@format@last}{%
      \let\crefrange@enumiii@format@last%
      \crefrange@enumii@format@last}{}%
    \@ifundefined{Crefrange@enumiii@format@last}{%
      \let\Crefrange@enumiii@format@last%
      \Crefrange@enumii@format@last}{}%
    \@ifundefined{cref@enumiv@format}{%
      \let\cref@enumiv@format%
      \cref@enumiii@format}{}%
    \@ifundefined{Cref@enumiv@format}{%
      \let\Cref@enumiv@format%
      \Cref@enumiii@format}{}%
    \@ifundefined{crefrange@enumiv@format}{%
      \let\crefrange@enumiv@format%
      \crefrange@enumiii@format}{}%
    \@ifundefined{Crefrange@enumiv@format}{%
      \let\Crefrange@enumiv@format%
      \Crefrange@enumiii@format}{}%
    \@ifundefined{cref@enumiv@format@first}{%
      \let\cref@enumiv@format@first%
      \cref@enumiii@format@first}{}%
    \@ifundefined{Cref@enumiv@format@first}{%
      \let\Cref@enumiv@format@first%
      \Cref@enumiii@format@first}{}%
    \@ifundefined{cref@enumiv@format@second}{%
      \let\cref@enumiv@format@second%
      \cref@enumiii@format@second}{}%
    \@ifundefined{Cref@enumiv@format@second}{%
      \let\Cref@enumiv@format@second%
      \Cref@enumiii@format@second}{}%
    \@ifundefined{cref@enumiv@format@middle}{%
      \let\cref@enumiv@format@middle%
      \cref@enumiii@format@middle}{}%
    \@ifundefined{Cref@enumiv@format@middle}{%
      \let\Cref@enumiv@format@middle%
      \Cref@enumiii@format@middle}{}%
    \@ifundefined{cref@enumiv@format@last}{%
      \let\cref@enumiv@format@last%
      \cref@enumiii@format@last}{}%
    \@ifundefined{Cref@enumiv@format@last}{%
      \let\Cref@enumiv@format@last%
      \Cref@enumiii@format@last}{}%
    \@ifundefined{crefrange@enumiv@format@first}{%
      \let\crefrange@enumiv@format@first%
      \crefrange@enumiii@format@first}{}%
    \@ifundefined{Crefrange@enumiv@format@first}{%
      \let\Crefrange@enumiv@format@first%
      \Crefrange@enumiii@format@first}{}%
    \@ifundefined{crefrange@enumiv@format@second}{%
      \let\crefrange@enumiv@format@second%
      \crefrange@enumiii@format@second}{}%
    \@ifundefined{Crefrange@enumiv@format@second}{%
      \let\Crefrange@enumiv@format@second%
      \Crefrange@enumiii@format@second}{}%
    \@ifundefined{crefrange@enumiv@format@middle}{%
      \let\crefrange@enumiv@format@middle%
      \crefrange@enumiii@format@middle}{}%
    \@ifundefined{Crefrange@enumiv@format@middle}{%
      \let\Crefrange@enumiv@format@middle%
      \Crefrange@enumiii@format@middle}{}%
    \@ifundefined{crefrange@enumiv@format@last}{%
      \let\crefrange@enumiv@format@last%
      \crefrange@enumiii@format@last}{}%
    \@ifundefined{Crefrange@enumiv@format@last}{%
      \let\Crefrange@enumiv@format@last%
      \Crefrange@enumiii@format@last}{}%
    \@ifundefined{cref@enumv@format}{%
      \let\cref@enumv@format%
      \cref@enumiv@format}{}%
    \@ifundefined{Cref@enumv@format}{%
      \let\Cref@enumv@format%
      \Cref@enumiv@format}{}%
    \@ifundefined{crefrange@enumv@format}{%
      \let\crefrange@enumv@format%
      \crefrange@enumiv@format}{}%
    \@ifundefined{Crefrange@enumv@format}{%
      \let\Crefrange@enumv@format%
      \Crefrange@enumiv@format}{}%
    \@ifundefined{cref@enumv@format@first}{%
      \let\cref@enumv@format@first%
      \cref@enumiv@format@first}{}%
    \@ifundefined{Cref@enumv@format@first}{%
      \let\Cref@enumv@format@first%
      \Cref@enumiv@format@first}{}%
    \@ifundefined{cref@enumv@format@second}{%
      \let\cref@enumv@format@second%
      \cref@enumiv@format@second}{}%
    \@ifundefined{Cref@enumv@format@second}{%
      \let\Cref@enumv@format@second%
      \Cref@enumiv@format@second}{}%
    \@ifundefined{cref@enumv@format@middle}{%
      \let\cref@enumv@format@middle%
      \cref@enumiv@format@middle}{}%
    \@ifundefined{Cref@enumv@format@middle}{%
      \let\Cref@enumv@format@middle%
      \Cref@enumiv@format@middle}{}%
    \@ifundefined{cref@enumv@format@last}{%
      \let\cref@enumv@format@last%
      \cref@enumiv@format@last}{}%
    \@ifundefined{Cref@enumv@format@last}{%
      \let\Cref@enumv@format@last%
      \Cref@enumiv@format@last}{}%
    \@ifundefined{crefrange@enumv@format@first}{%
      \let\crefrange@enumv@format@first%
      \crefrange@enumiv@format@first}{}%
    \@ifundefined{Crefrange@enumv@format@first}{%
      \let\Crefrange@enumv@format@first%
      \Crefrange@enumiv@format@first}{}%
    \@ifundefined{crefrange@enumv@format@second}{%
      \let\crefrange@enumv@format@second%
      \crefrange@enumiv@format@second}{}%
    \@ifundefined{Crefrange@enumv@format@second}{%
      \let\Crefrange@enumv@format@second%
      \Crefrange@enumiv@format@second}{}%
    \@ifundefined{crefrange@enumv@format@middle}{%
      \let\crefrange@enumv@format@middle%
      \crefrange@enumiv@format@middle}{}%
    \@ifundefined{Crefrange@enumv@format@middle}{%
      \let\Crefrange@enumv@format@middle%
      \Crefrange@enumiv@format@middle}{}%
    \@ifundefined{crefrange@enumv@format@last}{%
      \let\crefrange@enumv@format@last%
      \crefrange@enumiv@format@last}{}%
    \@ifundefined{Crefrange@enumv@format@last}{%
      \let\Crefrange@enumv@format@last%
      \Crefrange@enumiv@format@last}{}%
  \let\cref@language\relax%
}%  end of \AtBeginDocument
\InputIfFileExists{cleveref.cfg}%
  {\PackageInfo{cleveref}{reading definitions from cleveref.cfg}}{}
\endinput
%%
%% End of file `cleveref.sty'.

